Quantifying Spatial Under-reporting Disparities in Resident Crowdsourcing

Modern city governance relies heavily on crowdsourcing to identify problems such as downed trees and power lines. A major concern is that residents do not report problems at the same rates, with heterogeneous reporting delays directly translating to downstream disparities in how quickly incidents can be addressed. Here we develop a method to identify reporting delays without using external ground-truth data. Our insight is that the rates at which duplicate reports are made about the same incident can be leveraged to disambiguate whether an incident has occurred by investigating its reporting rate once it has occurred. We apply our method to over 100,000 resident reports made in New York City and to over 900,000 reports made in Chicago, finding that there are substantial spatial and socioeconomic disparities in how quickly incidents are reported. We further validate our methods using external data and demonstrate how estimating reporting delays leads to practical insights and interventions for a more equitable, efficient government service.

==> abstract_anon.tex <==
Modern city governance relies heavily on crowdsourcing (``co-production'') to identify problems such as downed trees and power-lines. A major concern is that residents do not report problems at the same rates, with heterogeneous reporting delays directly translating to downstream disparities in how quickly incidents can be addressed. Measuring such under-reporting is a difficult statistical task, as, by definition, we do not observe incidents that are not reported or when reported incidents first occurred. Thus, low reporting rates and low ground-truth incident rates cannot be naively distinguished. We develop a method to identify (heterogeneous) reporting rates, without using external ground truth data. Our insight is that rates on \textit{duplicate} reports about the same incident can be leveraged to disambiguate whether an incident has occurred with its reporting rate once it has occurred. Using this idea, we reduce the question to a standard Poisson rate estimation task---even though the full incident reporting interval is also unobserved.

We apply our method to over \num{100000} resident reports made to the New York City Department of Parks and Recreation and to over \num{900000} reports made to the Chicago Department of Transportation and Department of Water Management, finding that there are substantial spatial disparities in how quickly incidents are reported, even after controlling for incident characteristics -- some neighborhoods report three times as quickly as do others. These spatial disparities correspond to socio-economic characteristics: in NYC, higher population density, fraction of people with college degrees, income, and fraction of population that is White all positively correlate with reporting rates.

Finally, leveraging a collaboration with the NYC Department of Parks and Recreation, we demonstrate how estimating reporting delays leads to \textit{practical} insights and interventions for more equitable, efficient government service. 

% \blfootnote{
% 			We benefited from discussions with Allison Koenecke, Alex Kobald, Ben Laufer, Emma Pierson, Aaron Schein, Kiran Shiragur, and Qian Xie. We also thank the New York Department of Parks and Recreation for their valuable work, inside knowledge, and data, and we especially thank Fiona Watt.	This work was funded in part by the Urban Tech Hub at Cornell Tech, and we especially thank Anthony Townsend and Nneka Sobers.
% 	}



==> journal_subsections/journal_1_intro.tex <==


\begin{quote}
	If a tree falls in a forest, and no one reports it... does the city know about it?
\end{quote}
%
%
%	1. 311 systems are large and important, they determine allocation of city resources
%
%
Cities are complex socio-technical systems comprised of physical and human infrastructure, navigated by millions of people daily. A core part of monitoring such systems is crowdsourcing (or ``co-production'' \cite{yuan_co-production_2019,brabham_crowdsourcing_2015}), in which people report problems that they encounter; the New York City 311 system, for example, received \num{2592831} reports in 2020, and more than one hundred North American cities employ similar systems. Such reports are necessary, as they provide a real-time reflection on on-the-ground conditions that the city cannot hope to otherwise be aware of \citep{schwester2009examination, hacker_spatiotemporal_2020,minkoff_nyc_2016, lee_crowdsourcing_2021-1}. These reports are used alongside internal data collection and automated sensor technology to make both immediate decisions---such as which dangerous, downed trees to inspect and fix---and longer-term planning decisions, such as which streets to resurface. For example, the NYC Department of Parks and Recreation sends a forester to inspect about $\frac23$ of reports, and the incidents deemed risky (about $\frac12$ of inspected incidents) are resolved by a maintenance crew.

%2. However, if not used equitably, that's a problem. There is a large literature trying to measure this

While such reporting systems have gained popularity in the last few decades, there are many unresolved challenges in using reports efficiently and equitably. In particular, one long-standing concern is whether residents\footnote{We use the term ``residents'' to denote anyone who might report an issue to the 311 system, including visitors.} equitably use the system; or whether, conditional on experiencing the same issues, some residents are more likely to log a report and request government services \citep{thijssen2016you} -- for example, if socio-economically privileged neighborhoods submit more incident reports. If such reporting behavior is heterogeneous, then government services that rely on such reporting will also be inequitable. Though it is commonly believed that reporting behavior is heterogeneous, previous studies vary greatly in the quantification of such bias and how to attribute it to socio-economic or geographic characteristics
\citep{kontokosta_bias_2021,kontokosta_equity_2017,minkoff_nyc_2016,hacker_spatiotemporal_2020, clark_coproduction_2013,wu2020determinants, o2016311, thijssen2016you, vedlitz1980citizen,mclafferty_placing_2020, xu_closing_2020}.


%3. The issues with the current approach is either they can't identify, or they need ground truth to do so. This .

The central methodological challenge is the same reason that cities must rely on this information: ground truth conditions are unknown. This induces a missing data challenge: researchers do not observe what incidents occurred, or when they occurred. Thus, it is difficult to determine whether one neighborhood is \textit{under-reporting} issues compared to other neighborhoods, or whether they truly experience fewer issues (due to, e.g., differences in infrastructure). Previous work either does not attempt to distinguish between these cases (implicitly assuming that incident rates are similar across areas), or employs external data to construct \textit{proxies} for ground truth incident rates (such as number of trees, length of roadways). While accurate proxies can distinguish between incident rates and reporting rates, they may be difficult to construct or may not be precise enough to distinguish between types of incidents (e.g., whether reporting behavior differs by incident risk).

\parbold{A method to identify reporting rates without ground truth data.} In this work, we propose a method to identify (heterogeneous) reporting rates, using \textit{just} the reporting data itself. Our insight is that we can use information on \textit{duplicate} reports about the same incident (which cities commonly log), to \textit{disentangle} the reporting process from the incident occurrence process, thus identify reporting rates \textit{conditional on an incident having occurred}. This insight originates from the \textit{missing species} estimation literature, where the number of \textit{duplicate} observations provides evidence regarding the existence of unseen species \citep{orlitsky_optimal_2016, wu_chebyshev_2016, han2021competitive, charikar2019efficient}.

% Our setting differs from the classic \textit{missing species} formulation, in that the set of incidents is not static: new incidents occur (e.g., a tree falls down), and are resolved (the city fixes the issue, or it naturally disappears). And, even for observed incidents (those that are reported), we do not know \textit{when} they occurred, or \textit{how long} the incident existed. Thus, naively, we do not know, e.g., whether the incident was reported twice over a possible three month or one week period. This difference matters, as the possible reporting period varies substantially with incident characteristics and reporting behavior (e.g., hazardous incidents are reported and addressed more quickly).

Our setting differs from the classic \textit{missing species} formulation, in that the set of incidents, as opposed to species, is not static: new incidents occur and are resolved all the time. And, even for observed incidents (those that are reported), we do not know \textit{when} they occurred, or \textit{how long} the incident existed. Thus, naively, we do not know, e.g., whether the incident was reported twice over a possible three month or one week period. This difference matters, as the possible reporting period varies substantially with incident characteristics and reporting behavior (e.g., hazardous incidents are reported and addressed more quickly).

% We show how to nevertheless convert the task to a standard \textit{Poisson rate estimation} challenge, for which a large empirical and theoretical literature exists. In particular, one can use the number of reports between time of the first report (but not including it) and an estimated death time (that may depend on the data, e.g., time of the reports or when the incident was inspected), to recover a {Poisson} likelihood with a corresponding rate function. The method is valid if the estimated death time is an \textit{under-}estimate of the resolution time and is a \textit{stopping time} (does not depend on the future).

We show how to nevertheless convert the task to a standard \textit{Poisson rate estimation} challenge, for which a large empirical and theoretical literature exists. In particular, one can use the number of reports between time of the first report (but not including it) and an estimated death time, to recover a {Poisson} likelihood with a corresponding rate function. The method is valid if the estimated death time is an \textit{under-}estimate of the resolution time and is a \textit{stopping time} (does not depend on the future).

Then, we can leverage standard Poisson rate estimation methods (for example, use maximum-likelihood estimates(MLE) or train a Poisson regression model) to recover the rates that incidents of different types and in various neighborhoods are reported, conditional on the incident having occurred.

%5. Application oriented
%a. We apply it to Parks data, using data provided to us…

\parbold{Applying our method to understand (in)equity in resident crowdsourcing usage.} We apply our method to mass number of resident reports made in New York City and the City of Chicago \todo{potentially another city}, using mainly publicly accessible data, with the addition of internal logs on incident inspection outcomes and work orders in the New York case.
%
Using a Bayesian Poisson regression framework, we estimate how the reporting rate varies as a function of incident characteristics (e.g., the type of request), space, and socio-economic characteristics of the neighborhood in which the incident occurred.

We illustrate that our method is indeed precise enough to find differences in reporting rates; for example, we find that reports for riskier incidents are submitted at substantially higher rates across different cities, conditional on the incident having occurred.
%
We then study spatial and socio-economic heterogeneity. We find that there are substantial inter-location reporting differences; for example, comparing census tract level fixed effects, we find that reports occur at a three times higher rate in downtown Manhattan than in uptown Manhattan, even after controlling for the incident-level characteristics. We further find that factors like race/ethnicity and education levels are  associated with reporting rates, though such socio-economic characteristics cannot explain much of the spatial heterogeneity. These findings suggest that the allocation of government services, if reliant on incident reporting, may neither be efficient nor equitable.

\todo{update this summary with updated application}

%works in high dimension, use bayesian poisson regression approaches

\smallskip

We believe that our method is a general, powerful approach to understanding reporting behavior in resident crowdsourcing systems, delivering precise reporting estimates without requiring ground truth data---only duplicate report data, that are already collected by city agencies. The rest of this paper is organized as follows. \todo{organize}





==> journal_subsections/journal_1_relatedwork.tex <==
\subsection{Related Work}
\label{sec:related}
Our work is most closely related to literature studying equity and efficiency in co-production systems, often called 311 systems. Our empirical approach is motivated by the \textit{missing species} literature, and we employ Bayesian Poisson regression approaches. It broadly connects to commonly considered crowdsourcing and civic engagement challenges, including equitable participation.


\paragraph{Equity and efficiency in co-production systems.} Given the importance of 311-like systems in allocating government services, there has been much interest in quantifying how efficient and equitable these systems are. This work aims at answering the question of whether \textit{reporting} behavior is similar across socio-economic groups, with a particular focus on the type of reporting behavior known as \textit{under-reporting}, which is when people, faced with similar problems, differentially report those problems to the government. Such differences might emerge, for example, due to access to communications technologies, familiarity with the system, or trust in government \cite{buell2021surfacing}. As discussed above, the biggest challenge to studying \textit{under-reporting} is that researchers rarely directly observe an incident \textit{unless it is reported}. It is thus difficult to disentangle whether certain areas have fewer reports because problems truly occur less frequently there, or whether people in those areas are reporting less frequently given a similar distribution of problems. Towards this challenge, previous literature either assume a uniform incident occurrence, thus concluding any heterogeneity in the observed reports is a result of differential reporting rate \citep{clark_coproduction_2013,cavallo_digital_2014,minkoff_nyc_2016}; or construct proxies to account for differences in incident occurrence, and then compare the estimates with observed rates \citep{kontokosta_bias_2021, hacker_spatiotemporal_2020, pak_fixmystreet_2017, kontokosta_equity_2017}. Both lines of work require some form of external data or strong assumptions, which the technique we propose does not.




\paragraph{Missing species and Bayesian estimation.} The central idea of our work is that one can leverage \textit{duplicate} reports about the same incident to identify the true incident rate from the reporting rate. This insight derives from the \textit{missing species problem} \citep{goodtoulmin}, where the number of \textit{duplicate} observations provides evidence regarding the existence of unseen species. 



% \paragraph{Other crowdsourcing and civic engagement settings.} 311 (or `co-production') systems are part of a broader constellation of crowdsourcing and civic engagement systems, in which residents contribute to governmental decisions such as legislation and resource allocation; for example, participatory budgeting and deliberative democracy are well studied \cite{aziz2021participatory,pateman_participatory_2012,cabannes_participatory_2004,lee_crowdsourcing_2014,mcdermott_building_2010,posner_voting_2015,procaccia_approximate_2009,sintomer2008porto,gilman2020transformative,garg2019iterative,Aziz2021,FREEMAN2021105234,garg2021markets,goel2019knapsack,fishkin2018deliberative,deliberationjuryconsistent}. Whether participation is equitable is a common worry \citep{griffinjiao2019,brabham2009crowdsourcing,hudson2018does,shortall2021inclusion}, and others have attempted to improve representative-ness in such civic engagement systems \cite{gelauff2020,flanigan2021fair}.  Our setting also broadly relates to the peer prediction and grading literature, in evaluating crowdsourced answers without ground truth \citep{miller2005eliciting,witkowski2012peer,shnayder2016informed,liu2017machine,agarwal2020peer}. Surprisingly, given the popularity, scale, and importance of 311 systems---among the biggest, most consequential crowdsourcing systems in continuous use---to our knowledge their design (either a market design or operations perspective) has not been considered in the EconCS community.









==> journal_subsections/journal_2_model.tex <==

\label{sec:model}

 \begin{figure}[tbh]
	\centering
	\includegraphics[width=\textwidth]{plots/data_gen_1.pdf}
	\caption{Model of resident reports of an incident $i$ of type $\theta$. Observed and unobserved events are marked with solid and dotted lines, respectively. In this example, there are a total of 3 reports made about this incident. When the reporting rate is an homogeneous Poisson process with rate $\lambda_\theta$, the average reporting delay is $\frac{1}{\lambda_\theta}$.}
	\label{fig:reports_gen}
\end{figure}

We now introduce our model for how resident reports are generated, as well as our research questions. The data are composed of a set of resident \textbf{reports}, each belonging to an \textbf{incident} $i$ of type $\theta$.  Type $\theta$ encodes geographic and incident-specific (e.g., whether it is a hazard) characteristics.  \Cref{fig:reports_gen} illustrates the model for a given incident.

\parbold{Incident birth and death.} Incidents of type $\theta$ occur (``are born'') according to a random process parameterized by $\Lambda_\theta$. (For example, a homogeneous Poisson process with rate $\Lambda_\theta$). For each incident $i$, let $t_i$ denote its birth time. Furthermore, the incident `dies' at some time $t_i + T_i$, and no more reports are logged. The death time reflects, for example, a completed work order fixing the issue, or reports no longer being logged because the issue has been inspected. Though the birth and death processes of incidents may induce other interesting research questions, we do not make any further assumptions on them, as they are beyond the scope of this paper.


\parbold{Reports.} Incidents are not directly observed by the city. Rather, the city observes {reports} made by the public, once an incident has occurred. There are two notable facts regarding reports. First, they may not come in immediately after an incident occurs -- it takes a (random) amount of time for someone to first notice an incident and consider it worth reporting. Second, there often are \textit{duplicate} reports, about the same incident. Multiple residents may encounter the same incident and report it. Crucially, city agencies often identify and log such duplicates, as it is important to do so when deciding which reports to address and auditing response rates and times.

 For an incident $i$ of type $\theta$, we assume that---while it is alive, i.e., in time $[t_i, t_i + T_i]$---reports are submitted according to a (potentially non-homogeneous) Poisson process, with rate $\lambda_\theta(\tau)$ at incident age $\tau \in [0, T_i]$. Thus, the number of reports $M_i$ for incident $i$ follows a Poisson process, $M_i \sim \text{Poisson}\left(\int_{\tau = 0}^{T_i} \lambda_\theta(\tau) d\tau\right)$.






\parbold{Observed data.} We observe reports and city actions. Each report comes with a time-stamp and identifies its corresponding incident $i$ (thus, duplicate reports are assumed to be accurately connected to previous reports of the same incident). For each incident, we further know its type $\theta$ (as detailed in \Cref{sec:datapplication}, type $\theta$ can be composed of both data available at report time, or after an inspection; we assume each report about an incident is identical in terms of $\theta$).

Putting things together, from the viewpoint of the 311 system (and researchers), the observed data for a time interval $(0, T)$ consists of the following, for each type $\theta$. Suppose there are $N_\theta$ incidents of the type. We observe $N^{\obs}_\theta \leq N_\theta$ of these incidents, corresponding to the incidents $i$ with at least one report, $M_i \geq 1$. For each such incident, we observe $M_i$ and each report time.

Finally, we observe how the agency responded to the incident, such as when an inspection was completed, the outcome of the inspection, and the details of any completed work order.



\parbold{Research questions.} In this work, we are primarily interested in auditing the efficiency and equity of the reporting process: how quickly are incidents reported, and how does that reporting rate $\lambda_\theta$ vary with the incident type $\theta$? (While we primarily measure and interpret our results in terms of reporting rates $\lambda_\theta$, estimating this rate also allows us to calculate, for example, the fraction of incidents reported within a certain time period and other operationally relevant measures.)


The primary methodological task is overcoming the missing data challenge: we do not observe incidents that are never reported, nor birth times $t_i$ of the incidents that are reported. This missing data makes it difficult to distinguish between incident rate $\Lambda_\theta$ and reporting rate conditioned on an incident, $\lambda_\theta$. In fact, as we explain next in \Cref{sec:identification}, it is impossible to do so with just the above data, if one throws away the information on duplicates; our main insight is that by using this duplicate data, in contrast, one can identify $\lambda_\theta$ in practically reasonable settings.



\parbold{Model discussion.} As discussed in \Cref{sec:related}, \textit{mis-reporting} is also a concern in many settings. We in contrast assume that the reported types are correct (in the data section, if different reports for the same incident disagree, we keep the \textit{first} report type). Estimating such mis-reporting alongside under-reporting is an interesting avenue for future work. Furthermore, the data also enables calculating the \textit{inter-arrival times} between reports. Such information is valuable for estimating non-homogeneous Poisson rates, but we do not do so here. Finally, we note that our method does not directly consider \textit{causal} reasons that a neighborhood may have a lower reporting rate than another; \citet{buell2021surfacing} find that operational transparency increases trust in government and reporting rates, and technological access and familiarity may also play a role.


In what settings is the model applicable? First, while the incident occurrence process $\Lambda_\theta$ can be arbitrary, the reporting rates $\lambda_\theta$ must be Poisson --  reports about the same incident must be independent. This assumption requires filtering out duplicate reports made by the same individual, as we do in our application. Second, the analysis requires that the agency log information about duplicate reports; this is commonly done in co-production systems---e.g., \citet{kontokosta_equity_2017} mention filtering out duplicates in their work. While our data application focuses on reports to a single agency in NYC's 311 system, these requirements are widely met in other contexts, including beyond co-production systems.




This section lays the groundwork to estimate the rate function $\lambda_\theta$. There are two primary challenges: identification of $\lambda_\theta$ (primarily, disentangling reporting rates from incident occurrence rates $\Lambda_\theta$), and the high-dimensional nature of $\theta$ in our setting. \Cref{sec:identification} shows that $\lambda_\theta$ is identifiable -- using standard Poisson rate estimation techniques; then, we leverage this result in \Cref{sec:poissonreg} to develop Bayesian Poisson regression approaches to estimate $\lambda_\theta$ as a function of $\theta$. Finally, we evaluate our approach in simulation in \Cref{sec:simulation}.




\subsection{Identifying reporting rate $\lambda_\theta(\cdot)$}
\label{sec:identification}

Estimating reporting rates $\lambda_\theta$ as a function of $\theta$ is of interest to good governance activists and researchers, as 311 reports are a key data source in the allocation of government services. Existing approaches either do not disentangle reporting rates from incident rates, or use external data to do so. Here, we show, in contrast, that $\lambda_\theta$ is identifiable using just reporting data, \textit{if we use data on duplicate reports} about the same incident. In this section, we assume a \textit{fixed} incident type $\theta$, and so often omit it from the notation.


\subsubsection{Non-identifiability using just number of incidents observed} Our first result, however, formalizes that the task is impossible using just data on the total number of unique incidents observed for each type in a time interval $(0, T)$, even if both incident occurrence and reporting follow time-homogeneous Poisson processes, with $\Lambda_\theta(\tau) = \Lambda_\theta$ and $\lambda_\theta(\tau) = \lambda_\theta$.

\begin{restatable}[Non-identifiability of reporting rate]{proposition}{propnonidenti}\label{prop:identi} Consider the simplest setting: both incident occurrence and reporting follow time-homogeneous Poisson processes, with $\Lambda_\theta(\tau) = \Lambda_\theta$ and $\lambda_\theta(\tau) = \lambda_\theta$. Further, let incident reporting durations $T_i$ be distributed according to $F$. Then using just the number of observed incidents $N_\theta^\obs(T)$ of type $\theta$ in a known time duration $[0, T]$, the reporting rate $\lambda_\theta$ is not identifiable. In other words, $N_\theta^\obs(T)$ is a function of both $\Lambda_\theta$ and $\lambda_\theta$:
\begin{align*}
	&\lim_{T \to \infty} \frac{N_\theta^\obs(T)}{T} = \Lambda_{\theta}'\\
	\text{where\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,} &\Lambda_{\theta}' = \Lambda_{\theta}\left[1-\int_{0}^\infty\exp\left(-\lambda_\theta t\right)\text{d}F(t)\right].
\end{align*}
\end{restatable}

The proof follows from the observation that, conditional on the number of incidents that occurred, the number observed is a Binomially distributed random variable that depends on the reporting rate. The number of observed incidents thus depends on both reporting and incident rates; it is thus not possible to distinguish between high incident rate/low reporting rate and low incident rate/high reporting rate just based on the observed reports. An identical result holds if we only count the total number of reports. That result follows from compounding the reporting rate conditional on an incident being observed upon the observation rate. For brevity, the proofs for \Cref{prop:identi} and the later \Cref{thm:stoppingtimes} are omitted in this short version for brevity.


The idea -- confounding incident occurrence and reporting -- behind \Cref{prop:identi} is not novel, and has especially been pointed out in policing settings~\cite{lum2016predict}; e.g., recently in the context of predictive policing systems, \citet{akpinar2021effect} study the downstream consequences of mistakenly using $N_\theta^\obs(T)$ as a proxy for the incident rate. Nevertheless, many works in the literature use such a proxy. Next, we show how to disentangle reporting and incident rates, without needing external ground truth data, by using data on \textit{duplicate reports} about the same incident.





\subsubsection{Identifiability using data on duplicates}
\label{sec:convertingtopoissonregression}



Our main insight is that one can identify the reporting rate using \textit{duplicate} reports about the same incidents: the first incident report informs us that this incident exists, and the remaining reports identify the reporting rate.

% section outline
%	1. If we observed everything, just do Poisson regression
As starting intuition, suppose we observe every incident (even those without reports) and, for every incident, the birth times $t_i$ and death times $t_i + T_i$---that all events in \Cref{fig:reports_gen} are observed. Then one could directly apply standard Poisson estimation techniques in order to learn the rates $\lambda_\theta(\cdot)$ for each type $\theta$: under our assumptions, the number of reports for an incident $i$ follows a Poisson distribution, $M_i \sim \text{Poisson}\left(T_i \int_0^{T_i} \lambda_\theta(\tau)d\tau\right)$. Depending on the assumptions on the time-non-homogeneous nature of $\lambda_\theta(\cdot)$, the corresponding estimation challenge for $\lambda_\theta(\cdot)$ is tractable.

%2. First issue, only observe those for which M_i > 1; This is exactly the missing species problem. The key insight we use is duplicate…
The first complication is that we do not observe every incident, only those with at least one report, $M_i \geq 1$. Our first insight is that this challenge is akin to that in \textit{missing species} literature discussed above, where a biologist only knows of species they have spotted at least once. The key idea in that literature -- that we leverage and adapt -- is that the \textit{number of times} we observe a species \textit{that we have observed at least once} provides information about how many species exist but have not yet been observed. The conditioning removes the dependence on the birth process $\Lambda$. In particular, conditioning on observing each such species at least once, we can use the distribution of how many species we spot twice, thrice, etc, to estimate the rate at which one observes that species, and back out the probabilities for observing that kind of species at least once -- under some assumptions on how the rates at which one observes species multiple times relates to observing it the first time. As discussed in the related work, this line of work has a long history. Our central assumption is similar, that the rate of duplicate reports \textit{after} the first report about an incident $i$ -- after which the city has learned the incident exists -- is informative of the overall reporting rate.

%3. However, we have a second issue. For those we observe, we don't observe their birth times t_i, nor their death times T_i.
In our setting, however, there is a second complication that prevents us from using off-the-shelf  estimators from the {missing species} literature: incidents do not always exist (like species), but rather are born and die -- our system evolves over time, and we do not directly know $t_i$ or $t_i + T_i$ (as, by definition, the city only learns of incidents after they have been reported). Qualitatively, the difference is that we cannot naively distinguish between an incident being born a long time ago but with low reporting rate, or an incident just recently being born. Our second insight is that $\lambda_\theta(\cdot)$ is still identifiable, in a  (practically reasonable) setting described next.


%4. Here, we leverage the following result…

\textbf{Identification with stopping-time time intervals} Our empirical strategy is based on the following technical result, which shows that, even if the observation interval for a Poisson process is defined by \textit{stopping times}, the likelihood function can be decomposed such that we can leverage standard Poisson rate estimation techniques. Here, a time $t$ being a \textit{stopping time} means that it can depend on everything that occurs before that time (e.g., on the number of reports received up to time $t$), but, conditional on this past and type $\theta$, it is independent of the future and process parameter $\lambda$.

%a. And then the result, but just the first part
\begin{restatable}{theorem}{thmst}\label{thm:stoppingtimes}
	Consider each incident $i$, born and dead at unknown times $t_i$ and $t_i + T_i$. Suppose that, while alive and aged $\tau \in [0, T_i]$, the incident is reported at rate $\lambda(\tau)$.

	Let the data for incident $i$ be $D_i = (\tilde M_i, \tilde t_i, \tilde T_i)$, where $\tilde t_i$ is the start of an observation period, $\tilde T_i$ is the duration of that period, and $\tilde M_i$ is the number of reports observed in time period $(\tilde t_i, \tilde t_i + \tilde T_i]$. Further, suppose that $(\tilde t_i, \tilde t_i+ \tilde T_i] \subseteq [t_i, t_i + T_i]$ and that $\tilde t_i$ and $\tilde t_i + \tilde T_i$ are stopping times, adapted to the natural filtration of the Poisson process characterizing the reporting behavior, and independent of $\lambda$ given $\theta$.	Let $\tilde{Pr}(\{D_i\} | \lambda(\cdot))$ denote the likelihood function of the data, given the rate function $\lambda$. Then,
	\begin{align}
		\tilde{Pr}(\{D_i\} | \lambda(\cdot)) &= {Pr}(\{D_i\} | \lambda(\cdot)) g(\{D_i\}),
		\intertext{where ${Pr}({D_i} | \lambda(\cdot))$ corresponds to the standard Poisson likelihood with an appropriate rate function:}
		\tilde M_i &\sim \text{Poisson}\left(\int_{\tau = \tilde t_i - t_i}^{(\tilde t_i - t_i) + \tilde T_i } \lambda(\tau)d\tau \right), \label{eq:poissonnonhom}
		\intertext{and $g$ is a function that does not depend on $\lambda$. Thus, the MLE and the posterior distributions for $\lambda(\cdot)$ also match the corresponding Poisson values. For example, when reporting rate is homogeneous ($\lambda(\tau) \triangleq \lambda$), the maximum likelihood estimate for $\lambda$ is }
\hat{\lambda}^{MLE} &= \frac{\sum_{i}\tilde M_i}{\sum_{i}\tilde T_i}. \label{eq:MLE}
	\end{align}
The decomposition does not hold in general, if $\tilde t_i$, and $\tilde t_i + \tilde T_i$ are not stopping times.

\end{restatable}
%i. Note that this would be trivial from stopping time if T_i was fixed, but here as long as they are not functions of the future, we are fine.
%

The result follows directly from writing the likelihood function in terms of the report inter-arrival times, and then observing that the likelihood decomposes. We note that $\tilde t_i$ (the start of the observation period) being a stopping time not affecting estimation is a trivial consequence of the memory-less property for Poisson processes. Thus, if we had assumed fixed $T_i$ and $\tilde T_i$ (or random, but also independent of the sample path), the above result would immediately follow.
%
Surprisingly, we could not find rate estimation literature in which the length of each observation period $\tilde T_i$ depends on the sample path (but is a stopping time), and so require \Cref{thm:stoppingtimes}.

Why is the setting important? In our data, incidents may be fixed (via a work order) or reports may stop being tagged to the incident after an inspection -- these outcomes are represented by the death time $t_i + T_i$. However, these outcomes are \textit{potentially dependent on the reports}: for example, incidents with more reports or reported as a \textit{Hazard} type may be prioritized for an inspection or work order; \Cref{tab:Summary} suggests that, indeed, such prioritization occurs in our data. Without the above result, we would need to choose a fixed observation duration $\tilde T$ such that $\tilde t_i + \tilde T \leq t_i + T_i$ for all incidents $i$, leading us to discard much data. With \Cref{thm:stoppingtimes}, however, we can choose data dependent durations $\tilde T_i$, as described below.

Why is it necessary that $\tilde t_i + \tilde T_i$ be a stopping time, conditionally independent of the future and $\lambda$? Suppose we instead choose the end of the observation period $\tilde t_i + \tilde T_i$, as ``the time of the \textit{last} report for the incident.'' This time depends on the future, as we must know that there are no further reports. Then, our estimation for rate $\lambda(\cdot)$ would be biased upward, as we systematically exclude a time period in which the incident was alive but we know no more reports were submitted.


Finally, note that we also observe the inter-arrival times between reports; \Cref{thm:stoppingtimes} extends to using those as data (our proof in fact first writes down the likelihood in terms of the inter-arrivals, and then marginalizes them out). However, we exclude it from the statement for clarity, as our current model specifications (see \Cref{sec:poissonreg}) do not use this data.


\textbf{Applying the result to our setting} How do we apply \Cref{thm:stoppingtimes} to our setting? Given that we do not know birth time $t_i$ or lifetime $T_i$, we require a known interval $(\tilde t_i, \tilde t_i+ \tilde T_i] \subseteq [t_i, t_i + T_i]$ such that we know the number of reports in that interval, and that $\tilde t_i, \tilde t_i+ \tilde T_i$ are stopping times. 


The best choice for $\tilde t_i$ is the (observed) time of the first report, and so we count all reports after the first report and before our chosen end time $\tilde t_i + \tilde T_i$---this time is the earliest that we know the incident exists, and so it maximizes the interval length. This choice formalizes the idea that our method uses the first report to condition on an incident exists (and a time for it), and then other reports to identify the reporting rate.



Setting $\tilde T_i$ is a design choice. We require that the end time $\tilde t_i+ \tilde T_i$ is a stopping time, and that $\tilde t_i+ \tilde T_i \leq t_i + T_i$, i.e., that we do not extend the interval past when the incident can no longer be reported. Choosing too high a duration $\tilde T_i$ risks under-estimating $\lambda(\cdot)$; unfortunately, $t_i + T_i$ is unobserved and so the condition cannot be directly verified. On the other hand, choosing too low a duration $\tilde T_i$ throws away data, increasing variance.

In our empirical application in \Cref{sec:datapplication}, we leverage 311 \textit{agency response} data, detailing when each incident was inspected or worked on. We choose the minimum of this time and $\tilde t_i + \bar T$, where $\bar T$ is a maximum duration design choice; we validate our estimates with multiple choices of $\bar T$. Note that this choice is a stopping time (as opposed to the time of the last report, as discussed above).

Once we have the interval and the number of reports in it, we can leverage \Cref{thm:stoppingtimes} to convert our setting into a standard Poisson rate estimation task, for which a large literature exists (and, for example, calculate the MLE for an homogeneous $\lambda$ for each type $\theta$). However, that does not mean that the estimation is computationally or statistically tractable. In particular, up to now we have assumed a \textit{fixed} type $\theta$, and thus a fixed rate function $\lambda_\theta(\cdot)$. In our setting, $\theta$ is high-dimensional, but incidents of similar types may have similar rates. In the next sub-section, we present a tractable Bayesian Poisson regression approach -- with various specifications for $\lambda_\theta(\tau)$ -- that we will apply in our application.

\FloatBarrier




==> journal_subsections/journal_3_mlapproach.tex <==
\subsection{Bayesian Poisson Regression approach}
\label{sec:poissonreg}

Above, we show how to transform our setting into a standard Poisson rate estimation task. Here we assume that we have a dataset of incidents $i$ with types $\theta(i)$, where for each incident we observe an interval $(\tilde t_i, \tilde T_i]$ and the number of reports in that interval $\tilde M_i$.
%
We develop a Bayesian Poisson regression approach to estimate using our data. For each of our various model specifications, we describe `reasonable' data generating processes that would lead to such a specification.

Our choices are not exhaustive; other specifications may also be appropriate, preferable in various dimensions, or correspond to more realistic data generating processes; the empirical strategy developed in \Cref{sec:convertingtopoissonregression} allows a large Poisson rate estimation literature (spatial, time-dependent, feature-dependent, etc)  to be applied, off-the-shelf. Our approaches here are chosen for simplicity in model interpretation; however, as we discuss in \Cref{sec:datapplication}, the observed vs predicted data distributions suggest further improvements if the goal is predicting reporting rates.

First, we assume a dependence on how the reporting rate is affected by the type $\theta$. For each of these models, we have a base reporting rate $\lambda_\theta$, defined as:
\begin{equation}
\lambda_\theta = \exp\left(\alpha + \beta^T\theta\right), \label{eqn:lambdaregressionassumption}
\end{equation}
where $\beta$ is a coefficient vector of appropriate dimension, and $(\alpha, \beta)$ are coefficients to be estimated. All other rate parameters are shared across types $\theta$, providing statistical efficiency and easing analysis of how various type characteristics affect the reporting rate. %The covariates that compose $\theta$, as well as Bayesian priors, differ between model runs, and are discussed in \Cref{sec:simulation} and \Cref{sec:datapplication}.


\paragraph{Standard homogeneous Poisson regression} Our first specification is a standard homogeneous Poisson regression, where $\lambda_\theta(\tau) = \lambda_\theta$, for all $\tau$. Then, for each $i$, we have $\tilde M_i \sim \text{Poisson}\left(\tilde T_i\lambda_{\theta(i)} \right)$, where $\theta(i)$ is the type of incident $i$. This specification corresponds to the naive data generating process in which many residents independently encounter alive incidents and report them.

\paragraph{Zero-inflated Poisson regression} Next, we use a zero-inflated Poisson regression \cite{lambert1992zero}, in which $\lambda_\theta(\tau) = 0 $ with probability $\gamma$, and $\lambda_\theta$ otherwise, independently sampled for each incident.\footnote{While \Cref{thm:stoppingtimes} is proven for a deterministic rate $\lambda_\theta$ (conditioned on type $\theta$), it is easy to see that the analogous result extends for the Zero-inflated model, as long as the stopping times are independent of $\gamma$, given the sample path and type $\theta$. With a fixed $\gamma$ (or fixed given types $\theta$), this condition trivially holds.} Then, for each $i$, we have $\tilde M_i \sim \text{Bernoulli}(1 - \gamma)\times\text{Poisson}\left(\tilde T_i\lambda_{\theta(i)} \right)$.

Recall that, as discussed in \Cref{sec:convertingtopoissonregression}, $\tilde M_i$ is the number of reports \textit{after} the first report (up until the observation end time); thus, this specification corresponds to a data generating process in which for a fraction $\gamma$ of incidents, only one report is generated. For example, perhaps those incidents are personal requests for service (i.e., to plant a tree somewhere or to prune a tree to enable certain construction), for which duplicates are unlikely; alternatively, the Parks department may physically mark trees as ``report received; full inspection pending,'' preventing future reports.\footnote{A natural extension would be to also allow $\gamma$ to depend on $\theta$.} Such a model is typically used when one observes more zeros than would be expected from a Poisson distribution, as in our case.

\medskip As detailed in \Cref{sec:datapplication}, these two models reasonably match the observed distribution of the number of reports received in the observation period, except that the \textit{Basic} model under-estimates the number of incidents with zero reports $\tilde M_i = 0$, and the zero-inflated model over-estimates the number of incidents with large $\tilde M_i$. Such patterns suggest that a time non-homogeneous Poisson process (with decreasing rates with incident age) may be an appropriate extension. The estimation of such processes involve fitting a per-incident latent parameter that is the age of the incident when the first report occurred. Analogies of such processes have been considered in the marketing literature, e.g. \citep{abe_counting_2008}, and it is a strength of our analysis in \Cref{sec:convertingtopoissonregression} that such a connection is possible. We leave this as an extension due to the technical difficulties introduced by the need to estimate parameters whose number are on the magnitude of samples, and the scope of this paper.

% \paragraph{Non-homogeneous Poisson regression} Suppose the reporting rate is $\lambda_\theta(0)=\lambda_\theta$ at birth but changes with incident age. The challenge with non-homogeneous reporting rates with our data (beyond the standard statistical efficiency challenges to estimating such rates) is that our observation period does not start at incident age $\tau = 0$, but rather at the (unknown) age when the first report occurred, $\tau = \tilde t_i - t_i$. For example, suppose the reporting rate decreases exponentially with incident age: $\lambda_\theta(\tau) = \lambda_\theta\exp(-\gamma \tau)$, where $\gamma\ge 0$. Then, the Poisson likelihood in \Cref{eq:poissonnonhom} corresponds to
% \begin{align*}
% 	\tilde M_i&\sim \text{Poisson}\left(\frac{\lambda_\theta}{\gamma}e^{-(\tilde t_i - t_i)}\left[1 - e^{-\tilde T_i}\right]\right),
% \end{align*}
% where $(\tilde t_i - t_i)$ is a per-incident unknown latent variable; if just the number of reports $\tilde M_i$ is used as data, there are more unknown model parameters than data points. However, note that in 311 systems, the data also typically include time-stamps for each incident, using which we can calculate report inter-arrival times -- using these times would lead to more data points than parameters, but both would still be on the order of the number of incidents. Such latent variable Bayesian non-homogeneous Poisson processes are considered in the marketing literature with ``buy till you die'' models \cite{abe_counting_2008}, where an unknown parameter for whether a  customer has left the system must be estimated; it is possible that time-reversed versions of such models can be adapted to this setting -- it is a strength of our analysis in \Cref{sec:convertingtopoissonregression} that such a connection is possible.

In this work, we apply the \textbf{basic} and \textbf{zero-inflated} Poisson regression approaches to our data.



==> plots/basic_nocens2_dur100_repmedium_300300-1nocens2_latexsummary.tex <==
\begin{table}
\centering
\caption{Regression coefficients for Standard Poisson regression with incident-level covariates and Borough fixed effects for Max Duration 100 days, Default repeat caller removal.}
\begin{tabular}{lrrrrrr}
\toprule
                                &    Mean &  StdDev &     5\% &    50\% &    95\% &  R\_hat \\
\midrule
                          Intercept & -4.5700 &  0.0200 & -4.610 & -4.570 & -4.540 &    1.0 \\
               INSPCondtion[T.Dead] & -0.3300 &  0.0300 & -0.380 & -0.330 & -0.280 &    1.0 \\
     INSPCondtion[T.Excellent\_Good] & -0.4600 &  0.0230 & -0.500 & -0.460 & -0.420 &    1.0 \\
               INSPCondtion[T.Fair] & -0.3300 &  0.0230 & -0.360 & -0.330 & -0.290 &    1.0 \\
                INSP\_RiskAssessment &  0.2900 &  0.0098 &  0.270 &  0.290 &  0.310 &    1.0 \\
Log(Tree Diameter at Breast Height) & -0.0180 &  0.0079 & -0.031 & -0.018 & -0.005 &    1.0 \\
                     Borough[Bronx] &  0.0690 &  0.0220 &  0.030 &  0.070 &  0.100 &    1.0 \\
                  Borough[Brooklyn] & -0.1500 &  0.0160 & -0.170 & -0.150 & -0.120 &    1.0 \\
                 Borough[Manhattan] & -0.0160 &  0.0370 & -0.077 & -0.016 &  0.045 &    1.0 \\
                    Borough[Queens] & -0.1300 &  0.0170 & -0.160 & -0.130 & -0.100 &    1.0 \\
             Borough[Staten Island] &  0.2200 &  0.0270 &  0.180 &  0.220 &  0.270 &    1.0 \\
                   Category[Hazard] &  1.5000 &  0.0150 &  1.500 &  1.500 &  1.500 &    1.0 \\
      Category[Illegal Tree Damage] &  0.0170 &  0.0260 & -0.026 &  0.017 &  0.062 &    1.0 \\
                    Category[Prune] & -0.0790 &  0.0240 & -0.120 & -0.079 & -0.040 &    1.0 \\
              Category[Remove Tree] & -0.0018 &  0.0190 & -0.033 & -0.002 &  0.030 &    1.0 \\
      Category[Root/Sewer/Sidewalk] & -1.4000 &  0.0340 & -1.500 & -1.400 & -1.400 &    1.0 \\
\bottomrule
\end{tabular}
\end{table}


==> plots/basic_zeroinflated_bas_singlecens2_basic_zeroinflatedsinglecens2_dur100_repmedium_unicoefsequity.tex <==
%\begin{table}
%\centering
%\caption{Census Tract Demographic coefficients}
%\begin{tabular}{lrrrr}
%\toprule
%                      &   Mean &  StdDev &      5\% &     95\% \\
%\midrule
%           Median Age & -0.047 &  0.0083 & -0.0610 & -0.0340 \\
%    Fraction Hispanic &  0.035 &  0.0096 &  0.0190 &  0.0510 \\
%       Fraction white &  0.054 &  0.0091 &  0.0400 &  0.0680 \\
%       Fraction Black & -0.036 &  0.0089 & -0.0500 & -0.0210 \\
%    Fraction noHSGrad & -0.020 &  0.0088 & -0.0340 & -0.0054 \\
%Fraction college grad &  0.042 &  0.0088 &  0.0280 &  0.0570 \\
%     Fraction poverty & -0.018 &  0.0088 & -0.0320 & -0.0031 \\
%      Fraction renter &  0.054 &  0.0092 &  0.0390 &  0.0690 \\
% Fraction single unit & -0.064 &  0.0100 & -0.0820 & -0.0470 \\
%      Log(Avg income) &  0.018 &  0.0086 &  0.0037 &  0.0320 \\
%         Log(Density) &  0.100 &  0.0110 &  0.0850 &  0.1200 \\
%\bottomrule
%\end{tabular}
\begin{tabular}{lrr}
	\toprule
	&   Mean &  StdDev \\
	\midrule
	Median Age & -0.047 &  0.0083 \\
	Fraction Hispanic &  0.035 &  0.0096 \\
	Fraction white &  0.054 &  0.0091 \\
	Fraction Black & -0.036 &  0.0089 \\
	Fraction noHSGrad & -0.020 &  0.0088 \\
	Fraction college grad &  0.042 &  0.0088 \\
	Fraction in poverty & -0.018 &  0.0088 \\
	Fraction renter &  0.054 &  0.0092 \\
	Fraction single unit & -0.064 &  0.0100 \\
	Log(Avg income) &  0.018 &  0.0086 \\
	Log(Density) &  0.100 &  0.0110 \\
	\bottomrule
\end{tabular}
%\end{table}


==> plots/basic_zeroinflated_bas_singlecens2_basic_zeroinflatedsinglecens2_dur100_repmedium_unicoefsequity_full.tex <==
\begin{table}
\centering
\caption{Census Tract Demographic coefficients, estimated alone in a regression alongside the incident-specific covariates and the borough fixed effects. Full table corresponding to \Cref{tab:censuscoefficients}.}
\label{tab:coeffull}
\begin{tabular}{lrrrrr}
\toprule
                      &   Mean &  StdDev &      5\% &    50\% &     95\% \\
\midrule
           Median Age & -0.047 &  0.0083 & -0.0610 & -0.047 & -0.0340 \\
    Fraction Hispanic &  0.035 &  0.0096 &  0.0190 &  0.035 &  0.0510 \\
       Fraction white &  0.054 &  0.0091 &  0.0400 &  0.055 &  0.0680 \\
       Fraction Black & -0.036 &  0.0089 & -0.0500 & -0.036 & -0.0210 \\
    Fraction noHSGrad & -0.020 &  0.0088 & -0.0340 & -0.020 & -0.0054 \\
Fraction college grad &  0.042 &  0.0088 &  0.0280 &  0.042 &  0.0570 \\
     Fraction poverty & -0.018 &  0.0088 & -0.0320 & -0.018 & -0.0031 \\
      Fraction renter &  0.054 &  0.0092 &  0.0390 &  0.054 &  0.0690 \\
 Fraction single unit & -0.064 &  0.0100 & -0.0820 & -0.064 & -0.0470 \\
      Log(Avg income) &  0.018 &  0.0086 &  0.0037 &  0.018 &  0.0320 \\
         Log(Density) &  0.100 &  0.0110 &  0.0850 &  0.100 &  0.1200 \\
\bottomrule
\end{tabular}
\end{table}


==> plots/basic_zeroinflated_nocens2_dur100_repmedium_300300-1nocens2_latexsummary.tex <==
\begin{table}[t]
\caption{Regression coefficients for \textbf{zero-inflated Poisson regression} with our \textbf{Base} covariates: incident-level covariates and Borough fixed effects with a Max Duration of 100 days, and default repeat caller removal. $R\_hat$ is a Bayesian MCMC convergence diagnostic, where a value close to 1 indicates that multiple chains have mixed well.}
\label{tab:basicinfrefcoef}
\centering
\begin{tabular}{lrrrrrr}
\toprule
                                &   Mean &  StdDev &     5\% &    50\% &    95\% &  R\_hat \\
\midrule
                          Intercept & -3.230 &   0.030 & -3.270 & -3.230 & -3.180 &    1.0 \\
            Zero Inflation fraction &  0.660 &   0.000 &  0.650 &  0.660 &  0.660 &    1.0 \\
               INSPCondtion[T.Dead] & -0.350 &   0.037 & -0.410 & -0.350 & -0.290 &    1.0 \\
     INSPCondtion[T.Excellent\_Good] & -0.320 &   0.026 & -0.360 & -0.320 & -0.270 &    1.0 \\
               INSPCondtion[T.Fair] & -0.210 &   0.026 & -0.250 & -0.210 & -0.170 &    1.0 \\
                INSP\_RiskAssessment &  0.240 &   0.011 &  0.220 &  0.240 &  0.260 &    1.0 \\
Log(Tree Diameter at Breast Height) & -0.034 &   0.009 & -0.049 & -0.034 & -0.019 &    1.0 \\
                     Borough[Bronx] & -0.074 &   0.026 & -0.120 & -0.073 & -0.029 &    1.0 \\
                  Borough[Brooklyn] & -0.390 &   0.019 & -0.420 & -0.390 & -0.360 &    1.0 \\
                 Borough[Manhattan] &  0.500 &   0.048 &  0.430 &  0.500 &  0.580 &    1.0 \\
                    Borough[Queens] & -0.280 &   0.019 & -0.310 & -0.280 & -0.250 &    1.0 \\
             Borough[Staten Island] &  0.240 &   0.031 &  0.180 &  0.240 &  0.290 &    1.0 \\
                   Category[Hazard] &  1.500 &   0.017 &  1.400 &  1.500 &  1.500 &    1.0 \\
      Category[Illegal Tree Damage] &  0.210 &   0.034 &  0.150 &  0.200 &  0.260 &    1.0 \\
                    Category[Prune] & -0.081 &   0.027 & -0.130 & -0.081 & -0.035 &    1.0 \\
              Category[Remove Tree] &  0.054 &   0.024 &  0.013 &  0.054 &  0.092 &    1.0 \\
      Category[Root/Sewer/Sidewalk] & -1.600 &   0.036 & -1.700 & -1.600 & -1.600 &    1.0 \\
\bottomrule
\end{tabular}
\end{table}

==> plots/basic_zeroinflated_nocens2_dur100_repmostconservative_300300-1nocens2_latexsummary.tex <==
\begin{table}
\centering
\caption{Regression coefficients for Zero-inflated Poisson regression with incident-level covariates and Borough fixed effects for Max Duration 100 days, Remove all repeat callers and missing caller information.}
\begin{tabular}{lrrrrrr}
\toprule
                                &   Mean &  StdDev &      5\% &    50\% &    95\% &  R\_hat \\
\midrule
                          Intercept & -3.270 &  0.0300 & -3.3100 & -3.260 & -3.220 &   1.01 \\
            Zero Inflation fraction &  0.650 &  0.0000 &  0.6400 &  0.650 &  0.660 &   1.00 \\
               INSPCondtion[T.Dead] & -0.340 &  0.0350 & -0.4000 & -0.340 & -0.290 &   1.00 \\
     INSPCondtion[T.Excellent\_Good] & -0.350 &  0.0280 & -0.3900 & -0.350 & -0.300 &   1.00 \\
               INSPCondtion[T.Fair] & -0.220 &  0.0260 & -0.2600 & -0.220 & -0.180 &   1.00 \\
                INSP\_RiskAssessment &  0.230 &  0.0120 &  0.2100 &  0.230 &  0.250 &   1.00 \\
Log(Tree Diameter at Breast Height) & -0.025 &  0.0095 & -0.0410 & -0.025 & -0.010 &   1.00 \\
                     Borough[Bronx] & -0.084 &  0.0260 & -0.1300 & -0.084 & -0.042 &   1.00 \\
                  Borough[Brooklyn] & -0.390 &  0.0190 & -0.4200 & -0.390 & -0.360 &   1.00 \\
                 Borough[Manhattan] &  0.510 &  0.0480 &  0.4300 &  0.510 &  0.590 &   1.00 \\
                    Borough[Queens] & -0.270 &  0.0190 & -0.3000 & -0.270 & -0.240 &   1.00 \\
             Borough[Staten Island] &  0.230 &  0.0340 &  0.1800 &  0.230 &  0.290 &   1.00 \\
                   Category[Hazard] &  1.500 &  0.0180 &  1.4000 &  1.500 &  1.500 &   1.00 \\
      Category[Illegal Tree Damage] &  0.220 &  0.0330 &  0.1600 &  0.220 &  0.270 &   1.00 \\
                    Category[Prune] & -0.099 &  0.0290 & -0.1500 & -0.098 & -0.053 &   1.00 \\
              Category[Remove Tree] &  0.045 &  0.0230 &  0.0076 &  0.045 &  0.082 &   1.00 \\
      Category[Root/Sewer/Sidewalk] & -1.600 &  0.0400 & -1.7000 & -1.600 & -1.600 &   1.00 \\
\bottomrule
\end{tabular}
\end{table}


==> plots/basic_zeroinflated_nocens2_dur200_repmedium_300300-1nocens2_latexsummary.tex <==
\begin{table}
\centering
\caption{Regression coefficients for Zero-inflated Poisson regression with incident-level covariates and Borough fixed effects for Max Duration 200 days, Default repeat caller removal.}
\begin{tabular}{lrrrrrr}
\toprule
                                &   Mean &  StdDev &     5\% &    50\% &    95\% &  R\_hat \\
\midrule
                          Intercept & -3.500 &  0.0300 & -3.550 & -3.500 & -3.460 &    1.0 \\
            Zero Inflation fraction &  0.620 &  0.0000 &  0.620 &  0.620 &  0.630 &    1.0 \\
               INSPCondtion[T.Dead] & -0.470 &  0.0330 & -0.530 & -0.470 & -0.420 &    1.0 \\
     INSPCondtion[T.Excellent\_Good] & -0.250 &  0.0260 & -0.290 & -0.250 & -0.210 &    1.0 \\
               INSPCondtion[T.Fair] & -0.160 &  0.0250 & -0.200 & -0.160 & -0.120 &    1.0 \\
                INSP\_RiskAssessment &  0.240 &  0.0110 &  0.220 &  0.240 &  0.250 &    1.0 \\
Log(Tree Diameter at Breast Height) & -0.040 &  0.0086 & -0.054 & -0.040 & -0.027 &    1.0 \\
                     Borough[Bronx] & -0.160 &  0.0250 & -0.200 & -0.160 & -0.120 &    1.0 \\
                  Borough[Brooklyn] & -0.400 &  0.0180 & -0.430 & -0.400 & -0.370 &    1.0 \\
                 Borough[Manhattan] &  0.580 &  0.0460 &  0.500 &  0.580 &  0.660 &    1.0 \\
                    Borough[Queens] & -0.270 &  0.0180 & -0.300 & -0.270 & -0.240 &    1.0 \\
             Borough[Staten Island] &  0.240 &  0.0320 &  0.190 &  0.240 &  0.300 &    1.0 \\
                   Category[Hazard] &  1.500 &  0.0160 &  1.500 &  1.500 &  1.600 &    1.0 \\
      Category[Illegal Tree Damage] &  0.140 &  0.0320 &  0.093 &  0.140 &  0.190 &    1.0 \\
                    Category[Prune] & -0.055 &  0.0260 & -0.099 & -0.056 & -0.011 &    1.0 \\
              Category[Remove Tree] &  0.110 &  0.0210 &  0.072 &  0.110 &  0.140 &    1.0 \\
      Category[Root/Sewer/Sidewalk] & -1.700 &  0.0350 & -1.800 & -1.700 & -1.700 &    1.0 \\
\bottomrule
\end{tabular}
\end{table}


==> plots/basic_zeroinflated_nocens2_dur30_repmedium_300300-1nocens2_latexsummary.tex <==
\begin{table}
\centering
\caption{Regression coefficients for Zero-inflated Poisson regression with incident-level covariates and Borough fixed effects for Max Duration 30 days, Default repeat caller removal.}
\begin{tabular}{lrrrrrr}
\toprule
                                &    Mean &  StdDev &     5\% &     50\% &     95\% &  R\_hat \\
\midrule
                          Intercept & -2.6700 &  0.0300 & -2.710 & -2.6700 & -2.6200 &    1.0 \\
            Zero Inflation fraction &  0.7300 &  0.0000 &  0.720 &  0.7300 &  0.7300 &    1.0 \\
               INSPCondtion[T.Dead] & -0.2400 &  0.0390 & -0.300 & -0.2300 & -0.1700 &    1.0 \\
     INSPCondtion[T.Excellent\_Good] & -0.3900 &  0.0270 & -0.430 & -0.3900 & -0.3400 &    1.0 \\
               INSPCondtion[T.Fair] & -0.2100 &  0.0260 & -0.250 & -0.2100 & -0.1600 &    1.0 \\
                INSP\_RiskAssessment &  0.2000 &  0.0110 &  0.190 &  0.2100 &  0.2200 &    1.0 \\
Log(Tree Diameter at Breast Height) & -0.0058 &  0.0096 & -0.022 & -0.0056 &  0.0097 &    1.0 \\
                     Borough[Bronx] & -0.0670 &  0.0260 & -0.110 & -0.0670 & -0.0240 &    1.0 \\
                  Borough[Brooklyn] & -0.2100 &  0.0200 & -0.250 & -0.2100 & -0.1800 &    1.0 \\
                 Borough[Manhattan] &  0.3600 &  0.0490 &  0.280 &  0.3600 &  0.4500 &    1.0 \\
                    Borough[Queens] & -0.2700 &  0.0200 & -0.300 & -0.2700 & -0.2300 &    1.0 \\
             Borough[Staten Island] &  0.1800 &  0.0320 &  0.130 &  0.1800 &  0.2400 &    1.0 \\
                   Category[Hazard] &  1.4000 &  0.0200 &  1.300 &  1.4000 &  1.4000 &    1.0 \\
      Category[Illegal Tree Damage] &  0.2500 &  0.0350 &  0.190 &  0.2500 &  0.3000 &    1.0 \\
                    Category[Prune] & -0.1200 &  0.0320 & -0.170 & -0.1200 & -0.0670 &    1.0 \\
              Category[Remove Tree] & -0.0290 &  0.0260 & -0.072 & -0.0290 &  0.0140 &    1.0 \\
      Category[Root/Sewer/Sidewalk] & -1.5000 &  0.0380 & -1.500 & -1.5000 & -1.4000 &    1.0 \\
\bottomrule
\end{tabular}
\end{table}


==> plots/basic_zeroinflated_timein_nocens2_dur100_repmedium_300300-1nocens2_latexsummary.tex <==
\begin{table}
\centering
\caption{Regression coefficients for zero-inflated time-inhomogeneous model with incident-level covariates and Borough fixed effects.}
\begin{tabular}{lrrrrrr}
\toprule
                               name &    Mean &  StdDev &     5\% &     50\% &    95\% &  R\_hat \\
\midrule
                          Intercept & -0.4700 &  0.0300 & -0.520 & -0.4800 & -0.420 &    1.0 \\
            Zero Inflation fraction &  0.7800 &  0.0000 &  0.770 &  0.7800 &  0.780 &    1.0 \\
               INSPCondtion[T.Dead] & -0.1100 &  0.0380 & -0.170 & -0.1100 & -0.049 &    1.0 \\
     INSPCondtion[T.Excellent\_Good] & -0.3200 &  0.0290 & -0.360 & -0.3100 & -0.270 &    1.0 \\
               INSPCondtion[T.Fair] & -0.1400 &  0.0270 & -0.180 & -0.1400 & -0.093 &    1.0 \\
                INSP\_RiskAssessment &  0.1400 &  0.0110 &  0.120 &  0.1400 &  0.160 &    1.0 \\
Log(Tree Diameter at Breast Height) &  0.0029 &  0.0095 & -0.013 &  0.0029 &  0.018 &    1.0 \\
                      beta\_duration &  0.1000 &  0.0100 &  0.090 &  0.1000 &  0.110 &    1.0 \\
                     Borough[Bronx] &  0.1300 &  0.0270 &  0.087 &  0.1300 &  0.180 &    1.0 \\
                  Borough[Brooklyn] &  0.3300 &  0.0200 &  0.290 &  0.3300 &  0.360 &    1.0 \\
                 Borough[Manhattan] & -0.3400 &  0.0480 & -0.420 & -0.3400 & -0.260 &    1.0 \\
                    Borough[Queens] &  0.0056 &  0.0190 & -0.026 &  0.0063 &  0.036 &    1.0 \\
             Borough[Staten Island] & -0.1200 &  0.0330 & -0.180 & -0.1200 & -0.067 &    1.0 \\
                   Category[Hazard] &  0.7300 &  0.0190 &  0.700 &  0.7300 &  0.760 &    1.0 \\
      Category[Illegal Tree Damage] &  0.3700 &  0.0350 &  0.310 &  0.3700 &  0.420 &    1.0 \\
                    Category[Prune] & -0.0096 &  0.0280 & -0.056 & -0.0092 &  0.036 &    1.0 \\
              Category[Remove Tree] & -0.0680 &  0.0230 & -0.110 & -0.0670 & -0.030 &    1.0 \\
      Category[Root/Sewer/Sidewalk] & -1.0000 &  0.0350 & -1.100 & -1.0000 & -0.960 &    1.0 \\
\bottomrule
\end{tabular}
\end{table}


==> plots/chicago_basic.tex <==
\begin{table}
\centering
\caption{Regression coefficients for Base variables in Chicago, for Max Duration 100 days} 
\label{tab:chicagobasic}
\begin{tabular}{lrrr}
\toprule
{} &      Mean &    StdDev &  R\_hat \\
\midrule
Intercept                                          & -4.053200 &  0.060970 &    1.0 \\
Zero Inflation fraction                            &  0.539120 &  0.003080 &    1.0 \\
Category[Sewer Cave-In Inspection Request]         & -1.644740 &  0.094402 &    1.0 \\
Category[Water On Street Complaint]                &  0.523323 &  0.077660 &    1.0 \\
Category[Water in Basement Complaint]              &  0.627274 &  0.115326 &    1.0 \\
Category[Alley Sewer Inspection Request]           & -0.907884 &  0.126657 &    1.0 \\
Category[Sewer Cleaning Inspection Request]        & -1.018360 &  0.074177 &    1.0 \\
Category[Pavement Cave-In Inspection Request]      & -2.996230 &  1.121890 &    1.0 \\
Category[Protected Bike Lane - Debris Removal]     & -0.307539 &  0.285097 &    1.0 \\
Category[Sidewalk Inspection Request]              & -2.246020 &  0.105649 &    1.0 \\
Category[Sign Repair Request - Stop Sign]          &  2.764160 &  0.110638 &    1.0 \\
Category[Sign Repair Request - One Way Sign]       &  2.147160 &  0.211825 &    1.0 \\
Category[Sign Repair Request - Do Not Enter Sign]  &  1.080180 &  0.473904 &    1.0 \\
Category[Sign Repair Request - All Other Signs]    & -1.412860 &  0.076753 &    1.0 \\
Category[Bicycle Request/Complaint]                & -0.877855 &  0.184213 &    1.0 \\
Category[Alley Pothole Complaint]                  &  0.265150 &  0.067260 &    1.0 \\
Category[Pothole in Street Complaint]              &  0.831174 &  0.061610 &    1.0 \\
Category[Alley Light Out Complaint]                &  0.383289 &  0.063814 &    1.0 \\
Category[Traffic Signal Out Complaint]             &  2.569320 &  0.064007 &    1.0 \\
Category[Viaduct Light Out Complaint]              & -0.491269 &  0.162562 &    1.0 \\
Category[Street Light Out Complaint]               &  1.766720 &  0.061264 &    1.0 \\
Category[Street Light Pole Damage Complaint]       &  0.680213 &  0.116861 &    1.0 \\
Category[Street Light On During Day Complaint]     & -0.266965 &  0.106103 &    1.0 \\
Category[Street Light Pole Door Missing Complaint] & -2.498780 &  0.279745 &    1.0 \\
Category[Snow Removal - Protected Bike Lane or ... & -2.456730 &  0.813064 &    1.0 \\
Category[Snow – Uncleared Sidewalk Complaint]      &  0.286266 &  0.085892 &    1.0 \\
Category[No Water Complaint]                       &  2.432550 &  0.123870 &    1.0 \\
Category[Low Water Pressure Complaint]             & -0.961297 &  0.167591 &    1.0 \\
Category[Open Fire Hydrant Complaint]              &  4.221190 &  0.064634 &    1.0 \\
Category[Water Quality Concern]                    & -2.491440 &  0.397393 &    1.0 \\
\bottomrule
\end{tabular}
\end{table}


==> plots/chicago_demoplot_full.tex <==
\begin{table}
\centering
\caption{Census Tract Demographic coefficients in Chicago}
\label{tab:censuscoefficientschicago}
\begin{tabular}{lrrrrr}
\toprule
                      &      Mean &   StdDev &        5\% &       50\% &       95\% \\
\midrule
           Median Age & -0.001472 & 0.005340 & -0.010386 & -0.001397 &  0.006768 \\
    Fraction Hispanic &  0.055305 & 0.005633 &  0.046080 &  0.055368 &  0.065481 \\
       Fraction white & -0.035253 & 0.005519 & -0.043432 & -0.035479 & -0.026216 \\
       Fraction Black & -0.016526 & 0.005145 & -0.025283 & -0.016330 & -0.008997 \\
    Fraction noHSGrad &  0.054937 & 0.005666 &  0.045920 &  0.055098 &  0.063757 \\
Fraction college grad & -0.045110 & 0.005809 & -0.054237 & -0.045116 & -0.035509 \\
     Fraction poverty & -0.036907 & 0.005298 & -0.045327 & -0.037093 & -0.028027 \\
      Fraction renter &  0.010492 & 0.005708 &  0.001130 &  0.010662 &  0.019221 \\
 Fraction single unit &  0.011311 & 0.005318 &  0.003216 &  0.011211 &  0.019854 \\
      Log(Avg income) & -0.026773 & 0.005089 & -0.035165 & -0.026797 & -0.017888 \\
         Log(Density) &  0.012235 & 0.005770 &  0.002951 &  0.012161 &  0.021718 \\
\bottomrule
\end{tabular}
\end{table}


==> plots/tab_ratescontext.tex <==
\begin{table}[tb]
	\caption{Average reporting delay $\frac{1}{\lambda_\theta}$ for incidents of different types $\theta$ as implied by \Cref{tab:basicinfrefcoef}.}
	\label{tab:contextualizingrates}
		\centering
	\begin{tabular}{lcc}
		\toprule
		{Incident characteristics}              & {Manhattan} & {Queens} \\ \midrule
		Hazard, tree in Poor condition,   High risk         & 2.5 days           & 4.7 days        \\
		Illegal Tree Damage, tree in Poor condition                         & 15 days            & 28 days         \\
		Root/Sewer/Sidewalk issue, tree in Fair condition & 112 days           & 209 days\\
		\bottomrule
	\end{tabular}
\end{table}

==> plots/tab_summary_stats_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[tb]
\caption{Summary statistics: service requests and inspections statistics are directly from the DPR reports data; unique incidents statistics are derived from the inspected service requests, where the average duration is calculated using the stopping times definition. The \textit{Others} category includes four other categories: Rescue/Preservation, Remove Stump, Pest/Disease, Planting Space, that together account for less than 0.5\% of the service requests; we exclude them in our further analysis due to lack of data.}
\label{tab:Summary}
\centering
\resizebox{.9\textwidth}{!}{%
\begin{tabular}{r|r|rr|rrr}
\multicolumn{1}{c|}{\textbf{}}             & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Service \\ requests\end{tabular}}} & \multicolumn{2}{c|}{\textbf{Inspections}}                                                                                                                          & \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Incidents\\ (derived from inspected)\end{tabular}}}                                                                                                                                             \\
\multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{}                                                                     & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Inspected \\ SRs\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Percentage\\ inspected\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Unique\\ incidents\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Avg. \\ \# reports\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Avg. duration \\ (days)\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\textbf{Total number}} & 223417                                                                                    & 116493                                                                       & 0.52                                                                                & 98971                                                                          & 1.18                                                                           & 20.39                                                                               \\
\multicolumn{1}{l|}{\textbf{By Borough}}   &                                                                                           &                                                                              &                                                                                     &                                                                                &                                                                                &                                                                                     \\
\textit{Queens}                            & 90930                                                                                     & 49458                                                                        & 0.54                                                                                & 43082                                                                          & 1.15                                                                           & 18.22                                                                               \\
\textit{Brooklyn}                          & 67852                                                                                     & 35875                                                                        & 0.53                                                                                & 28268                                                                          & 1.27                                                                           & 27.29                                                                               \\
\textit{Staten Island}                     & 27263                                                                                     & 11204                                                                        & 0.41                                                                                & 10064                                                                          & 1.11                                                                           & 15.49                                                                               \\
\textit{Bronx}                             & 22629                                                                                     & 13360                                                                        & 0.59                                                                                & 11409                                                                          & 1.17                                                                           & 20.27                                                                               \\
\textit{Manhattan}                         & 14702                                                                                     & 6595                                                                         & 0.45                                                                                & 6147                                                                           & 1.07                                                                           & 12.10                                                                               \\
\multicolumn{1}{l|}{\textbf{By Category}}  &                                                                                           &                                                                              &                                                                                     &                                                                                &                                                                                &                                                                                     \\
\textit{Hazard}                                     & 87864                                                                                     & 52035                                                                        & 0.59                                                                                & 40922                                                                          & 1.27                                                                           & 10.65                                                                               \\
\textit{Prune}                             & 48649                                                                                     & 14261                                                                        & 0.29                                                                                & 12637                                                                          & 1.13                                                                           & 23.51                                                                               \\
\textit{Remove Tree}                       & 44177                                                                                     & 27647                                                                        & 0.63                                                                                & 24520                                                                          & 1.13                                                                           & 20.31                                                                               \\
\textit{Root/Sewer/Sidewalk}               & 30856                                                                                     & 15902                                                                        & 0.52                                                                                & 15222                                                                          & 1.04                                                                           & 37.48                                                                               \\
\textit{Illegal Tree Damage}               & 11061                                                                                     & 6648                                                                         & 0.60                                                                                & 5670                                                                           & 1.17                                                                           & 38.23                                                                               \\
\textit{Others}                            & 809                                                                                       & -                                                                            & -                                                                                   & -                                                                              & -                                                                              & -
\end{tabular}%
}

\end{table}

==> plots/table_example.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[tb]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lrrrrr}
    \toprule
    \multicolumn{1}{c}{} &
      \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Ground truth \\ conditions\end{tabular}}} &
      \multicolumn{2}{c}{\textbf{Reporting behavior}} &
      \multicolumn{2}{c}{\textbf{Observed data}} \\ \midrule
    \multicolumn{1}{c}{Neighborhood} &
      \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Number \\ of incidents\end{tabular}} &
      \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Percentage that\\  gets reported\end{tabular}} &
      \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# reports for each \\ reported incidents\end{tabular}} &
      \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Total \\ observed reports\end{tabular}} &
      \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Total \\ observed incidents\end{tabular}} \\ \midrule
    A &
      10 &
      100\% &
      2 &
      20 &
      10 \\
    B &
      20 &
      50\% &
      1 &
      10 &
      10 \\
    C &
      5 &
      80\% &
      5 &
      20 &
      4 \\ \bottomrule
    \end{tabular}%
    }
    \caption{In this toy example, the three neighborhoods have totally different reporting patterns. However, by only analyzing the observed reports, neighborhoods A and B are indistinguishable; and by only analyzing the observed incidents, neighborhoods A and C are indistinguishable. \todo{add more to caption}}
    \label{tab:egunidenti}
    \end{table}
    
    % \begin{table}[tb]
    % \centering
    % \resizebox{\textwidth}{!}{%
    % \begin{tabular}{lrrrrr}
    % \toprule
    % \multicolumn{1}{c}{} &
    %   \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Ground truth \\ conditions\end{tabular}}} &
    %   \multicolumn{1}{c}{\textbf{Reporting behavior}} &
    %   \multicolumn{1}{c}{\textbf{Observed data}} \\ \midrule
    % \multicolumn{1}{c}{Neighborhood} &
    % %   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Number \\ of incidents \\ per day\end{tabular}} &
    % %   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Percentage of incidents \\ ever reported\end{tabular}} &
    % %   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# reports for each \\ reported incidents\end{tabular}} &
    % %   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Total \\ observed reports\end{tabular}} &
    % %   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Total \\ observed incidents\end{tabular}} \\ \midrule
    %   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Number \\ of incidents \\ per day\end{tabular}} &
    %   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Report probability \\ (fraction of incidents reported \\ per day)\end{tabular}} &
    % %   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# reports for each \\ reported incidents\end{tabular}} &
    %   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Total \\ observed incidents \\ per day\end{tabular}} \\ \midrule
    % %   \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Total \\ observed incidents\end{tabular}} \\ \midrule
    % A &
    %   10 &
    %   1 &
    % %   2 &
    % %   20 &
    %   10 \\
    % B &
    %   20 &
    %   0.5 & %50\% &
    % %   1 &
    % %   10 &
    %   10 \\
    % % A &
    % %   10 &
    % %   100\% &
    % %   2 &
    % %   20 &
    % %   10 \\
    % % B &
    % %   20 &
    % %   50\% &
    % %   1 &
    % %   10 &
    % %   10 \\
    % % C &
    % %   5 &
    % %   80\% &
    % %   5 &
    % %   20 &
    % %   4 \\
    %   \bottomrule
    % \end{tabular}%
    % }
    % \caption{In this toy example, the three neighborhoods have totally different reporting patterns. However, by only analyzing the observed reports, neighborhoods A and B are indistinguishable; and by only analyzing the observed incidents, neighborhoods A and C are indistinguishable.}
    % \label{tab:egunidenti}
    % \end{table}

==> plots/tract_hierarchy_zeroinflated_hiertract11medpriornocens2_dur100_repmedium_300300-1nocens2_latexsummary.tex <==
\begin{table}[tbh]
\centering
\caption{Regression coefficients for Zero-inflated Poisson regression with Spatial Hierarchy with incident-level covariates and Borough fixed effects for Max Duration 100 days, Default repeat caller removal. }
\begin{tabular}{lrrrrrr}
\toprule
                                &   Mean &  StdDev &      5\% &    50\% &     95\% &  R\_hat \\
\midrule
                          Intercept & -3.180 &  0.0400 & -3.2500 & -3.180 & -3.1100 &   1.01 \\
            Zero Inflation fraction &  0.660 &  0.0000 &  0.6500 &  0.660 &  0.6700 &   1.00 \\
               INSPCondtion[T.Dead] & -0.380 &  0.0330 & -0.4300 & -0.380 & -0.3200 &   1.00 \\
     INSPCondtion[T.Excellent\_Good] & -0.370 &  0.0280 & -0.4100 & -0.370 & -0.3200 &   1.00 \\
               INSPCondtion[T.Fair] & -0.220 &  0.0260 & -0.2700 & -0.220 & -0.1800 &   1.00 \\
                INSP\_RiskAssessment &  0.230 &  0.0120 &  0.2100 &  0.240 &  0.2500 &   1.00 \\
Log(Tree Diameter at Breast Height) & -0.024 &  0.0093 & -0.0390 & -0.024 & -0.0086 &   1.00 \\
                     Borough[Bronx] & -0.043 &  0.0650 & -0.1500 & -0.044 &  0.0660 &   1.00 \\
                  Borough[Brooklyn] & -0.440 &  0.0520 & -0.5200 & -0.440 & -0.3500 &   1.00 \\
                 Borough[Manhattan] &  0.490 &  0.0780 &  0.3600 &  0.490 &  0.6200 &   1.00 \\
                    Borough[Queens] & -0.240 &  0.0580 & -0.3400 & -0.240 & -0.1500 &   1.00 \\
             Borough[Staten Island] &  0.230 &  0.1000 &  0.0550 &  0.230 &  0.3900 &   1.00 \\
                   Category[Hazard] &  1.500 &  0.0170 &  1.5000 &  1.500 &  1.5000 &   1.00 \\
      Category[Illegal Tree Damage] &  0.180 &  0.0360 &  0.1200 &  0.180 &  0.2400 &   1.00 \\
                    Category[Prune] & -0.085 &  0.0300 & -0.1400 & -0.084 & -0.0380 &   1.00 \\
              Category[Remove Tree] &  0.042 &  0.0240 &  0.0033 &  0.042 &  0.0800 &   1.00 \\
      Category[Root/Sewer/Sidewalk] & -1.600 &  0.0380 & -1.7000 & -1.600 & -1.6000 &   1.00 \\
\bottomrule
\end{tabular}
\end{table}


==> subsections/1_intro.tex <==
% \begin{itemize}
%     \item Background on crowd-sourced data: briefly explain why they are valuable, their usage, the operational insights (depending on which audience we want to appeal to)
%     \item Background on the problem facing data crowdsourcing: inequity stemming from technological literacy, cultural differences, and other factors
%     \item Background on the difficulty of identifying the inequity problems and counter its effect: this could relate to other kinds of systems where inequity arises. we should explain why identifying the real problem is hard:
%     \item We choose under-reporting to measure inequity: Explain why we choose under-reporting, and not mis-reporting.
%     \item We used a method inspired by missing species problem: operationally, we need to identify all the incidents; reports have duplicates, etc
%     \item We found that the reporting rate, conditional on an incident happening, relies on certain factors:
% \end{itemize}

\vspace{.2cm}
\begin{quote}
	If a tree falls in a forest, and no one reports it... does the city know about it?
\end{quote}
\vspace{.2cm}
%
%
%	1. 311 systems are large and important, they determine allocation of city resources
%
%
Cities are complex socio-technical systems comprised of physical and human infrastructure, navigated by millions of people daily. A core part of monitoring such systems is crowdsourcing (or ``co-production'' \cite{yuan_co-production_2019,brabham_crowdsourcing_2015}), in which people report problems that they encounter; the New York City 311 system, for example, received \num{2592831} reports in 2020, and more than one hundred North American cities employ similar systems. Such reports are necessary, as they provide a real-time reflection on on-the-ground conditions that the city cannot hope to otherwise be aware of \citep{schwester2009examination, hacker_spatiotemporal_2020,minkoff_nyc_2016, lee_crowdsourcing_2021-1}. These reports are used alongside internal data collection and automated sensor technology to make both immediate decisions---such as which dangerous, downed trees to inspect and fix---and longer-term planning decisions, such as which streets to resurface. For example, the NYC Department of Parks and Recreation sends a forester to inspect about $\frac23$ of reports, and the incidents deemed risky (about $\frac12$ of inspected incidents) are resolved by a maintenance crew.

%2. However, if not used equitably, that's a problem. There is a large literature trying to measure this

While such reporting systems have gained popularity in the last few decades, there are many unresolved challenges in using reports efficiently and equitably. In particular, one long-standing concern is whether residents\footnote{We use the term ``residents'' to denote anyone who might report an issue to the 311 system, including visitors.} equitably use the system; or whether, conditional on experiencing the same issues, some residents are more likely to log a report and request government services \citep{thijssen2016you} -- for example, if socio-economically privileged neighborhoods submit more incident reports. If such reporting behavior is heterogeneous, then government services that rely on such reporting will also be inequitable. Though it is commonly believed that reporting behavior is heterogeneous, previous studies vary greatly in the quantification of such bias and how to attribute it to socio-economic or geographic characteristics
\citep{kontokosta_bias_2021,kontokosta_equity_2017,minkoff_nyc_2016,hacker_spatiotemporal_2020, clark_coproduction_2013,wu2020determinants, o2016311, thijssen2016you, vedlitz1980citizen,mclafferty_placing_2020, xu_closing_2020}.





% Reports do not uniformly reflect the underlying rate of problems, such as if . First-come-first-serve processing then both misses some hazardous events and inequitably serves various communities, reinforcing historical disparities. The objective of the proposed research agenda is to develop algorithmic approaches to address such shortcomings – to develop Bayesian techniques to measure current shortcomings, to derive decision-making algorithms that more effectively make use of crowdsourced and other data, and to deploy simple, near-optimal processes to optimally allocate resources.

%These reports are triaged to the appropriate city agency, which then makes decisions regarding which reports to further inspect. This data is used alongside internal city agency data collection and automated sensor technology to make longer-term planning decisions.


%However, resident reported data may not be an objective and precise representation of reality. The bias in resident reports stems from multiple sources. For a start, problems tend to arise in neighborhoods with poorer conditions; even conditional on the existence of a problem, residents may have different responses . This drawback rather overshadows the benefits, leading questions of equity to the outcomes of using resident reports for data-driven decision making, especially when limited resources have to be allocated \citep{clark_coproduction_2013, kontokosta_equity_2017, , mclafferty_placing_2020, xu_closing_2020}.

%The benefit of using resident reports is that they , such as potholes, heat and water outages, and bug infestations .

%In modern smart cities, decision-making in governance and operations increasingly rely on data-driven approaches, with a significant amount of data gathered through citizen-sourcing, or crowd sourcing from city residents . Such systems are commonly referred to as coproduction systems, and among them is the 311 system used in . The 311 system enable local governments to engage citizens as “detectors” or “reporters” of the problems facing the city, and then use these reports to inform city governments in their effort to resolve the issues .



%3. The issues with the current approach is either they can't identify, or they need ground truth to do so. This .

The central methodological challenge is the same reason that cities must rely on this information: ground truth conditions are unknown. This induces a missing data challenge: researchers do not observe what incidents occurred, or when they occurred. Thus, it is difficult to determine whether one neighborhood is \textit{under-reporting} issues compared to other neighborhoods, or whether they truly experience fewer issues (due to, e.g., differences in infrastructure). Previous work either does not attempt to distinguish between these cases (implicitly assuming that incident rates are similar across areas), or employs external data to construct \textit{proxies} for ground truth incident rates (such as population, length of roadways, number of apartments, or incident rates detected by the occasional active/random inspections). While accurate proxies can distinguish between incident rates and reporting rates, they may be difficult to construct or may not be precise enough to distinguish between types of incidents (e.g., whether reporting behavior differs by incident risk).

%4. Methodological
%a. We propose a way to measure this. Motivated by missing species, but additional issues. Turn it into poisson regression, etc.

\parbold{A method to identify reporting rates without ground truth data.} In this work, we propose a method to identify (heterogeneous) reporting rates, using \textit{just} the reporting data itself, without relying on external ground truth data. Our insight is that we can use information on \textit{duplicate} reports about the same incident (which cities commonly log), to identify reporting rates \textit{conditional on an incident having occurred}. This insight originates from the \textit{missing species} estimation literature, where the number of \textit{duplicate} observations provides evidence regarding the existence of unseen species \citep{orlitsky_optimal_2016, wu_chebyshev_2016, han2021competitive, charikar2019efficient}; if for every observed unique species, we have observed it many times, then it is unlikely that there are similar species that have never been observed.

Our setting differs from the classic \textit{missing species} formulation, in that the set of incidents is not static: new incidents occur (e.g., a tree falls down), and are resolved (the city fixes the issue, or it naturally disappears). And, even for observed incidents (those that are reported), we do not know \textit{when} they occurred, or \textit{how long} the incident existed. Thus, naively, we do not know, e.g., whether the incident was reported twice over a possible three month or one week period. This difference matters, as the possible reporting period varies substantially with incident characteristics and reporting behavior (e.g., hazardous incidents are reported and addressed more quickly).

We show how to nevertheless convert the task to a standard \textit{Poisson rate estimation} challenge, for which a large empirical and theoretical literature exists. In particular, one can use the number of reports between time of the first report (but not including it) and an estimated death time (that may depend on the data, e.g., time of the reports or when the incident was inspected), to recover a {Poisson} likelihood with a corresponding rate function. The method is valid if the estimated death time is an \textit{under-}estimate of the resolution time and is a \textit{stopping time} (does not depend on the future).

Then, we can leverage standard Poisson rate estimation methods (for example, estimate the MLE or a Poisson regression) to recover the (heterogeneous) rates that incidents of different types and in various neighborhoods are reported, conditional on the incident having occurred.

%5. Application oriented
%a. We apply it to Parks data, using data provided to us…

\parbold{Applying our method to understand equity in 311 usage.} We apply our method to over \num{100000} resident reports made to the forestry unit in the New York City Department of Parks and Recreation (DPR), using both publicly accessible data and internal logs on incident inspection outcomes and work orders, provided to us by DPR.
%
Using a Bayesian Poisson regression framework, we estimate how the reporting rate varies as a function of incident characteristics (e.g., the risk rating assigned by a forester upon inspection), space (location within New York City), and socio-economic characteristics of the neighborhood in which the incident occurred.

We illustrate that our method is indeed precise enough to find differences in reporting rates; for example, we find that reports for riskier incidents and trees in more critical condition are submitted at substantially higher rates, conditional on the incident having occurred.
%
Finally, we study spatial and socio-economic heterogeneity. We find that there are substantial inter-location reporting differences; for example, comparing census tract level fixed effects, we find that reports occur at a three times higher rate in downtown Manhattan than in uptown Manhattan, even after controlling for the incident-level characteristics. We further find that factors like race/ethnicity and education levels are  associated with reporting rates, though such socio-economic characteristics cannot explain much of the spatial heterogeneity. These findings suggest that the allocation of government services, if reliant on incident reporting, may neither be efficient nor equitable.

%works in high dimension, use bayesian poisson regression approaches

\smallskip

We believe that our method is a general, powerful approach to understanding reporting behavior in resident crowdsourcing systems, delivering precise reporting estimates without requiring ground truth data---only duplicate report data, that are already collected by city agencies. The rest of this paper is organized as follows. The remainder of this section contains related work. In \Cref{sec:model}, we formalize our model and research questions. In \Cref{sec:3}, we develop and analyze our method. In \Cref{sec:datapplication}, we apply our findings to data from the New York Department of Parks and Recreation. We conclude in \Cref{sec:conclusion}.

%In this work, we propose a simple yet powerful technique in measuring bias in resident crowdsourcing systems, and we apply it to a real data set to show its power in practice. Our contributions can be summarized into two aspects.

%We provide a new perspective on the problem of identifying inequities in resident contacting government, by defining the metric of under-reporting as the rate at which residents make reports to an incident, conditional on it has happened. This metric reflects on people's perception of residents' willingness to make contacts, and can better distinguishes different existing conditions in various areas than directly measuring the number of reports. We show that using information in the \textit{duplicate} data is crucial to achieving the estimation of this reporting rate, which has not been seen in the literature.



%In order to estimate this rate, we formalize a stylized data-generating model, by drawing insights from the \textit{missing species} literature. We overcome two difficulties in this process: not all incidents are observed, and incidents are `dying', i.e. getting resolved with time. We get around these two difficulties by only starting to observe an incident once a report is made, by which point we know this incident exists, and terminate the incident at a designed stopping time. Under a Poisson process assumption akin to standard missing species literature \citep{goodtoulmin}, we first proposed a simple empirical estimation approach based solely on the maximum likelihood estimator.



%Given the high-dimensional nature of the characteristics of the reports, and that our end goal is to study the relationship between reporting behavior and various covariates of the incidents, we turn to more sophisticated machine learning approaches. The Poisson assumption helps us transform the estimation problem into a Poisson regression model, where it provides good generalization ability to other settings where the assumption also holds, and show potential for more elaborately designed machine learning techniques.


%\textbf{An application to DPR dataset and potential generalization.} We apply our methods  Via a hierarchical spatial zero-inflated Poisson regression model, we obtain estimates for the influence of spatial variables and incident-specific variables on the reporting rate, as well as an estimate for the reporting rate itself. We find that reporting behavior substantially and statistically significantly varies across different boroughs and different categories of the incident. A closer look into the linkage of socio-economic clustering and spatial heterogeneity of reporting rate reveals that there are substantial associations between reporting rate and socio-economic characteristics,

%
%\todo{edit below this}

%raising inequity concerns in using these reports for data-driven decision making in operation. Though our dataset is highly specialized, our method and model can extend to more general settings where there are duplicate reports by resident, which is prominent in many agencies in practice. This wide applicability amplifies the power of our approach.


%b. Can be used in other settings, is general, etc

%The benefit of our metric is that it circumvents problems in data collection as it does not require accurate ground-truth information for the estimation methods to work. It also has operational insights as this rate helps determine the time an incident occurred, which could become a useful piece of information when scheduling inspections.



%\todo{say more here why that's not guaranteed, and how ours is more precise. We should think carefully about how ours leads to better operations potential}

%Then section outline


















%\todo{actually describe the method, why it turns into poisson, missing species}




%\nikhil{intro language --}



% Paper 1 -- “Statistics/Science/Estimation” paper: Missing species as a method to identify underreporting in crowdsourcing, with an application to identify inequity/inefficiency in 311 data
% Claim 1: Here’s a method that works…
% It handles hierarchy well (we need to be more careful with this)
% Can add tree level covariates/location level covariates
% Can handle anything with duplicates -- that’s the connection with missing species
% Unlike naive missing species, we can estimate report rate even with incidents being born and dying
% Claim 2: We show that 311 crowdsourcing reporting is unequal by socioeconomics, and that this influences who gets government services (once we have lambda estimates)
% Metric: Some estimate for delay in services due to this unequal reporting
% We could set the stage for an operations paper -- maybe we do some simple simulations/something with undoing the effective of lambda
% Smaller claims:
% Other people have studied 311; their methods don’t work/our methods are better
% What are various pieces of the paper?
% There’s no reason to limit to tree data -- can use all the 311 data, as long as it has this parentID -- figure out what out of the public data has this parent id
% We could do simulations where we know the data generating process, and show our method works and the methods from other papers don’t
% Do we have any theory/proofs?




==> subsections/1_intro_short.tex <==


\begin{quote}
	If a tree falls in a forest, and no one reports it... does the city know about it?
\end{quote}
%
%
%	1. 311 systems are large and important, they determine allocation of city resources
%
%
Cities are complex socio-technical systems comprised of physical and human infrastructure, navigated by millions of people daily. A core part of monitoring such systems is crowdsourcing (or ``co-production'' \cite{yuan_co-production_2019,brabham_crowdsourcing_2015}), in which people report problems that they encounter; the New York City 311 system, for example, received \num{2592831} reports in 2020, and more than one hundred North American cities employ similar systems. Such reports are necessary, as they provide a real-time reflection on on-the-ground conditions that the city cannot hope to otherwise be aware of \citep{schwester2009examination, hacker_spatiotemporal_2020,minkoff_nyc_2016, lee_crowdsourcing_2021-1}. These reports are used alongside internal data collection and automated sensor technology to make both immediate decisions---such as which dangerous, downed trees to inspect and fix---and longer-term planning decisions, such as which streets to resurface. For example, the NYC Department of Parks and Recreation sends a forester to inspect about $\frac23$ of reports, and the incidents deemed risky (about $\frac12$ of inspected incidents) are resolved by a maintenance crew.

%2. However, if not used equitably, that's a problem. There is a large literature trying to measure this

While such reporting systems have gained popularity in the last few decades, there are many unresolved challenges in using reports efficiently and equitably. In particular, one long-standing concern is whether residents\footnote{We use the term ``residents'' to denote anyone who might report an issue to the 311 system, including visitors.} equitably use the system; or whether, conditional on experiencing the same issues, some residents are more likely to log a report and request government services \citep{thijssen2016you} -- for example, if socio-economically privileged neighborhoods submit more incident reports. If such reporting behavior is heterogeneous, then government services that rely on such reporting will also be inequitable. Though it is commonly believed that reporting behavior is heterogeneous, previous studies vary greatly in the quantification of such bias and how to attribute it to socio-economic or geographic characteristics
\citep{kontokosta_bias_2021,kontokosta_equity_2017,minkoff_nyc_2016,hacker_spatiotemporal_2020, clark_coproduction_2013,wu2020determinants, o2016311, thijssen2016you, vedlitz1980citizen,mclafferty_placing_2020, xu_closing_2020}.



%3. The issues with the current approach is either they can't identify, or they need ground truth to do so. This .

The central methodological challenge is the same reason that cities must rely on this information: ground truth conditions are unknown. This induces a missing data challenge: researchers do not observe what incidents occurred, or when they occurred. Thus, it is difficult to determine whether one neighborhood is \textit{under-reporting} issues compared to other neighborhoods, or whether they truly experience fewer issues (due to, e.g., differences in infrastructure). Previous work either does not attempt to distinguish between these cases (implicitly assuming that incident rates are similar across areas), or employs external data to construct \textit{proxies} for ground truth incident rates (such as population, length of roadways, number of apartments, or incident rates detected by the occasional active/random inspections). While accurate proxies can distinguish between incident rates and reporting rates, they may be difficult to construct or may not be precise enough to distinguish between types of incidents (e.g., whether reporting behavior differs by incident risk).

%4. Methodological
%a. We propose a way to measure this. Motivated by missing species, but additional issues. Turn it into poisson regression, etc.

\parbold{A method to identify reporting rates without ground truth data.} In this work, we propose a method to identify (heterogeneous) reporting rates, using \textit{just} the reporting data itself, without relying on external ground truth data. Our insight is that we can use information on \textit{duplicate} reports about the same incident (which cities commonly log), to identify reporting rates \textit{conditional on an incident having occurred}. This insight originates from the \textit{missing species} estimation literature, where the number of \textit{duplicate} observations provides evidence regarding the existence of unseen species \citep{orlitsky_optimal_2016, wu_chebyshev_2016, han2021competitive, charikar2019efficient}; if for every observed unique species, we have observed it many times, then it is unlikely that there are similar species that have never been observed.

Our setting differs from the classic \textit{missing species} formulation, in that the set of incidents is not static: new incidents occur (e.g., a tree falls down), and are resolved (the city fixes the issue, or it naturally disappears). And, even for observed incidents (those that are reported), we do not know \textit{when} they occurred, or \textit{how long} the incident existed. Thus, naively, we do not know, e.g., whether the incident was reported twice over a possible three month or one week period. This difference matters, as the possible reporting period varies substantially with incident characteristics and reporting behavior (e.g., hazardous incidents are reported and addressed more quickly).

We show how to nevertheless convert the task to a standard \textit{Poisson rate estimation} challenge, for which a large empirical and theoretical literature exists. In particular, one can use the number of reports between time of the first report (but not including it) and an estimated death time (that may depend on the data, e.g., time of the reports or when the incident was inspected), to recover a {Poisson} likelihood with a corresponding rate function. The method is valid if the estimated death time is an \textit{under-}estimate of the resolution time and is a \textit{stopping time} (does not depend on the future).

Then, we can leverage standard Poisson rate estimation methods (for example, estimate the MLE or a Poisson regression) to recover the (heterogeneous) rates that incidents of different types and in various neighborhoods are reported, conditional on the incident having occurred.

%5. Application oriented
%a. We apply it to Parks data, using data provided to us…

\parbold{Applying our method to understand equity in 311 usage.} We apply our method to over \num{100000} resident reports made to the forestry unit in the New York City Department of Parks and Recreation (DPR), using both publicly accessible data and internal logs on incident inspection outcomes and work orders, provided to us by DPR.
%
Using a Bayesian Poisson regression framework, we estimate how the reporting rate varies as a function of incident characteristics (e.g., the risk rating assigned by a forester upon inspection), space (location within New York City), and socio-economic characteristics of the neighborhood in which the incident occurred.

We illustrate that our method is indeed precise enough to find differences in reporting rates; for example, we find that reports for riskier incidents and trees in more critical condition are submitted at substantially higher rates, conditional on the incident having occurred.
%
Finally, we study spatial and socio-economic heterogeneity. We find that there are substantial inter-location reporting differences; for example, comparing census tract level fixed effects, we find that reports occur at a three times higher rate in downtown Manhattan than in uptown Manhattan, even after controlling for the incident-level characteristics. We further find that factors like race/ethnicity and education levels are  associated with reporting rates, though such socio-economic characteristics cannot explain much of the spatial heterogeneity. These findings suggest that the allocation of government services, if reliant on incident reporting, may neither be efficient nor equitable.

%works in high dimension, use bayesian poisson regression approaches

\smallskip

We believe that our method is a general, powerful approach to understanding reporting behavior in resident crowdsourcing systems, delivering precise reporting estimates without requiring ground truth data---only duplicate report data, that are already collected by city agencies. The rest of this paper is organized as follows. The remainder of this section contains related work. In \Cref{sec:model}, we formalize our model and research questions. In \Cref{sec:3}, we develop and analyze our method. In \Cref{sec:datapplication}, we apply our findings to data from the New York Department of Parks and Recreation. We conclude in \Cref{sec:conclusion}.





==> subsections/1_related_work.tex <==
\subsection{Related Work}
\label{sec:related}
Our work is most closely related to literature studying equity and efficiency in co-production systems, often called 311 systems. Our empirical approach is motivated by the \textit{missing species} literature, and we employ Bayesian Poisson regression approaches. It broadly connects to commonly considered crowdsourcing and civic engagement challenges, including equitable participation.

%Most generally, \todo{write}while having implications for the broader design of data .


\textbf{Equity and efficiency in co-production systems.} Given the importance of 311-like systems in allocating government services, there has been much interest in quantifying how efficient and equitable these systems are. Previous works mainly aim to answer two questions: (1) is \textit{reporting} behavior similar across socio-economic groups, and (2) do governments \textit{respond} to the reporting equitably, or do they prioritize some neighborhoods for the same types of requests? If there are disparities in either stage of the process, then government services may be allocated inequitably.


Towards the second question, there has been a long line of work since the late 1970s, documenting how the allocation of government services has changed since the adoption of co-production systems. Early works warned of the potential of biases in how governments responded \citep{jones1977,thomas1982}. Researchers have found response time differences between neighborhoods, e.g., during Hurricane Katrina \citep{elliott_race_2006}; other recent studies suggest that the practical differences induced by these differential response times are negligible \citep{clark_advanced_2020} or explained by other factors \citep{xu_closing_2020}.

This work considers the first question, on how reporting behavior varies across demographic and incident characteristics. The literature here focuses on two types of reporting behavior: \textit{under-reporting}, and \textit{misreporting}. The latter refers to when residents report problems that, upon inspection by the agency, are not found or are less severe than reported; there is some evidence that such misreporting occurs and is heterogeneous across areas \citep{mclafferty_placing_2020}.

On the other hand, differential \textit{under-reporting} is when people, faced with similar problems, differentially report those problems to the government. Such differences might emerge, for example, due to access to communications technologies, familiarity with the system, or trust in government \cite{buell2021surfacing}. As discussed above, the biggest challenge to studying \textit{under-reporting} is that researchers rarely directly observe an incident \textit{unless it is reported}. It is thus difficult to disentangle whether certain areas have fewer reports because problems truly occur less frequently there, or whether people in those areas are reporting less frequently given a similar distribution of problems.

One line of work in answering this question does not attempt to distinguish between these two possibilities. Such work entails regressing the number of reports (or number of unique incidents, if some incidents are reported multiple times) as a function of socio-economic and report characteristics, as well as potentially space and time \citep{clark_coproduction_2013,cavallo_digital_2014,minkoff_nyc_2016}. Such works have found that the number of reports may (but does not always) differ by wealth, race, and education level. However, as we formalize in \Cref{sec:identification}, such a method cannot identify whether these fewer reports are due to fewer true incidents, or less reporting for the same incidents. Rather, these works must assume that the latter is the cause. \citet{akpinar2021effect} point out that such an assumption may not always hold, affecting downstream models, in the context of crime reporting and predictive police systems.

Another approach to quantifying under-reporting is to construct a proxy for the true incident rate and then compare the estimates with the observed rates. \citet{kontokosta_bias_2021} analyze pothole complaints in Kansas City, Missouri, at a fine-grained spatial level; they leverage additional street assessment data (resulting from scheduled visual inspections) that grade the quality of roadways to construct relative predictions for the true number of potholes. They find that low-income and minority neighborhoods are less likely to report street condition or ``nuisance'' issues while prioritizing more serious problems. \citet{hacker_spatiotemporal_2020} use a similar metric, with the addition of temporal trends geared more towards an epidemiological study, and \citet{pak_fixmystreet_2017} use roadway length as part of their proxy. Finally, \citet{kontokosta_equity_2017} analyze residential building problem complaints in New York City's 311 system---using building conditions as a proxy---and also find that many socio-economic factors contribute to differential reporting behavior. While the approach can disentangle reporting behavior from true incident rates, it heavily relies on the accuracy of the `ground-truth' proxy estimate. It may be difficult to find such proxies or to validate their accuracy, especially for different types of incidents within the same class (e.g., more vs less serious potholes).

The challenge between identifying occurrence rates as opposed to reporting rates is also present in the ecology literature, when counting the number of animals of a given species in an area. Some works similarly use proxy methods -- such as by normalizing by occurrence rates in neighboring geographies or using reference species whose occurrence rates are approximately known \cite{hill2012local,renner2013equivalence,kery2008hierarchical}.


To this literature, our work contributes a statistical technique to identifying under-reporting---that does not require such external data or the construction of proxies for the ground truth incident rate. Rather, it relies only on report data already logged by many agencies, and connects this task to a large literature on Poisson rate estimation. In applying our method to 311 data, we find reporting rate differences across neighborhoods and associated with socio-economic status, and show that these differences are beyond what one would expect from just incident-level characteristics.




%. The authors predicted the likelihood of failure based on conditions of each building, and compared the prediction with actual number of complaints to characterize `over-reporting'. They found that a number of socio-economic factors contribute to difference reporting behavior.






%define a `reporting rate' as the ratio between number of actual reports and number of expected reports estimated by examining the conditions in each geographic location, basing on which classified neighborhoods into `over-reporting'.





%\citep{pak_fixmystreet_2017} used roadwork requests from FixMyStreet in Brussels, a Belgian counterpart of the 311 system, and constructed a variable indicating the number of reports relative to the total number of users and total street length in a district, with higher values of which suggests `over-reporting'. The authors tested the dependence of this variable on several socio-economic aspects, and found that higher income and less racially diverse neighborhoods tend to have higher values in this variable, which can be interpreted as a sign of higher participation.

%an essential task in identifying `over-reporting' behavior is distinguishing between the rate at which incidents, in their case crimes happen, and the rate at which residents report on these incidents.


% \citep{clark_coproduction_2013} used public from Boston's 311 system across difference departments and different data sources. For the citizen reports, the authors treated them as count data and performed a negative binomial regression to investigate its relationship with multiple socio-economic factors, with more reports in a neighborhood potentially meaning `over-reporting'. They concluded that though 311 system's favor towards specific racial groups is negligible in practice, that towards more affluent neighbourhoods is a concern. \citep{cavallo_digital_2014} used the same count data as dependent variable from three major US cities' 311 system, and performed a linear regression with socio-economic factors of each neighborhood as independent variables. The authors suggest that factors such as gender, racial diversity and education level have significant impact in the number of reports.\citep{minkoff_nyc_2016} used data from New York City's 311 system and tract level census data, and found that the number of contacts made by residents is dependent on a couple of socio-economic factors, with this dependency pattern varying across different types of reports.

%, and instead directly studies




%Other works tend to study the observed data themselves.



%Under-reporting
%
%; there has long been a concern that not all residents equally participate in reporting problems. The unequal access to modern information and communications technologies across difference demographics groups has worsened this fear. There has been multiple ways of characterizing and quantifying this equity concern. One of such ways is through testing the existence of different levels of `misreporting', that residents in certain neighborhoods tend to falsely report incidents at a higher rate in order to gain advantage of the system .

%More related to this work is another line of works which quantify equity concerns by examining the relationship between `over-reporting' behavior and socio-economic factors, where among them we see a divide in the definition of `over-reporting' behavior.

%On the one hand, a number of works used the ratio between the observed and the `ground-truth' as the measure for `over-reporting'. \cite{kontokosta_bias_2021} used data of self-reported non-emergency complaints on a variety of problems from Kansas City, Missouri's 311 system. The authors defined a `reporting rate' as the ratio between number of actual reports and number of expected reports estimated by examining the conditions in each geographic location, basing on which classified neighborhoods into `over-reporting'. They found that low-income and minority neighborhoods are less likely to report street condition or “nuisance” issues while prioritizing more serious problems. \citep{hacker_spatiotemporal_2020} used a similar metric, with the addition of temporal trends geared more towards an epidemiological study. From a similar starting point, \cite{kontokosta_equity_2017} used data from New York City's 311 system on residential building problem complaints. The authors predicted the likelihood of failure based on conditions of each building, and compared the prediction with actual number of complaints to characterize `over-reporting'. They found that a number of socio-economic factors contribute to difference reporting behavior. This approach to `over-reporting' heavily relies on the accuracy of the `ground-truth' estimation.
%
%
%
%\citep{pak_fixmystreet_2017} used roadwork requests from FixMyStreet in Brussels, a Belgian counterpart of the 311 system, and constructed a variable indicating the number of reports relative to the total number of users and total street length in a district, with higher values of which suggests `over-reporting'. The authors tested the dependence of this variable on several socio-economic aspects, and found that higher income and less racially diverse neighborhoods tend to have higher values in this variable, which can be interpreted as a sign of higher participation.










%To address this difficulty, we quantify the behavior of `over-reporting' by looking at the rate at which residents report on an incident, conditional on the incident has taken place, thus providing a methodology to effectively distinguish the incident rate and the reporting rate.

\textbf{Missing species and Bayesian estimation.} The central idea of our work is that one can leverage \textit{duplicate} reports about the same incident to identify the true incident rate from the reporting rate. This insight derives from the \textit{missing species problem} \citep{goodtoulmin}, where the number of \textit{duplicate} observations provides evidence regarding the existence of unseen species. Tackling this challenge has been regarded as ``very first empirical Bayes success story'' \cite{casi}, and there has been substantial recent theoretical interest in the transformation of this question to that of estimating the support of probability distributions that satisfy certain general properties \citep{orlitsky_optimal_2016, wu_chebyshev_2016, han2021competitive, charikar2019efficient}. A related technique is ``mark-recapture,'' to count the population of a given species \cite{petit2006estimating,crosbie1985parsimonious}. %\zhi{put Kiran's two most related works here, and added a bit intro for them}

Our setting differs from the classic missing species setup in that incidents are \textit{born} and \textit{die} (are fixed, or otherwise resolved), and that we do not observe the birth and death times. This temporal dynamic induces a further identification challenge; nevertheless, we show how to transform our task into a standard Poisson \textit{rate estimation} challenge. In this way, we are able to utilize a wide swath of literature dedicated to this question, both on the estimation side, e.g. \citep{lambert1992zero} and on the modeling side, e.g., \citep{efron_2010, ignatiadis2020}. While we focus on Bayesian Poisson regression and spatial aspects, we note that the latent (unknown) incident occurrence time in our setting is akin to the unknown `death' time in ``buy-till-you-die'' models in the marketing literature \citep{fader2005counting, abe_counting_2008}.  It is possible that time-reversed versions of those models can be adapted for this setting.


% \todo{cite more}\zhi{I believe these two should be sufficient}.
%We, on the other hand, formalize the intuition of using duplicate reports, and by building on a simple Poisson distribution assumption central to the original missing species problem, are able to transform our problem into a \textit{rate estimation} problem.


% \todo{cont here...that it transforms to bayesian regression..., add missing species citations}

% Once we have used the above insight to transform the challenge into a more traditional rate estimation question, we can leverage a wide swath of literature dedicated to this question. \todo{e.g., find fancy poisson regression applications, spatial regression, etc.}  \todo{cite -- \url{https://pubsonline.informs.org/doi/pdf/10.1287/mksc.1090.0502?casa_token=9J_giM2a-4cAAAAA:QTjclotyTy7bVpLaHw9neB413lji4a4Of7oUHkiXNZ73ddZKvOcJjUbY3io1Uox3dUrIb7G2FRE}};



% \todo{Zhi -- can you take these papers (and others Kiran sent over email) and put them in bibtex and add them here as \cite{}? That would make it easier a I'm writing; also feel free to do a first draft of this}
% \zhi{on it -- finished as far as I can see}

% Not sure: how to approach the missing species literature, as we do not really use that much technical tools

% Missing species papers (from Kiran):
% https://arxiv.org/abs/1504.01227, \citep{wu_chebyshev_2016} https://www.pnas.org/content/113/47/13283
% \citep{orlitsky_optimal_2016}

%"The very first empirical Bayes success story related to the butterfly data of Table 6.2." -- pg 78 of CASI
%\citep{casi} \zhi{not sure where this belongs}

%"The crucial point, and the surprise, is that large data sets of parallel situations carry within them their own Bayesian information. Large parallel data sets are a hallmark of twenty-first-century scientific investigation, promoting the popularity of empirical Bayes methods."

% Empirical bayes citations: [Efron, 2010, Robbins, 1964].   \citep{robbins_1964} From 1906.01611.pdf (arxiv.org) \citep{ignatiadis2020}


%Intepreting coefficients in poisson -- page 267 \zhi{not sure what this is referring to, CASI?}

\textbf{Other crowdsourcing and civic engagement settings.} 311 (or `co-production') systems are part of a broader constellation of crowdsourcing and civic engagement systems, in which residents contribute to governmental decisions such as legislation and resource allocation; for example, participatory budgeting and deliberative democracy are well studied \cite{aziz2021participatory,pateman_participatory_2012,cabannes_participatory_2004,lee_crowdsourcing_2014,mcdermott_building_2010,posner_voting_2015,procaccia_approximate_2009,sintomer2008porto,gilman2020transformative,garg2019iterative,Aziz2021,FREEMAN2021105234,garg2021markets,goel2019knapsack,fishkin2018deliberative,deliberationjuryconsistent}. Whether participation is equitable is a common worry \citep{griffinjiao2019,brabham2009crowdsourcing,hudson2018does,shortall2021inclusion}, and others have attempted to improve representative-ness in such civic engagement systems \cite{gelauff2020,flanigan2021fair}.  Our setting also broadly relates to the peer prediction and grading literature, in evaluating crowdsourced answers without ground truth \citep{miller2005eliciting,witkowski2012peer,shnayder2016informed,liu2017machine,agarwal2020peer}. Surprisingly, given the popularity, scale, and importance of 311 systems---among the biggest, most consequential crowdsourcing systems in continuous use---to our knowledge their design (either a market design or operations perspective) has not been considered in the EconCS community.


%This work also contributes to the broader literature on crowdsourcing and civic engagement. Used in multiple areas involving planning \citep{griffinjiao2019,brabham2009crowdsourcing} and even legislature \citep{hudson2018does}, the equity concerns in the usage of crowdsourced data and the crowdsourcing approach is through much scrutiny.

% There are literature focusing on the mechanism design aspects of common job crowdsourcing \citep{easley2015, stouras2020, yin2015bonus},\zhi{these papers seem to be good fit for the EC flavor} discussing topics such as rewarding agents and designing contracts  in order to achieve better performance as a platform. We see the potential of those mechanism design problems being applied to study the equitable design of data crowdsourcing platforms, and our work provides a solid foundation for a first step in implementation.


%\todo{Connect to crowdsourcing/other literature from EC communities}

%cite regarding other work in inequities in civic participation: https://arxiv.org/abs/2006.03983



% equity in crowdsourcing -- \url{https://journals.sagepub.com/doi/full/10.1177/0361198118823498}

%\nikhil{other 311 uses:} \citep{wang2017structure}







==> subsections/1_related_work_short.tex <==
\subsection{Related Work}
\label{sec:related}
Our work is most closely related to literature studying equity and efficiency in co-production systems, often called 311 systems. Our empirical approach is motivated by the \textit{missing species} literature, and we employ Bayesian Poisson regression approaches. It broadly connects to commonly considered crowdsourcing and civic engagement challenges, including equitable participation.


\paragraph{Equity and efficiency in co-production systems.} Given the importance of 311-like systems in allocating government services, there has been much interest in quantifying how efficient and equitable these systems are. This work aims at answering the question of whether \textit{reporting} behavior is similar across socio-economic groups, with a particular focus on the type of reporting behavior known as \textit{under-reporting}, which is when people, faced with similar problems, differentially report those problems to the government. Such differences might emerge, for example, due to access to communications technologies, familiarity with the system, or trust in government \cite{buell2021surfacing}. As discussed above, the biggest challenge to studying \textit{under-reporting} is that researchers rarely directly observe an incident \textit{unless it is reported}. It is thus difficult to disentangle whether certain areas have fewer reports because problems truly occur less frequently there, or whether people in those areas are reporting less frequently given a similar distribution of problems. Towards this challenge, previous literature either assume a uniform incident occurrence, thus concluding any heterogeneity in the observed reports is a result of differential reporting rate \citep{clark_coproduction_2013,cavallo_digital_2014,minkoff_nyc_2016}; or construct proxies to account for differences in incident occurrence, and then compare the estimates with observed rates \citep{kontokosta_bias_2021, hacker_spatiotemporal_2020, pak_fixmystreet_2017, kontokosta_equity_2017}. Both lines of work require some form of external data or strong assumptions, which the technique we propose does not.




\paragraph{Missing species and Bayesian estimation.} The central idea of our work is that one can leverage \textit{duplicate} reports about the same incident to identify the true incident rate from the reporting rate. This insight derives from the \textit{missing species problem} \citep{goodtoulmin}, where the number of \textit{duplicate} observations provides evidence regarding the existence of unseen species. 



% \paragraph{Other crowdsourcing and civic engagement settings.} 311 (or `co-production') systems are part of a broader constellation of crowdsourcing and civic engagement systems, in which residents contribute to governmental decisions such as legislation and resource allocation; for example, participatory budgeting and deliberative democracy are well studied \cite{aziz2021participatory,pateman_participatory_2012,cabannes_participatory_2004,lee_crowdsourcing_2014,mcdermott_building_2010,posner_voting_2015,procaccia_approximate_2009,sintomer2008porto,gilman2020transformative,garg2019iterative,Aziz2021,FREEMAN2021105234,garg2021markets,goel2019knapsack,fishkin2018deliberative,deliberationjuryconsistent}. Whether participation is equitable is a common worry \citep{griffinjiao2019,brabham2009crowdsourcing,hudson2018does,shortall2021inclusion}, and others have attempted to improve representative-ness in such civic engagement systems \cite{gelauff2020,flanigan2021fair}.  Our setting also broadly relates to the peer prediction and grading literature, in evaluating crowdsourced answers without ground truth \citep{miller2005eliciting,witkowski2012peer,shnayder2016informed,liu2017machine,agarwal2020peer}. Surprisingly, given the popularity, scale, and importance of 311 systems---among the biggest, most consequential crowdsourcing systems in continuous use---to our knowledge their design (either a market design or operations perspective) has not been considered in the EconCS community.









==> subsections/2_data_generating_model.tex <==

\label{sec:model}

 \begin{figure}[tbh]
	\centering
	\includegraphics[width=\textwidth]{plots/data_gen_1.pdf}
	\caption{Model of resident reports of an incident $i$ of type $\theta$. Observed and unobserved events are marked with solid and dotted lines, respectively. In this example, there are a total of 3 reports made about this incident. When the reporting rate is an homogeneous Poisson process with rate $\lambda_\theta$, the average reporting delay is $\frac{1}{\lambda_\theta}$.}
	\label{fig:reports_gen}
\end{figure}

We now introduce our model for how 311 reports are generated, as well as our research questions. % and empirical strategy for answering them.
% We note that our descriptive language language we focus on the setting where residents report on incidents concerning trees in the public space.
%\subsection{Model of data generating process}
The data are composed of a set of resident \textbf{reports}, each belonging to an \textbf{incident} $i$ of type $\theta$.  Type $\theta$ encodes geographic (e.g., location, and demographic and place characteristics thereof) and incident-specific (e.g., tree height, whether it is a hazard, and inspection results) characteristics.  \Cref{fig:reports_gen} illustrates the model for a given incident.

\parbold{Incident birth and death.} Incidents of type $\theta$ occur (``are born'') according to a random process parameterized by $\Lambda_\theta$. (For example, a homogeneous Poisson process with rate $\Lambda_\theta$). For each incident $i$, let $t_i$ denote its birth time. Furthermore, the incident `dies' at some time $t_i + T_i$, and no more reports are logged. The death time reflects, for example, a completed work order fixing the issue, another resolution, or reports no longer being logged because the issue has been inspected. Though the birth and death processes of incidents may induce other interesting research questions, we do not make any further assumptions on them, as they are beyond the scope of this paper.

%It follows that in a time interval of length $t$, the number of incidents $N_\theta$ of type $\theta$ follows a Poisson distribution with parameter $t \Lambda_\theta$. \nikhil{Is anything we do tied to this Poisson process, or can incident process be arbitrary?}

\parbold{Reports.} Incidents are not directly observed by the city. Rather, the city observes {reports} made by the public, once an incident has occurred. There are two notable facts regarding reports. First, they may not come in immediately after an incident occurs -- it takes a (random) amount of time for someone to first notice an incident and consider it worth reporting. Second, there often are \textit{duplicate} reports, about the same incident. Multiple residents may encounter the same incident and report it. Crucially, city agencies often identify and log such duplicates, as it is important to do so when deciding which reports to address and auditing response rates and times.

 For an incident $i$ of type $\theta$, we assume that---while it is alive, i.e., in time $[t_i, t_i + T_i]$---reports are submitted according to a (potentially non-homogeneous) Poisson process, with rate $\lambda_\theta(\tau)$ at incident age $\tau \in [0, T_i]$. Thus, the number of reports $M_i$ for incident $i$ follows a Poisson process, $M_i \sim \text{Poisson}\left(\int_{\tau = 0}^{T_i} \lambda_\theta(\tau) d\tau\right)$.






\parbold{Observed data.} We observe reports and city actions. Each report comes with a time-stamp and identifies its corresponding incident $i$ (thus, duplicate reports are assumed to be accurately connected to previous reports of the same incident). For each incident, we further know its type $\theta$ (as detailed in \Cref{sec:datapplication}, type $\theta$ can be composed of both data available at report time, or after an inspection; we assume each report about an incident is identical in terms of $\theta$).

Putting things together, from the viewpoint of the 311 system (and researchers), the observed data for a time interval $(0, T)$ consists of the following, for each type $\theta$. Suppose there are $N_\theta$ incidents of the type. We observe $N^{\obs}_\theta \leq N_\theta$ of these incidents, corresponding to the incidents $i$ with at least one report, $M_i \geq 1$. For each such incident, we observe $M_i$ and each report time.

Finally, we observe how the agency responded to the incident, such as when an inspection was completed, the outcome of the inspection, and the details of any completed work order.

%\nikhil{Not sure need this here} We further observe report inter-arrival times \textit{after the first report}; i.e., let $t_i^m$ for $m  \in \{0, \dots M_i-1\}$ be the inter-arrival time between the $(m+1)$th and $m$th reports, where $m=0$ corresponds to the incident birth. Then, we observe $\{t_i^m\}_{m = 1}^{M-1}$ but not $t_i^0$, the time between incident birth the first report, as we do not observe the incident birth time $t_i$. We further do not directly observe the incident death time $T_i$, or the time between the last report and death, $t_i^{M_i}$.

% For an incident with $M_i$ total reports, we denote by ;


%  , and $t_i^M$ denotes the time between the death time and time of last report. It follows that $T_i= \sum_{m=0}^{M_i} t_i^m$. Note that we only observe $t_i^m$ for $m=1,...,M_i$.
%\zhi{how does this notation work?} \nikhil{notation fine I think}


%, and truthfully reports its type $\theta$ \nikhil{think about observable vs unobservable?}. Further, we assume .




%We use $t_i^m$ to denote the time that the $m$th report about incident $i$ is observed. For each report, we observe the report time and the incident $i$ to which it belongs (and thus its type).



%\subsection{Research questions and model discussion}


\parbold{Research questions.} In this work, we are primarily interested in auditing the efficiency and equity of the reporting process: how quickly are incidents reported, and how does that reporting rate $\lambda_\theta$ vary with the incident type $\theta$? (While we primarily measure and interpret our results in terms of reporting rates $\lambda_\theta$, estimating this rate also allows us to calculate, for example, the fraction of incidents reported within a certain time period and other operationally relevant measures.)


The primary methodological task is overcoming the missing data challenge: we do not observe incidents that are never reported, nor birth times $t_i$ of the incidents that are reported. This missing data makes it difficult to distinguish between incident rate $\Lambda_\theta$ and reporting rate conditioned on an incident, $\lambda_\theta$. In fact, as we explain next in \Cref{sec:identification}, it is impossible to do so with just the above data, if one throws away the information on duplicates; our main insight is that by using this duplicate data, in contrast, one can identify $\lambda_\theta$ in practically reasonable settings.



\parbold{Model discussion.} As discussed in \Cref{sec:related}, \textit{mis-reporting} is also a concern in many settings. We in contrast assume that the reported types are correct (in the data section, if different reports for the same incident disagree, we keep the \textit{first} report type). Estimating such mis-reporting alongside under-reporting is an interesting avenue for future work. Furthermore, the data also enables calculating the \textit{inter-arrival times} between reports. Such information is valuable for estimating non-homogeneous Poisson rates, but we do not do so here. Finally, we note that our method does not directly consider \textit{causal} reasons that a neighborhood may have a lower reporting rate than another; \citet{buell2021surfacing} find that operational transparency increases trust in government and reporting rates, and technological access and familiarity may also play a role.


In what settings is the model applicable? First, while the incident occurrence process $\Lambda_\theta$ can be arbitrary, the reporting rates $\lambda_\theta$ must be Poisson --  reports about the same incident must be independent. This assumption requires filtering out duplicate reports made by the same individual, as we do in our application. Second, the analysis requires that the agency log information about duplicate reports; this is commonly done in co-production systems---e.g., \citet{kontokosta_equity_2017} mention filtering out duplicates in their work. While our data application focuses on reports to a single agency in NYC's 311 system, these requirements are widely met in other contexts, including beyond co-production systems.

%One extra information that is included in the data, but not specified in our model, is . This , or if determining the `death-rate' of incidents is important, which is seen in `but-till-you-die' models. However, since our empirical approaches and application are primarily focused on the time homogeneous setting, this part of the information is omitted in our modeling.

%\todo{not talking about misreporting yet -- assume that type is correct. in preprocessing, that we took the first report type.}

% \todo{need to finish this language} \nikhil{talk about real world that generates these poisson reporting distributions} Duplicate reports may consist of the same reporter calling again regarding the same incident, in order to receive an update or to suggest urgency in the situation being resolved. Our approach (especially one with homogeneous rates until a resolution time) is best suited for unique callers, so that report inter-arrival times remain independent. 311 systems often ask (but do not require) that reporters provide their contact information so that they may follow up. In \Cref{sec:datapplication}, we use this (anonymized) data provided to us by NYC DPR to check the robustness of our calculations to such repeat callers. \nikhil{This one, and some of the others above, probably in a conclusion/discussion as opposed to here}




%\nikhil{unedited text below this}

%In this subsection we introduce the data generating process for 311 resident reports. More specifically, we focus on the setting where residents report on incidents concerning trees in the public space.

%This rate parameter is dependent on two sets of variables: a set of variables indicating the category of the incident, which includes its severity, the type of tree that it occurs on, denoted by $\kappa$, and a set of geographical variables, denoted by $\theta$. Thus we will be using $\Lambda(\kappa, \theta)$ to denote the rate of an incident of category $\kappa$ happening in a specific region $\theta$. Naturally,  We will be using $N(\cdot)$ to denote variables related to the number of incidents.

%Sometime after an incident happens, it would either be planned to be fixed by the City, or would be inspected and determined that no further actions are needed. We denote by $T$ the time horizon that residents are interested in reporting this incident to the 311 system, i.e. the time between an incident is `born' and `dies'.

%\todo{consider nonhomogeneous reporting}

%During this reporting horizon, we assume that residents report this incident to the 311 system according to a Poisson process with time-invariant rate parameter denoted by $\lambda$. This reporting rate is dependent on two sets of variables: the same set of variables $\kappa$ which indicate the characteristic of the incident itself, and a set of socio-economic variables $\gamma$, which reflects the geographic region $\theta$. Thus we will be using $\lambda(\kappa,\gamma)$ to denote the rate of an incident of category $\kappa$ being reported in a region with socio-economic status $\gamma$. It follows that the number of reports on an incident, given this set of variables over a time period $T$, denoted by $M(\kappa,\gamma,T)$ follows a Poisson distribution with parameter $T\lambda(\kappa,\gamma)$. We will be using $M(\cdot)$ to denote variables related to the number of reports.

%Standing at the viewpoint of the 311 system, the observed data consist of several parts. Consider a period of time $t$, we would observe the total number of reports $M(\kappa,\gamma,t)$ for all $\kappa,\gamma$ and the number of observed incidents $N_{observed}(\kappa,\theta,t)$ for all $\kappa, \theta$, where we say an incident is observed if at least one report about it came in. For all $\kappa,\gamma$, each report of this kind, $i_{\kappa,\gamma} = 1,\dots,M(\kappa,\gamma,t)$, we observe the time that it comes in, $t_{i_{\kappa,\gamma}}$. For all $\kappa,\theta$, each incident of this kind, $j_{\kappa,\theta} = 1,\dots,N_{observed}(\kappa,\theta,t)$, we observe an estimate of the time that it dies, $t_{j_{\kappa,\theta}}$. Denote $I_{j_{\kappa,\theta}}\subset \{1,\dots,M(\kappa,\gamma,t)\}$ the set of indices of the reports about incident $j_{\kappa,\theta}$, \todo{unclear how to write dependence of $\theta$ and $\gamma$, might just make them the same?}we also observe all sets $I_{j_{\kappa,\theta}}$ for all $j_{\kappa,\theta}$ and $\kappa,\theta$.

% we would observe the total number of reports $M(\kappa,\gamma,t)$ for all $\kappa,\gamma$ and the number of observed incidents $N_{observed}(\kappa,\theta,t)$ for all $\kappa, \theta$, where we say an incident is observed if at least one report about it came in. For all $\kappa,\gamma$, each report of this kind, $i_{\kappa,\gamma} = 1,\dots,M(\kappa,\gamma,t)$, we observe the time that it comes in, $t_{i_{\kappa,\gamma}}$. For all $\kappa,\theta$, each incident of this kind, $j_{\kappa,\theta} = 1,\dots,N_{observed}(\kappa,\theta,t)$, we observe an estimate of the time that it dies, $t_{j_{\kappa,\theta}}$. Denote $I_{j_{\kappa,\theta}}\subset \{1,\dots,M(\kappa,\gamma,t)\}$ the set of indices of the reports about incident $j_{\kappa,\theta}$, \todo{unclear how to write dependence of $\theta$ and $\gamma$, might just make them the same?}we also observe all sets $I_{j_{\kappa,\theta}}$ for all $j_{\kappa,\theta}$ and $\kappa,\theta$.

%We further denote $d_{j_{\kappa,\theta}}=|I_{j_{\kappa,\theta}}|$ as the number of reports about incident $j_{\kappa,\theta} = 1,\dots,N_{observed}(\kappa,\theta,t)$ for all $\kappa,\theta$, and denote $T_{j_{\kappa,\theta}}=t_{j_{\kappa,\theta}}-\min\{t_{i_{\kappa,\gamma}}|i_{\kappa,\gamma}\in I_{j_{\kappa,\theta}}\}$ as the time between the observed death of an incident and the time that the first report about it came in, for all incidents $j_{\kappa,\theta} = 1,\dots,N_{observed}(\kappa,\theta,t)$ and all $\kappa,\theta$.


% all the reports and the time they are made are observed. In hindsight, if several reports are related to the same incident, this duplicate behavior is noted. Finally, a noisy signal of the incident death time is observed. This can either be the time that the work order is placed, or the time of the inspection which closes the case.






==> subsections/2_identifiability_issue_new.tex <==
%In this section, stemming from the difficulty in identifying the true reporting rate in order to quantify over-reporting behavior, we introduce a number of empirical approaches, which all draw upon the valuable information embedded in the duplicate reports.


This section lays the groundwork to estimate the rate function $\lambda_\theta$. There are two primary challenges: identification of $\lambda_\theta$ (primarily, disentangling reporting rates from incident occurrence rates $\Lambda_\theta$), and the high-dimensional nature of $\theta$ in our setting. \Cref{sec:identification} shows that $\lambda_\theta$ is identifiable -- using standard Poisson rate estimation techniques; then, we leverage this result in \Cref{sec:poissonreg} to develop Bayesian Poisson regression approaches to estimate $\lambda_\theta$ as a function of $\theta$. Finally, we evaluate our approach in simulation in \Cref{sec:simulation}.


% first, due to the missing data (incidents never reported, and birth times $t )

\subsection{Identifying reporting rate $\lambda_\theta(\cdot)$}
\label{sec:identification}

Estimating reporting rates $\lambda_\theta$ as a function of $\theta$ is of interest to good governance activists and researchers, as 311 reports are a key data source in the allocation of government services. Existing approaches either do not disentangle reporting rates from incident rates, or use external data to do so. Here, we show, in contrast, that $\lambda_\theta$ is identifiable using just reporting data, \textit{if we use data on duplicate reports} about the same incident. In this section, we assume a \textit{fixed} incident type $\theta$, and so often omit it from the notation.


\subsubsection{Non-identifiability using just number of incidents observed} Our first result, however, formalizes that the task is impossible using just data on the total number of unique incidents observed for each type in a time interval $(0, T)$, even if both incident occurrence and reporting follow time-homogeneous Poisson processes, with $\Lambda_\theta(\tau) = \Lambda_\theta$ and $\lambda_\theta(\tau) = \lambda_\theta$.

\begin{restatable}[Non-identifiability of reporting rate]{proposition}{propnonidenti}\label{prop:identi} Consider the simplest setting: both incident occurrence and reporting follow time-homogeneous Poisson processes, with $\Lambda_\theta(\tau) = \Lambda_\theta$ and $\lambda_\theta(\tau) = \lambda_\theta$. Further, let incident reporting durations $T_i$ be distributed according to $F$. Then using just the number of observed incidents $N_\theta^\obs(T)$ of type $\theta$ in a known time duration $[0, T]$, the reporting rate $\lambda_\theta$ is not identifiable. In other words, $N_\theta^\obs(T)$ is a function of both $\Lambda_\theta$ and $\lambda_\theta$:
\begin{align*}
	&\lim_{T \to \infty} \frac{N_\theta^\obs(T)}{T} = \Lambda_{\theta}'\\
	\text{where\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,} &\Lambda_{\theta}' = \Lambda_{\theta}\left[1-\int_{0}^\infty\exp\left(-\lambda_\theta t\right)\text{d}F(t)\right].
\end{align*}
% Thus, $\lambda_\theta$ cannot be identified.
\end{restatable}

The proof follows from the observation that, conditional on the number of incidents that occurred, the number observed is a Binomially distributed random variable that depends on the reporting rate. The number of observed incidents thus depends on both reporting and incident rates; it is thus not possible to distinguish between high incident rate/low reporting rate and low incident rate/high reporting rate just based on the observed reports. An identical result holds if we only count the total number of reports. That result follows from compounding the reporting rate conditional on an incident being observed upon the observation rate. For brevity, the proofs for \Cref{prop:identi} and the later \Cref{thm:stoppingtimes} are omitted in this short version for brevity.


The idea -- confounding incident occurrence and reporting -- behind \Cref{prop:identi} is not novel, and has especially been pointed out in policing settings~\cite{lum2016predict}; e.g., recently in the context of predictive policing systems, \citet{akpinar2021effect} study the downstream consequences of mistakenly using $N_\theta^\obs(T)$ as a proxy for the incident rate. Nevertheless, many works in the literature use such a proxy. Next, we show how to disentangle reporting and incident rates, without needing external ground truth data, by using data on \textit{duplicate reports} about the same incident.

%Combined with the Poisson assumption of incident occurrence, we arrive at the conclusion that reporting rate and the incident rate are `mixed up' to generate the unique incidents that we can observe.


%In conclusion, either counting unique incidents observed or counting reports without concerning to which incident they belong, will not get around this non-identifiability issue. Some previous works \citep{clark_coproduction_2013,cavallo_digital_2014,minkoff_nyc_2016} may suffer from this deficiency. However, as we will show next, there is a straightforward remedy to this problem,




\subsubsection{Identifiability using data on duplicates}
\label{sec:convertingtopoissonregression}



Our main insight is that one can identify the reporting rate using \textit{duplicate} reports about the same incidents: the first incident report informs us that this incident exists, and the remaining reports identify the reporting rate.

% section outline
%	1. If we observed everything, just do Poisson regression
As starting intuition, suppose we observe every incident (even those without reports) and, for every incident, the birth times $t_i$ and death times $t_i + T_i$---that all events in \Cref{fig:reports_gen} are observed. Then one could directly apply standard Poisson estimation techniques in order to learn the rates $\lambda_\theta(\cdot)$ for each type $\theta$: under our assumptions, the number of reports for an incident $i$ follows a Poisson distribution, $M_i \sim \text{Poisson}\left(T_i \int_0^{T_i} \lambda_\theta(\tau)d\tau\right)$. Depending on the assumptions on the time-non-homogeneous nature of $\lambda_\theta(\cdot)$, the corresponding estimation challenge for $\lambda_\theta(\cdot)$ is tractable.

%2. First issue, only observe those for which M_i > 1; This is exactly the missing species problem. The key insight we use is duplicate…
The first complication is that we do not observe every incident, only those with at least one report, $M_i \geq 1$. Our first insight is that this challenge is akin to that in \textit{missing species} literature discussed above, where a biologist only knows of species they have spotted at least once. The key idea in that literature -- that we leverage and adapt -- is that the \textit{number of times} we observe a species \textit{that we have observed at least once} provides information about how many species exist but have not yet been observed. The conditioning removes the dependence on the birth process $\Lambda$. In particular, conditioning on observing each such species at least once, we can use the distribution of how many species we spot twice, thrice, etc, to estimate the rate at which one observes that species, and back out the probabilities for observing that kind of species at least once -- under some assumptions on how the rates at which one observes species multiple times relates to observing it the first time. As discussed in the related work, this line of work has a long history. Our central assumption is similar, that the rate of duplicate reports \textit{after} the first report about an incident $i$ -- after which the city has learned the incident exists -- is informative of the overall reporting rate.

%3. However, we have a second issue. For those we observe, we don't observe their birth times t_i, nor their death times T_i.
In our setting, however, there is a second complication that prevents us from using off-the-shelf  estimators from the {missing species} literature: incidents do not always exist (like species), but rather are born and die -- our system evolves over time, and we do not directly know $t_i$ or $t_i + T_i$ (as, by definition, the city only learns of incidents after they have been reported). Qualitatively, the difference is that we cannot naively distinguish between an incident being born a long time ago but with low reporting rate, or an incident just recently being born. Our second insight is that $\lambda_\theta(\cdot)$ is still identifiable, in a  (practically reasonable) setting described next.


%4. Here, we leverage the following result…

\textbf{Identification with stopping-time time intervals} Our empirical strategy is based on the following technical result, which shows that, even if the observation interval for a Poisson process is defined by \textit{stopping times}, the likelihood function can be decomposed such that we can leverage standard Poisson rate estimation techniques. Here, a time $t$ being a \textit{stopping time} means that it can depend on everything that occurs before that time (e.g., on the number of reports received up to time $t$), but, conditional on this past and type $\theta$, it is independent of the future and process parameter $\lambda$.

%a. And then the result, but just the first part
\begin{restatable}{theorem}{thmst}\label{thm:stoppingtimes}
	Consider each incident $i$, born and dead at unknown times $t_i$ and $t_i + T_i$. Suppose that, while alive and aged $\tau \in [0, T_i]$, the incident is reported at rate $\lambda(\tau)$.

	Let the data for incident $i$ be $D_i = (\tilde M_i, \tilde t_i, \tilde T_i)$, where $\tilde t_i$ is the start of an observation period, $\tilde T_i$ is the duration of that period, and $\tilde M_i$ is the number of reports observed in time period $(\tilde t_i, \tilde t_i + \tilde T_i]$. Further, suppose that $(\tilde t_i, \tilde t_i+ \tilde T_i] \subseteq [t_i, t_i + T_i]$ and that $\tilde t_i$ and $\tilde t_i + \tilde T_i$ are stopping times, adapted to the natural filtration of the Poisson process characterizing the reporting behavior, and independent of $\lambda$ given $\theta$.	Let $\tilde{Pr}(\{D_i\} | \lambda(\cdot))$ denote the likelihood function of the data, given the rate function $\lambda$. Then,
	\begin{align}
		\tilde{Pr}(\{D_i\} | \lambda(\cdot)) &= {Pr}(\{D_i\} | \lambda(\cdot)) g(\{D_i\}),
		\intertext{where ${Pr}({D_i} | \lambda(\cdot))$ corresponds to the standard Poisson likelihood with an appropriate rate function:}
		\tilde M_i &\sim \text{Poisson}\left(\int_{\tau = \tilde t_i - t_i}^{(\tilde t_i - t_i) + \tilde T_i } \lambda(\tau)d\tau \right), \label{eq:poissonnonhom}
		\intertext{and $g$ is a function that does not depend on $\lambda$. Thus, the MLE and the posterior distributions for $\lambda(\cdot)$ also match the corresponding Poisson values. For example, when reporting rate is homogeneous ($\lambda(\tau) \triangleq \lambda$), the maximum likelihood estimate for $\lambda$ is }
\hat{\lambda}^{MLE} &= \frac{\sum_{i}\tilde M_i}{\sum_{i}\tilde T_i}. \label{eq:MLE}
	\end{align}
The decomposition does not hold in general, if $\tilde t_i$, and $\tilde t_i + \tilde T_i$ are not stopping times.

\end{restatable}
%i. Note that this would be trivial from stopping time if T_i was fixed, but here as long as they are not functions of the future, we are fine.
%

The result follows directly from writing the likelihood function in terms of the report inter-arrival times, and then observing that the likelihood decomposes. We note that $\tilde t_i$ (the start of the observation period) being a stopping time not affecting estimation is a trivial consequence of the memory-less property for Poisson processes. Thus, if we had assumed fixed $T_i$ and $\tilde T_i$ (or random, but also independent of the sample path), the above result would immediately follow.
%
Surprisingly, we could not find rate estimation literature in which the length of each observation period $\tilde T_i$ depends on the sample path (but is a stopping time), and so require \Cref{thm:stoppingtimes}.

Why is the setting important? In our data, incidents may be fixed (via a work order) or reports may stop being tagged to the incident after an inspection -- these outcomes are represented by the death time $t_i + T_i$. However, these outcomes are \textit{potentially dependent on the reports}: for example, incidents with more reports or reported as a \textit{Hazard} type may be prioritized for an inspection or work order; \Cref{tab:Summary} suggests that, indeed, such prioritization occurs in our data. Without the above result, we would need to choose a fixed observation duration $\tilde T$ such that $\tilde t_i + \tilde T \leq t_i + T_i$ for all incidents $i$, leading us to discard much data. With \Cref{thm:stoppingtimes}, however, we can choose data dependent durations $\tilde T_i$, as described below.

Why is it necessary that $\tilde t_i + \tilde T_i$ be a stopping time, conditionally independent of the future and $\lambda$? Suppose we instead choose the end of the observation period $\tilde t_i + \tilde T_i$, as ``the time of the \textit{last} report for the incident.'' This time depends on the future, as we must know that there are no further reports. Then, our estimation for rate $\lambda(\cdot)$ would be biased upward, as we systematically exclude a time period in which the incident was alive but we know no more reports were submitted.


Finally, note that we also observe the inter-arrival times between reports; \Cref{thm:stoppingtimes} extends to using those as data (our proof in fact first writes down the likelihood in terms of the inter-arrivals, and then marginalizes them out). However, we exclude it from the statement for clarity, as our current model specifications (see \Cref{sec:poissonreg}) do not use this data.


% \nikhil{talk about the confounding example? or say something about fixed theta in beginning of this section}

\textbf{Applying the result to our setting} How do we apply \Cref{thm:stoppingtimes} to our setting? Given that we do not know birth time $t_i$ or lifetime $T_i$, we require a known interval $(\tilde t_i, \tilde t_i+ \tilde T_i] \subseteq [t_i, t_i + T_i]$ such that we know the number of reports in that interval, and that $\tilde t_i, \tilde t_i+ \tilde T_i$ are stopping times. 

% Appendix \Cref{fig:observation_gen} summarizes the design of a valid observation period in our setting.

%5. How does this result help us?
%a. We have such a \tilde t_i --- since we have the time of the first report.

The best choice for $\tilde t_i$ is the (observed) time of the first report, and so we count all reports after the first report and before our chosen end time $\tilde t_i + \tilde T_i$---this time is the earliest that we know the incident exists, and so it maximizes the interval length. This choice formalizes the idea that our method uses the first report to condition on an incident exists (and a time for it), and then other reports to identify the reporting rate.


% \nikhil{I think should emphasize this more, currently we emphasize the stopping time more than this time}

%b. How do we get a reasonable \tilde T_i…

Setting $\tilde T_i$ is a design choice. We require that the end time $\tilde t_i+ \tilde T_i$ is a stopping time, and that $\tilde t_i+ \tilde T_i \leq t_i + T_i$, i.e., that we do not extend the interval past when the incident can no longer be reported. Choosing too high a duration $\tilde T_i$ risks under-estimating $\lambda(\cdot)$; unfortunately, $t_i + T_i$ is unobserved and so the condition cannot be directly verified. On the other hand, choosing too low a duration $\tilde T_i$ throws away data, increasing variance.

In our empirical application in \Cref{sec:datapplication}, we leverage 311 \textit{agency response} data, detailing when each incident was inspected or worked on. We choose the minimum of this time and $\tilde t_i + \bar T$, where $\bar T$ is a maximum duration design choice; we validate our estimates with multiple choices of $\bar T$. Note that this choice is a stopping time (as opposed to the time of the last report, as discussed above).

Once we have the interval and the number of reports in it, we can leverage \Cref{thm:stoppingtimes} to convert our setting into a standard Poisson rate estimation task, for which a large literature exists (and, for example, calculate the MLE for an homogeneous $\lambda$ for each type $\theta$). However, that does not mean that the estimation is computationally or statistically tractable. In particular, up to now we have assumed a \textit{fixed} type $\theta$, and thus a fixed rate function $\lambda_\theta(\cdot)$. In our setting, $\theta$ is high-dimensional, but incidents of similar types may have similar rates. In the next sub-section, we present a tractable Bayesian Poisson regression approach -- with various specifications for $\lambda_\theta(\tau)$ -- that we will apply in our application.

\FloatBarrier

% In particular, note that \Cref{eq:poissonnonhom} has, in the integral interval, the (unknown) birth time $t_i$. Depending on how we specify the age-dependence of $\lambda(\cdot)$, estimating the rate parameters may require latent variables $\{t_i\}$.

%\nikhil{talk about needing to know birth time in the poisson inhomogeneous case, which is not known. language below already talks about high dimensional}

%Theorem \ref{MLE} establishes an easy analytical way to estimate the reporting rate for each type of incidents, assuming homogenous reporting. In section \ref{simulation}, we demonstrate that when homogenous reporting is indeed the case and the number of types of incident is relatively small, this naive method actually works well.

%However, there are two critical weaknesses in this naive method. First, it does not extend easily to the more general non-homogenous reporting scenario, which is a more natural reflection of the reporting behavior. Second, when the dimensionality of incident type $\theta$ becomes large, we are often left with an extremely small number of reports in each type, which results in large variance of the estimator. These concerns call for the addition of machine learning approaches in estimating reporting rate.





%\todo{Nikhil rewriting below this (see tex comments for outline of this ``paragraph'')}

%This technique is : the number of reports \textit{for each given incident} identifies the reporting rate from the incident occurrence rate. If we know the birth and death times, then, one can directly apply the methods from missing species literature \nikhil{cite them...actually not sure what this claim means}.

%Our work points at what is missing in most existing literature: the use of duplicate data. Next we demonstrate the power of the duplicates with a naive version of the model \nikhil{maybe not naive...} and a surprisingly simple estimation method.



%  \nikhil{discussion on this eliminating the dependence on $\Lambda$ -- separating incidents from how often. that's the missing species connection. Need to call it a "first" insight}


%The additional challenge is that
%\todo{Below language moved from above...not sure where to put parts of this, or if need any of it? likely will comment out everything below this until the next paragraph}
%; we will use this additional data to estimate a duration $(t_i, t_i + \tilde T_i)$ during which each incident is alive.
%It follows that for an incident $i$ that occurred at time $t_i$, the expected number of reports $M_i(\tau)$ by time $t_i + \tau$  is $\bbE[M_i(\tau)] = \int_{\tau = t_i}^{t_i + \tau} \lambda_\theta(\tau - t_i) dp$.
% We assume that for an incident occurred at $t_i$, it `dies' at some point $t_i+T_i$, at which point reports about it stop coming in.
%The city does not observe incident time $t_i$ and so cannot directly estimate the reporting rate $\lambda(\tau)$ for $\tau$ less than the time of the first \textit{report} for incident $i$.

%For example, below we prove theoretical results about the following birth-death reporting process, though the empirical analysis is more general \nikhil{language -- I think some rewriting here around how insight is that lambda relates before and after first report, but exact relationship depends on various data generating process assumptions; theoretical results with some assumption, empirical with others}.
%
%Suppose an incident occurs (is `born') at time $t_i$, after which reports start being submitted according to a homogeneous process with rate $\lambda_\theta$.
%Then, as long as $T_i$ is a stopping time (i.e., not dependent on the future, just the realization of the reports up to that time), then $M_i(T_i)$ follows a Poisson distribution with parameter $T_i\lambda_\theta$.
% Reporting horizon $T$ is assumed to be exponentially distribution with mean $\frac{1}{\mu}$, independentally and identically distributed across all incidents. \nikhil{just make this known death time}
%\nikhil{writing?} In the next section, we first detail this identification challenge; then, in \Cref{sec:poissonreg}, we show how to transform our setting to a standard Poisson regression task, which helps us overcome the high-dimensional nature of our problem, where the number of reports is small compared to the dimensionality of $\theta$.


%The central challenge to identifiability is that we do not observe incident birth times $t_i$ or death times $t_i + T_i$---the time of each report . If we observed these values,
%In this subsection, we enumerate under which despite not observing $t_i$ and $T_i$, laying the ground work for our empirical estimation approach.


% Our method follows from the following observations under our model. First, due to the memory-less property of Poisson distributions, the number of reports \textit{after} the first report also follows a Poisson distribution---and we know the first report time, $\tilde t_i \triangleq t_i + t_i^0$, even though we do not know either $t_i$ or $t_i^0$.




% Second, while we do not directly observe death time $t_i + T_i$, we do not need to. Given $\tilde t_i$ (known), we only require knowledge of a time $\tilde t_i + \tilde T_i$, where $\tilde t_i + \tilde T_i \leq t_i + T_i$ and -- crucially -- $\tilde T_i$ is independent of $\lambda_\theta$ given the reports before time $t_i + \tilde T_i$; in other words, $\tilde T_i$ is a stopping time. \nikhil{more discussion here, what this means practically...how can estimate $\tilde T_i$, sensitivity to it, why it doesn't hold otherwise...for theorem to make sense in terms of why we're including it, would have to make stopping times a big deal here}




%\nikhil{older langauge} For this purpose, let us assume that the reporting rate of type $\theta$ incidents is homogeneous, that is $\lambda_\theta(\tau) \equiv \lambda_\theta, \tau \in [0,\infty)$. We further assume the death time of any incident is defined as a stopping time , and that its distribution is independent of the reporting process, conditional on the number of reports already logged. The next Theorem shows that in this case, we have an easy way of giving a point estimate for $\lambda_\theta$:

%\nikhil{Should emphasize the ``hard'' part of this theorem -- even if $T_i$ is a stopping time. Otherwise it's just a poisson distribution}

%\todo{new theorem statement and proof -- time inhomogeneous, notation 2/7, etc}




%\nikhil{proof intuition}

%\nikhil{write the exceptions around this --- when does it fail, and why? e.g., when confounding in $T_i$, i.e., not a stopping time}




% \zhi{problem: the current ML method using the first report time as the start of the exposure, will this be a problem for the non-homogeneous setting? that potentially different incidents have different $\lambda_\theta(t_i)$; propose a method to overcome this}

==> subsections/2_machinelearningapproach.tex <==
\subsection{Bayesian Poisson Regression approach}
\label{sec:poissonreg}

Above, we show how to transform our setting into a standard Poisson rate estimation task. Here we assume that we have a dataset of incidents $i$ with types $\theta(i)$, where for each incident we observe an interval $(\tilde t_i, \tilde T_i]$ and the number of reports in that interval $\tilde M_i$.
%
We develop a Bayesian Poisson regression approach to estimate using our data. For each of our various model specifications, we describe `reasonable' data generating processes that would lead to such a specification.

Our choices are not exhaustive; other specifications may also be appropriate, preferable in various dimensions, or correspond to more realistic data generating processes; the empirical strategy developed in \Cref{sec:convertingtopoissonregression} allows a large Poisson rate estimation literature (spatial, time-dependent, feature-dependent, etc)  to be applied, off-the-shelf. Our approaches here are chosen for simplicity in model interpretation; however, as we discuss in \Cref{sec:datapplication}, the observed vs predicted data distributions suggest further improvements if the goal is predicting reporting rates.

First, we assume a dependence on how the reporting rate is affected by the type $\theta$. For each of these models, we have a base reporting rate $\lambda_\theta$, defined as:
\begin{equation}
\lambda_\theta = \exp\left(\alpha + \beta^T\theta\right), \label{eqn:lambdaregressionassumption}
\end{equation}
where $\beta$ is a coefficient vector of appropriate dimension, and $(\alpha, \beta)$ are coefficients to be estimated. All other rate parameters are shared across types $\theta$, providing statistical efficiency and easing analysis of how various type characteristics affect the reporting rate. %The covariates that compose $\theta$, as well as Bayesian priors, differ between model runs, and are discussed in \Cref{sec:simulation} and \Cref{sec:datapplication}.


\paragraph{Standard homogeneous Poisson regression} Our first specification is a standard homogeneous Poisson regression, where $\lambda_\theta(\tau) = \lambda_\theta$, for all $\tau$. Then, for each $i$, we have $\tilde M_i \sim \text{Poisson}\left(\tilde T_i\lambda_{\theta(i)} \right)$, where $\theta(i)$ is the type of incident $i$. This specification corresponds to the naive data generating process in which many residents independently encounter alive incidents and report them.

\paragraph{Zero-inflated Poisson regression} Next, we use a zero-inflated Poisson regression \cite{lambert1992zero}, in which $\lambda_\theta(\tau) = 0 $ with probability $\gamma$, and $\lambda_\theta$ otherwise, independently sampled for each incident.\footnote{While \Cref{thm:stoppingtimes} is proven for a deterministic rate $\lambda_\theta$ (conditioned on type $\theta$), it is easy to see that the analogous result extends for the Zero-inflated model, as long as the stopping times are independent of $\gamma$, given the sample path and type $\theta$. With a fixed $\gamma$ (or fixed given types $\theta$), this condition trivially holds.} Then, for each $i$, we have $\tilde M_i \sim \text{Bernoulli}(1 - \gamma)\times\text{Poisson}\left(\tilde T_i\lambda_{\theta(i)} \right)$.

Recall that, as discussed in \Cref{sec:convertingtopoissonregression}, $\tilde M_i$ is the number of reports \textit{after} the first report (up until the observation end time); thus, this specification corresponds to a data generating process in which for a fraction $\gamma$ of incidents, only one report is generated. For example, perhaps those incidents are personal requests for service (i.e., to plant a tree somewhere or to prune a tree to enable certain construction), for which duplicates are unlikely; alternatively, the Parks department may physically mark trees as ``report received; full inspection pending,'' preventing future reports.\footnote{A natural extension would be to also allow $\gamma$ to depend on $\theta$.} Such a model is typically used when one observes more zeros than would be expected from a Poisson distribution, as in our case.

\medskip As detailed in \Cref{sec:datapplication}, these two models reasonably match the observed distribution of the number of reports received in the observation period, except that the \textit{Basic} model under-estimates the number of incidents with zero reports $\tilde M_i = 0$, and the zero-inflated model over-estimates the number of incidents with large $\tilde M_i$. Such patterns suggest that a time non-homogeneous Poisson process (with decreasing rates with incident age) may be appropriate. Below, we describe one such process and the challenge in estimating it.

\paragraph{Non-homogeneous Poisson regression} Suppose the reporting rate is $\lambda_\theta(0)=\lambda_\theta$ at birth but changes with incident age. The challenge with non-homogeneous reporting rates with our data (beyond the standard statistical efficiency challenges to estimating such rates) is that our observation period does not start at incident age $\tau = 0$, but rather at the (unknown) age when the first report occurred, $\tau = \tilde t_i - t_i$. For example, suppose the reporting rate decreases exponentially with incident age: $\lambda_\theta(\tau) = \lambda_\theta\exp(-\gamma \tau)$, where $\gamma\ge 0$. Then, the Poisson likelihood in \Cref{eq:poissonnonhom} corresponds to
\begin{align*}
	\tilde M_i&\sim \text{Poisson}\left(\frac{\lambda_\theta}{\gamma}e^{-(\tilde t_i - t_i)}\left[1 - e^{-\tilde T_i}\right]\right),
\end{align*}
where $(\tilde t_i - t_i)$ is a per-incident unknown latent variable; if just the number of reports $\tilde M_i$ is used as data, there are more unknown model parameters than data points. However, note that in 311 systems, the data also typically include time-stamps for each incident, using which we can calculate report inter-arrival times -- using these times would lead to more data points than parameters, but both would still be on the order of the number of incidents. Such latent variable Bayesian non-homogeneous Poisson processes are considered in the marketing literature with ``buy till you die'' models \cite{abe_counting_2008}, where an unknown parameter for whether a  customer has left the system must be estimated; it is possible that time-reversed versions of such models can be adapted to this setting -- it is a strength of our analysis in \Cref{sec:convertingtopoissonregression} that such a connection is possible.

In this work, we apply the \textbf{basic} and \textbf{zero-inflated} Poisson regression approaches to our data.


%\todo{finish writing this section}

%In the case where $\gamma=0$, it becomes the homogenous reporting rate setting.

%\nikhil{need to edit below}


%We can extend our model into a Poisson regression model with offset $T_i-t_i$, that is:
%$$
%M_i-1\sim \text{Poisson}\left(\exp\left(\alpha + \beta^T\theta+\log(T_i-t_i)\right)\right)
%$$
%Thus the task of examining variation of $\lambda_\theta$ with $\theta$ has now been transformed into the estimation of $\beta$ and potentially $\alpha$.

%Traditional Poisson regression method introduce the offset term $\log(T_i-t_i)$ to account for the difference in exposure of each individual event. However, in our setting, when we relax the homogeneity assumption, this approach is flawed. Recall that under non-homogenous reporting, we assume $\lambda_\theta(\tau)$ as the reporting rate of an incident of type $\theta$ when it is aged $\tau$. When we first observe a report of an incident, we do not know its age, thus we cannot determine its reporting rate as a function of $\tau$. To derive a way round this issue, we enforce the following assumption.

%\begin{assumption}\label{exprep}
%
%\end{assumption}

%Under assumption \ref{exprep}, the reporting rate for an incident aged $\tau$ becomes
%$$
%\lambda_\theta(\tau) = \exp\left(\alpha + \beta^T\theta - \gamma\tau\right), \tau \ge 0
%$$

%Now let us suppose for each observed incident $i$, their true birth time is an unobserved random variable $x_i$. Thus for any time $t$ between $t_i$ and $T_i$, the reporting rate dependent on $x_i$ is
%$$
%\lambda_\theta(t) = \exp\left(\alpha + \beta^T\theta - \gamma(t-x_i)\right), t_i\le t\le T_i
%$$
%and the distribution of the number of duplicates, dependent on the true birth time is
%\begin{align*}
%	M_i-1&\sim \text{Poisson}\left(\int_{t_i}^{T_i} \lambda_\theta(t) dt\right)\\
%	&=\text{Poisson}\left(\exp\left(\alpha +\beta^T\theta-\log\gamma -\gamma x_i\right)\left[\exp(-\gamma t_i)-\exp(-\gamma T_i)\right]\right)
%\end{align*}


%Finally, we use the following non-homogeneous specification: for each $i$ at age $\tau$, $\lambda_{\theta(i)}(\tau) = \lambda_{\theta(i)} \times h\left(\tau - (\tilde t_i - t_i)\right)$, where $h(x)$ is such that,\footnote{In other words, $h(x) = \gamma \tau ^ {\gamma - 1}$, defined only for $x > 0$, and so $\lambda_{\theta(i)}(\tau)$ is only defined for $\tau > (\tilde t_i - t_i)$.}
%\begin{align*}
%\tilde M_i &\sim \text{Poisson}\left(\lambda_{\theta(i)}\tilde T_i^\gamma \right).
%\end{align*}
%where $h(\tau) = \tau^{\gamma}$. Then,
%\begin{align*}
%	\tilde M_i &\sim \text{Poisson}\left(\int_{\tau = \tilde t_i - t_i}^{(\tilde t_i - t_i) + \tilde T_i } \lambda_{\theta(i)}h\left(\tau - (\tilde t_i - t_i)\right)d\tau \right)
%	\iff \tilde M_i \sim \text{Poisson}\left(\lambda_{\theta(i)}\int_{\tau = 0}^{\tilde T_i } \tau^\gamma d\tau \right).
%\end{align*} \todo{not true...actually the function needs to be uglier, to correspond to T to the gamma, which is what we actually learned.}


%\todo{not true...actually the function needs to be uglier, to correspond to T to the gamma, which is what we actually learned.}
%\nikhil{caveat that this is not that well-defined...}\nikhil{Not sure there's a natural one...meant to approximate...}






%\todo{Old language below, need to move/remove}

%In this subsection, we first propose a Poisson regression approach to overcome the high-dimensionality issue.

% We then introduce a slight change in the method to accommodate time-varying reporting rate.

%We begin by maintaining the assumption that the reporting rate is homogeneous. Recalling that our main goal in this work is to uncover the dependence of reporting rate $\lambda_\theta$ on the incident type $\theta$, and that we have established for all incidents $i$ in type $\theta$, the number of duplicates we observe about them follows a Poisson distribution $M_i-1\sim \text{Poisson}(\lambda_\theta(T_i-t_i))$ \nikhil{should be more explicit in previous subsection}, a natural way to model this is through \textit{Poisson regression}.

% We can extend our model into a Poisson regression model with offset $T_i-t_i$, that is:
%$$
%M_i-1\sim \text{Poisson}\left(\exp\left(\alpha + \beta^T\theta+\log(T_i-t_i)\right)\right)
%$$
%
%Thus the task of examining variation of $\lambda_\theta$ with $\theta$ has now been transformed into the estimation of $\beta$ and potentially $\alpha$.
%
%Traditional Poisson regression method introduce the offset term $\log(T_i-t_i)$ to account for the difference in exposure of each individual event. However, in our setting, when we relax the homogeneity assumption, this approach is flawed. Recall that under non-homogenous reporting, we assume $\lambda_\theta(\tau)$ as the reporting rate of an incident of type $\theta$ when it is aged $\tau$. When we first observe a report of an incident, we do not know its age, thus we cannot determine its reporting rate as a function of $\tau$. To derive a way round this issue, we enforce the following assumption.

% \begin{assumption}\label{exprep}
% The non-homogenous reporting rate is exponentially decreasing with the age of the incident. I.e., suppose at birth, the reporting rate is $\lambda_\theta(0)=\lambda_\theta$, then when the incident is aged $\tau\ge 0$, the reporting rate becomes
% $$
% \lambda_\theta(\tau) = \lambda_\theta\tau^{-\gamma}
% $$
% where $0\le \gamma <1$. In the case where $\gamma=0$, it becomes the homogenous reporting rate setting.
% \end{assumption}

% Under assumption \ref{exprep}, the reporting rate for an incident aged $\tau$ becomes
% $$
% \lambda_\theta(\tau) = \exp\left(\alpha + \beta^T\theta - \gamma\log(\tau)\right), \tau \ge 0
% $$

% Now let us suppose for each observed incident $i$, their true birth time is an unobserved random variable $\tau_i$. Thus for any time between $t_i$ and $T_i$, the reporting rate dependent on $\tau_i$ is
% $$
% \lambda_\theta(t) = \exp\left(\alpha + \beta^T\theta - \gamma\log(t-\tau_i)\right), t_i\le t\le T_i
% $$
% and the distribution of the number of duplicates, dependent on the true birth time is
% $$
% M_i-1\sim \text{Poisson}\left(\int_{t_i}^{T_i} \lambda_\theta(t) dt\right)=\text{Poisson}\left(
% $$

%\begin{assumption}\label{exprep}
%Suppose at birth, the reporting rate is $\lambda_\theta(0)=\lambda_\theta$. The non-homogenous reporting rate is decreasing with the age of the incident $\tau\ge 0$ according to
%$$
%\lambda_\theta(\tau) = \lambda_\theta\exp(-\gamma \tau)
%$$
%where $\gamma\ge 0$. In the case where $\gamma=0$, it becomes the homogenous reporting rate setting.
%\end{assumption}
%
%Under assumption \ref{exprep}, the reporting rate for an incident aged $\tau$ becomes
%$$
%\lambda_\theta(\tau) = \exp\left(\alpha + \beta^T\theta - \gamma\tau\right), \tau \ge 0
%$$
%
%Now let us suppose for each observed incident $i$, their true birth time is an unobserved random variable $x_i$. Thus for any time $t$ between $t_i$ and $T_i$, the reporting rate dependent on $x_i$ is
%$$
%\lambda_\theta(t) = \exp\left(\alpha + \beta^T\theta - \gamma(t-x_i)\right), t_i\le t\le T_i
%$$
%and the distribution of the number of duplicates, dependent on the true birth time is
%\begin{align*}
%    M_i-1&\sim \text{Poisson}\left(\int_{t_i}^{T_i} \lambda_\theta(t) dt\right)\\
%    &=\text{Poisson}\left(\exp\left(\alpha +\beta^T\theta-\log\gamma -\gamma x_i\right)\left[\exp(-\gamma t_i)-\exp(-\gamma T_i)\right]\right)
%\end{align*}





==> subsections/2_machinelearningapproach_short.tex <==
\subsection{Bayesian Poisson Regression approach}
\label{sec:poissonreg}

Above, we show how to transform our setting into a standard Poisson rate estimation task. Here we assume that we have a dataset of incidents $i$ with types $\theta(i)$, where for each incident we observe an interval $(\tilde t_i, \tilde T_i]$ and the number of reports in that interval $\tilde M_i$.
%
We develop a Bayesian Poisson regression approach to estimate using our data. For each of our various model specifications, we describe `reasonable' data generating processes that would lead to such a specification.

Our choices are not exhaustive; other specifications may also be appropriate, preferable in various dimensions, or correspond to more realistic data generating processes; the empirical strategy developed in \Cref{sec:convertingtopoissonregression} allows a large Poisson rate estimation literature (spatial, time-dependent, feature-dependent, etc)  to be applied, off-the-shelf. Our approaches here are chosen for simplicity in model interpretation; however, as we discuss in \Cref{sec:datapplication}, the observed vs predicted data distributions suggest further improvements if the goal is predicting reporting rates.

First, we assume a dependence on how the reporting rate is affected by the type $\theta$. For each of these models, we have a base reporting rate $\lambda_\theta$, defined as:
\begin{equation}
\lambda_\theta = \exp\left(\alpha + \beta^T\theta\right), \label{eqn:lambdaregressionassumption}
\end{equation}
where $\beta$ is a coefficient vector of appropriate dimension, and $(\alpha, \beta)$ are coefficients to be estimated. All other rate parameters are shared across types $\theta$, providing statistical efficiency and easing analysis of how various type characteristics affect the reporting rate. %The covariates that compose $\theta$, as well as Bayesian priors, differ between model runs, and are discussed in \Cref{sec:simulation} and \Cref{sec:datapplication}.


\paragraph{Standard homogeneous Poisson regression} Our first specification is a standard homogeneous Poisson regression, where $\lambda_\theta(\tau) = \lambda_\theta$, for all $\tau$. Then, for each $i$, we have $\tilde M_i \sim \text{Poisson}\left(\tilde T_i\lambda_{\theta(i)} \right)$, where $\theta(i)$ is the type of incident $i$. This specification corresponds to the naive data generating process in which many residents independently encounter alive incidents and report them.

\paragraph{Zero-inflated Poisson regression} Next, we use a zero-inflated Poisson regression \cite{lambert1992zero}, in which $\lambda_\theta(\tau) = 0 $ with probability $\gamma$, and $\lambda_\theta$ otherwise, independently sampled for each incident.\footnote{While \Cref{thm:stoppingtimes} is proven for a deterministic rate $\lambda_\theta$ (conditioned on type $\theta$), it is easy to see that the analogous result extends for the Zero-inflated model, as long as the stopping times are independent of $\gamma$, given the sample path and type $\theta$. With a fixed $\gamma$ (or fixed given types $\theta$), this condition trivially holds.} Then, for each $i$, we have $\tilde M_i \sim \text{Bernoulli}(1 - \gamma)\times\text{Poisson}\left(\tilde T_i\lambda_{\theta(i)} \right)$.

Recall that, as discussed in \Cref{sec:convertingtopoissonregression}, $\tilde M_i$ is the number of reports \textit{after} the first report (up until the observation end time); thus, this specification corresponds to a data generating process in which for a fraction $\gamma$ of incidents, only one report is generated. For example, perhaps those incidents are personal requests for service (i.e., to plant a tree somewhere or to prune a tree to enable certain construction), for which duplicates are unlikely; alternatively, the Parks department may physically mark trees as ``report received; full inspection pending,'' preventing future reports.\footnote{A natural extension would be to also allow $\gamma$ to depend on $\theta$.} Such a model is typically used when one observes more zeros than would be expected from a Poisson distribution, as in our case.

\medskip As detailed in \Cref{sec:datapplication}, these two models reasonably match the observed distribution of the number of reports received in the observation period, except that the \textit{Basic} model under-estimates the number of incidents with zero reports $\tilde M_i = 0$, and the zero-inflated model over-estimates the number of incidents with large $\tilde M_i$. Such patterns suggest that a time non-homogeneous Poisson process (with decreasing rates with incident age) may be an appropriate extension. The estimation of such processes involve fitting a per-incident latent parameter that is the age of the incident when the first report occurred. Analogies of such processes have been considered in the marketing literature, e.g. \citep{abe_counting_2008}, and it is a strength of our analysis in \Cref{sec:convertingtopoissonregression} that such a connection is possible. We leave this as an extension due to the technical difficulties introduced by the need to estimate parameters whose number are on the magnitude of samples, and the scope of this paper.

% \paragraph{Non-homogeneous Poisson regression} Suppose the reporting rate is $\lambda_\theta(0)=\lambda_\theta$ at birth but changes with incident age. The challenge with non-homogeneous reporting rates with our data (beyond the standard statistical efficiency challenges to estimating such rates) is that our observation period does not start at incident age $\tau = 0$, but rather at the (unknown) age when the first report occurred, $\tau = \tilde t_i - t_i$. For example, suppose the reporting rate decreases exponentially with incident age: $\lambda_\theta(\tau) = \lambda_\theta\exp(-\gamma \tau)$, where $\gamma\ge 0$. Then, the Poisson likelihood in \Cref{eq:poissonnonhom} corresponds to
% \begin{align*}
% 	\tilde M_i&\sim \text{Poisson}\left(\frac{\lambda_\theta}{\gamma}e^{-(\tilde t_i - t_i)}\left[1 - e^{-\tilde T_i}\right]\right),
% \end{align*}
% where $(\tilde t_i - t_i)$ is a per-incident unknown latent variable; if just the number of reports $\tilde M_i$ is used as data, there are more unknown model parameters than data points. However, note that in 311 systems, the data also typically include time-stamps for each incident, using which we can calculate report inter-arrival times -- using these times would lead to more data points than parameters, but both would still be on the order of the number of incidents. Such latent variable Bayesian non-homogeneous Poisson processes are considered in the marketing literature with ``buy till you die'' models \cite{abe_counting_2008}, where an unknown parameter for whether a  customer has left the system must be estimated; it is possible that time-reversed versions of such models can be adapted to this setting -- it is a strength of our analysis in \Cref{sec:convertingtopoissonregression} that such a connection is possible.

In this work, we apply the \textbf{basic} and \textbf{zero-inflated} Poisson regression approaches to our data.



==> subsections/4_applying_to_data.tex <==
\label{sec:datapplication}

\input{plots/tab_summary_stats}
This section applies our methods to data from the NYC Department and Parks and Recreation.

\subsection{Problem setting, dataset and pre-processing}

Our data is composed of partially public data,\footnote{The publicly available part is here: \url{https://data.cityofnewyork.us/Environment/Forestry-Service-Requests/mu46-p9is/data}. The NYC DPR additionally provided us with internal data on inspection and work order outcomes and hashed, anonymized identifiers for the caller's name, email, and phone number, if provided by the caller.} from the NYC Department of Parks and Recreation (DPR). It contains \num{214553} service requests made by the public in a 3-year period between 2017/06/30 and 2020/06/30 about street trees. For each request, we have location and incident-specific covariates. We further observe whether the service request led to an inspection (a DPR inspector attempting to find and evaluate the issue), the outcome of the inspection (e.g., an assessment of the risk the problem poses), and what type of work order was created (if any). For each event, we further observe time stamps. Crucially, for inspected requests (65\%), the DPR marks which other requests refer to the same incident. See \Cref{tab:Summary} for summary statistics.

%\nikhil{not sure where this text} A service request may be marked closed either because it is deemed insignificant or because an inspection is performed, and potentially other subsequent measures such as a work orders are put into place. When an inspection is performed and found that multiple service requests turn out to be pointing at the same incident, they are labeled duplicate reports. For each inspection, we have the date it is conducted and the outcome of the inspection.

\subsubsection{Two potential sources of bias}

There are two potential sources of bias, due to ways in which the data differs from the model assumed in \Cref{sec:model}. Here, we evaluate these concerns, and conclude that they likely do not substantially affect our measurements.

% We are primarily focusing on these service requests, since these are the ones that are inherently decided to be of more significance by the parks department, and we can determine whether they are duplicate reports on the same incident.

\paragraph{Repeat callers about the same incident.} One potential worry is that duplicate reports are a mirage: that they are primarily generated by the same resident repeatedly calling about an incident until it is addressed. If that is the case, our method does not work: we rely on a Poisson rate assumption for the reporting behavior (that reporting behavior is memory-less and so that one report does not affect the likelihood of another for that incident), which is likely violated if the same person makes multiple reports about the same incident. In theory, such repeats should be minimal: NYC makes available a portal to check the status of past reports, and so a reporter does not need to call again to remain up-to-date. In practice, however, our contacts at DPR indicated that repeat calls occur.

To mitigate the effect of such repeat callers on our analysis, we obtain anonymized (hashed) caller information from DPR for each report: if the caller provided it, their name, phone number, and/or email address. We then filter out the duplicate reports for each incident where either the phone number or emails match, or both the first and last names match. Our analyses are run on the resulting filtered dataset.
%
The above approach may not filter out all repeat callers: if callers choose not to leave their information, but call multiple times. Thus, we also run our main analyses on a filtered dataset where we additionally assume that any caller who did not leave their information is a repeat of a previous caller with no information. Our estimates are largely the same on this more conservative dataset, suggesting that repeat callers do not substantially bias our estimates.


%Another concern for the anomalies in the dataset is that there may be \textit{repeat callers} for the same incident, in which case the reports are clearly not generated independently, violating our model assumptions.

%To eliminate this concern as much as possible,  This is a somewhat moderate approach to eliminating repeat callers as opposed to the most conservative way of filtering out duplicate reports where any field matches. The reason behind this choice is that we find the most conservative approach results in an aggregated dataset that yields largely the same conclusions, but with a higher level of noise. In the interest of retaining more information in the dataset, we chose this moderate approach.

%\todo{if have time, potentially include histograms of reports for different repeat caller methods}



\paragraph{Censored data: incidents that were not inspected}
\input{subsections/inspection_discussion}



\subsubsection{Creating an aggregated incident dataset.}
 \begin{figure}[tb]
	\centering
	%	\begin{subfigure}{.5\textwidth}
	% 		\centering
	\subfloat[][Number of reports per incident.]{
		\includegraphics[width=.45\textwidth]{plots/NumberReports_hist}
		% 		\caption{Census tract fixed effects}
		\label{fig:numreportshist}
		% 		\end{subfigure}
	}
	\hfill
	\subfloat[][Length of observation period.]{
		\includegraphics[width=.45\textwidth]{plots/Duration_hist}
		% 		\caption{Census tract fixed effects}
		\label{fig:durationhist}
		% 		\end{subfigure}
	}
	\caption{Distribution of number of reports and length of observation for each unique incident in the aggregated dataset. For most incidents, there are no reports after the first report (at least not in the observation period). There is a peak at 100 days for the observation period, due to our configuration in \Cref{eq:duration}, where we truncate longer periods to 100 days.}
\end{figure}




Before training models, we need to construct a dataset in which each row corresponds to an incident, and where we have the number of reports $\tilde M_i$ in an observation interval, the duration $\tilde T_i$ of that interval, and covariates $\theta$. We separated out an exploratory dataset of 8000 unique incidents, on which we conducted covariate selection as detailed below.\footnote{While the exploratory data was used to filter variables for ultimate analysis, and to develop and fine-tune our models, we note that we did not hold out a separate test set at the outset of the project; it was not clear how to cluster assign reports to test and train before developing our empirical strategy, and there were initial (ultimately resolved) data errors on how reports were tagged to unique incidents. Thus, our overall approach was selected and developed using the data on which we ultimately report results, and so it may be useful to acquire more recent data from DPR and verify our findings. The exploratory dataset was ultimately composed of 4463 unique incidents, after the filtering as described below.}


We filter out the reports corresponding to the uninspected service requests (as discussed above, we do not have duplicate information for these), and then use the provided incident label to group all service requests for the same incident. Then, we remove repeat caller reports as described above, comparing each caller to previous (ordered by time) callers for the same incident. Next, we must construct a valid observation interval for each incident.


%To create an aggregated dataset workable for our empirical methods, we focus on the information observed for each unique incident.

\paragraph{Constructing an observation interval $(\tilde t_i, \tilde t_i + \tilde T_i]$} As outlined in \Cref{thm:stoppingtimes}, we must be careful in how we choose an observation interval $(\tilde t_i, \tilde t_i + \tilde T_i]$ in which we count reports -- we need that the interval is inside the incident lifetime, i.e., we must end the interval before the incident is addressed, $\tilde t_i + \tilde T_i \leq t_i + T_i$. Both endpoints of the interval must also be stopping times, i.e., not use information from the future. As discussed above, the natural choice to start the observation period $\tilde t_i$ is the time of the first report, but choosing the observation end is a design choice.

We make the following choice. Let $t_i^{\text{INSP}}$ be the inspection time of incident $i$, and, $t_i^{\text{WO}}$ be the time that a work order is placed for incident $i$, if applicable. Then, $\tilde{T}_i$ of each incident $i$ is:
\begin{equation}
	\tilde{T}_i = \min \left\{100\text{ days},\  t_i^{\text{INSP}} - \tilde{t}_i,\  t_i^{\text{WO}} - \tilde{t}_i\right\}. 	\label{eq:duration}
\end{equation}
The maximum duration 100 is a design choice, for which we perform robustness checks (with 30 and 200 days); a maximum mitigates -- for incidents not inspected for a long time -- the inclusion of a time period in which an issue might have been resolved before an inspection, which would bias our estimates downward. \Cref{eq:duration} requires that inspection and work order times are stopping times; that they do not depend on the future trivially holds, and it is likely that they do not depend on the reporting {rate} except through the type $\theta$ and the sample path number of reports received up to that time. (It is not a problem that incidents with more reports are inspected sooner).

\vspace{1em}

\noindent \Cref{fig:numreportshist} shows the histogram of the number of reports per incident during the observation interval; \Cref{fig:durationhist} shows the distribution of durations; and \Cref{tab:Summary} shows how the average duration differs by Borough and report category. The heterogeneity in duration length (due to the speed of being inspected or worked on) demonstrates the value of \Cref{thm:stoppingtimes}.  For example, compared to `Prune' incidents, `Hazard' incidents tend to have more reports on average and shorter duration: residents have a higher reporting rate for hazardous incidents, and these incidents tend to be addressed more quickly. Suppose we had to use a fixed duration $D$, instead of an inspection/work order dependent time. If $D$ is large (e.g., $D \approx 15$ days), then we bias our estimates downward, as we're including time periods after an incident has already been addressed -- and the bias heterogeneously affects incident types, since some incidents are addressed sooner. On the other hand, a much shorter duration would substantially limit the data. Finally, Appendix \Cref{fig:daysfirstcomplaint} shows the average number of days after the first report that the $\ell$th duplicate report was submitted for an incident, for incidents with at least $k \geq \ell$ reports. The plots are largely linear (i.e., the average delay between the first and second report is the same as that between the third and forth report), consistent with reporting rates being homogeneous Poisson within the interval.



%Note that in practice, though inspection and work orders may depend on the number of reports that one incident receives, conditional on the number of reports an incident has received, the inspection time and work order placed time are typically independent on the reporting process, and only depend on the inspection personnel or the scheduling system for such inspection, thus $\tilde{t}_i+\tilde{T}_i$ satisfies our assumption in Theorem \ref{thm:stoppingtimes}.

%The benefit of such setting is that we are able to avoid anomalies created by human error where, for example, the inspection time is incorrectly logged.


%Even from these crude summary statistics, we are able to make some interesting observations.Our setting which uses stopping times as death times comes in handy here, as if using stopping times was not an option, we would have to use a fixed observation duration instead of a minimum of inspection time, work order time and some fixed value. In other words, using stopping times helps us bring out the variation of incidents in the data, which in turn helps with the estimation and recognition of heterogeneity.  These benefits all result from the use of stopping times as the hallmarks of the observation period, as established by \Cref{thm:stoppingtimes}.



\paragraph{Covariate selection and processing} Next, we select the covariates that compose type $\theta$. The data given to us by DPR includes a set of \textit{report} covariates (e.g., report \textit{Category}),\footnote{Occaisonally, different reports about the same incident disagree on the report covariates. We select the first report characteristics in those cases.} \textit{inspection} results (e.g., condition of tree at inspection time), and \textit{tree} characteristics (e.g., diameter of tree at breast height, tree species). We augment this data with \textit{socio-economic characteristics} as follows. Our data contains latitude-longitude coordinates for each inspection (and thus incident), using which we identify which of the over 2000 census tracts in New York City the incident is in, through a FCC API.\footnote{FCC Area API, https://geo.fcc.gov/api/census/} We then join this information with 2020 Census data obtained from the United States Census Bureau, which includes socio-economic characteristics such as race/ethnicity, education, income, and population density for each census tract. We are unable to match 9473 incidents to census tracts and discard them in our analysis.

Next, we perform covariate selection using the exploratory dataset. We remove report and inspection variables that are highly collinear, low variance, or with high number of missing values. Conversations with DPR also played a role in selection. %: for example, we include Borough fixed effects our analyses, as DPR indicated that each Borough has an agency sub-unit which handles requests---and so there might be differences in how different Boroughs conduct inspections.
Finally, we log transform several variables, and standardize all data. Appendix \Cref{tab:desc} contains the covariates we use.



%\nikhil{Covariate selection on exploratory dataset}  \nikhil{For example: how select from report characteristics}

%Then, we separate an exploratory and model development dataset, on which we do the following.



\smallskip

Starting with the dataset discussed above, we filter out the incidents for which any of the covariates are missing, those with short logged reporting periods (Duration less than 0.1 days), and those in the exploratory dataset. We are left with a dataset of $78151$ incidents on which we conduct our main analyses; for each incident $i$, we have the duration of observance $\tilde{T}_i$, the number of total reports $\tilde M_i$, and all the various geographic and demographic covariates associated with it.

% \zhi{do we want this in the appendix? do we want the unused here as well?}\nikhil{yes, move to appendix, current table fine}

% \input{plots/tab_covariates}


\subsection{Analyses, training, and evaluation}

We fit the models using Stan \citep{carpenter2017stan}, a Bayesian probabilistic programming language.

We use three sets of covariates. Every analysis includes our incident-specific covariates (inspection results, report \textit{Category}, tree size) and an intercept. Our \textbf{Base} analysis includes just these covariates along with \textit{Borough} level fixed effects. As the covariates are standardized, these coefficients all have a zero-mean Normal prior. \textit{Borough} and \textit{Category} are categorical variables; instead of dropping one level for each variable, to maintain identifiability we enforce a sum zero constraint\footnote{\url{https://mc-stan.org/docs/2_28/stan-users-guide/parameterizing-centered-vectors.html}} on their coefficients to ease interpretability. For the other categorical covariates, we drop one level each.
%%
%In our \textbf{Hierarchical Spatial} analysis, we additionally include coefficients for each of the (over 2000) census tracts, with hierarchically defined priors. Each \textit{Borough} coefficient is as above. Then, we set coefficients for the 59 \textit{Community Boards},\footnote{New York City is split into five Boroughs, and each Borough is further subdivided into Community Boards. Each Borough and Community Board maintains a level of local governance.} with prior means centered at the corresponding Borough coefficient; and, for each \textit{census tract}, we set coefficients with prior means centered at the corresponding\footnote{Our tract labels come from the FCC API on coordinates as described above, but Community Board labels are present in the data. Labeled census tracts may not be a sub-partition of community boards. In the rare case that a census tract belongs to multiple Community Boards, we select the most frequent Community Board associated with that tract in the data.} \textit{Community Board}.
%
In our \textbf{Spatial} analysis, we include coefficients for each of the (over 2000) census tracts. We use an Intrinsic Conditional Auto-Regressive (ICAR) model~\cite{morris2019bayesian} for the spatial coefficients, alongside the incident level coefficients. In such models, each census tract coefficient is assumed to be normally distributed with a mean equal to the average of its neighbors -- i.e., spatial smoothness is encoded into the model, and so census tracts with few incidents borrow information from neighboring census tracts.
%
Finally, in our \textbf{Socio-economic} analyses, we include each census \textit{socio-economic} covariate \textit{individually} with the incident-specific covariates (e.g., the regression with \textit{Median Age} contains as coefficients the base covariates, but not \textit{Fraction Hispanic}; this choice is due to the census covariates being highly collinear). These covariates are also standardized, and coefficients prior means are set to zero.

For the \textbf{Base} covariates, we fit both the \textbf{standard} and \textbf{zero-inflated} Poisson regressions, and evaluate model fit. Both models perform similarly in terms of overall predictive power, with Pearson correlations of $0.1335$ and $0.1248$, respectively, for the mean prediction for number of reports for each incident vs the observed number of reports. Next, we perform a standard check for Bayesian models: whether the posterior prediction distribution matches the observed data distribution, as a test for whether the model captures the underlying data generating process; Appendix \Cref{fig:posteriors} compares the distribution for each model specification. We observe that each model roughly matches the observed distribution, but differ in various ways. The \textbf{standard} Poisson Regression under-estimates the (large) fraction that $\tilde M_i = 0$, but more accurately captures the distribution tail. Inversely, the \textbf{zero-inflated} Poisson Regression matches the fraction for small $\tilde M_i$ (where the majority of the mass is), at the cost of mis-estimating the tail.

These results suggest that if the goal is to predict number of reports for each incident, then there are model improvements to be made (for example, by allowing the zero-inflation fraction to depend on incident type, or by allowing non-homogeneous reporting rates). However, to understand how $\lambda_\theta$ varies by incident type $\theta$, we prefer our simpler specification; for the analyses below, we primarily report results with the \textbf{zero-inflated} Poisson regressions, choosing it because it better matches the primary distribution mass. Results with the \textbf{standard} model are similar.
%\todo{still editing below this}


%\nikhil{, why include borough level fixed effects, etc.} \nikhil{Priors, spatial, etc}





% \paragraph{Generating incident dataset} \todo{everything to generate aggregate dataset from raw data here}


% \nikhil{talk about estimating $T_i = \min(100, inspection time or work order)$, such that it is a stopping time}


% \nikhil{discuss the columns used, normalizing the data}

% \nikhil{Removing duplicate callers}


%\paragraph{Models, training, and evaluation}


%The results are reported in the remaining data, with a total of 80374 unique incidents.



%\todo{mention that choice of theta, priors on those, can differ between models? Yes need a subsection for that}

%\nikhil{training models in stan, which models we ran}


%\nikhil{posterior predictive checks, other ways to check models} \nikhil{why went with zero inflated model here}

%0.1231 &      0.1354 & 0.6544

%\nikhil{discuss fit measures (posterior p value, fit plots, joint distribution, etc.), regression specification}

%\todo{Discuss 'overall' results, what the basic regression tells us not just about heterogeneity but in terms of reporting delay, what that means}



==> subsections/4_applying_to_data_short.tex <==
\label{sec:datapplication}

\input{plots/tab_summary_stats}
This section applies our methods to data from the NYC Department and Parks and Recreation.

\subsection{Problem setting, dataset and pre-processing}

Our data is composed of partially public data,\footnote{The publicly available part is here: \url{https://data.cityofnewyork.us/Environment/Forestry-Service-Requests/mu46-p9is/data}. The NYC DPR additionally provided us with internal data on inspection and work order outcomes and hashed, anonymized identifiers for the caller's name, email, and phone number, if provided by the caller.} from the NYC Department of Parks and Recreation (DPR). It contains \num{214553} service requests made by the public in a 3-year period between 2017/06/30 and 2020/06/30 about street trees. For each request, we have location and incident-specific covariates. We further observe whether the service request led to an inspection (a DPR inspector attempting to find and evaluate the issue), the outcome of the inspection (e.g., an assessment of the risk the problem poses), and what type of work order was created (if any). For each event, we further observe time stamps. Crucially, for inspected requests (65\%), the DPR marks which other requests refer to the same incident. See \Cref{tab:Summary} for summary statistics.

%\nikhil{not sure where this text} A service request may be marked closed either because it is deemed insignificant or because an inspection is performed, and potentially other subsequent measures such as a work orders are put into place. When an inspection is performed and found that multiple service requests turn out to be pointing at the same incident, they are labeled duplicate reports. For each inspection, we have the date it is conducted and the outcome of the inspection.

\subsubsection{Two potential sources of bias}

There are two potential sources of bias, due to ways in which the data differs from the model assumed in \Cref{sec:model}. Here, we evaluate these concerns, and conclude that they likely do not substantially affect our measurements.

% We are primarily focusing on these service requests, since these are the ones that are inherently decided to be of more significance by the parks department, and we can determine whether they are duplicate reports on the same incident.

\paragraph{Repeat callers about the same incident.} One potential worry is that duplicate reports are primarily generated by the same resident repeatedly calling about an incident until it is addressed. If that is the case, our method does not work: we rely on a Poisson rate assumption for the reporting behavior (that reporting behavior is memory-less and so that one report does not affect the likelihood of another for that incident), which is likely violated if the same person makes multiple reports about the same incident. In theory, such repeats should be minimal: NYC makes available a portal to check the status of past reports, and so a reporter does not need to call again to remain up-to-date. In practice, however, our contacts at DPR indicated that repeat calls occur.

To mitigate the effect of such repeat callers on our analysis, we obtain anonymized (hashed) caller information from DPR for each report. We then filter out the duplicate reports for each incident where they may be from the same caller, with different specifications. Our estimates are largely the same on these more conservative datasets, suggesting that repeat callers do not substantially bias our estimates. For brevity, the results obtained on these filtered datasets are omitted. 

% To mitigate the effect of such repeat callers on our analysis, we obtain anonymized (hashed) caller information from DPR for each report: if the caller provided it, their name, phone number, and/or email address. We then filter out the duplicate reports for each incident where either the phone number or emails match, or both the first and last names match. Our analyses are run on the resulting filtered dataset.
% %
% The above approach may not filter out all repeat callers: if callers choose not to leave their information, but call multiple times. Thus, we also run our main analyses on a filtered dataset where we additionally assume that any caller who did not leave their information is a repeat of a previous caller with no information. Our estimates are largely the same on this more conservative dataset, suggesting that repeat callers do not substantially bias our estimates.




\paragraph{Censored data: incidents that were not inspected}
% \input{subsections/inspection_discussion}

The DPR only marks duplicate reports corresponding to incidents that were inspected: for the $35\%$ of service requests not connected to an inspected incident, we do not know which (if any) other reports also refer to the same incident. As our method relies on the rate of duplicate reports, we must discard service requests not inspected.

This censoring may limit the generalizability of our findings, from measuring the reporting rates of all incidents, to measuring the reporting of incidents that tend to be inspected. This limitation to external validity may be acceptable: if the inspection decisions are correlated with incident importance, then studying the reporting behavior for these incidents is a more important task than is studying that of minor incidents not deemed worth inspecting.

There is a second reason we believe that the censoring is relatively acceptable. In particular, we measure reporting rates as a function of incident type $\theta$, where, as described next, the type includes characteristics such as report category and incident risk. If our models are correctly specified, and $\theta$ is rich enough to capture inspection decisions (there is no confounding), then this censoring does not affect our estimates.\footnote{We aim to model $\tilde{Pr}(Y | \theta)$, where $Y$ is reporting behavior. However, with just data on inspected incidents, we can only estimate $\tilde{Pr}(Y | \theta, \text{inspected})$. If $Y$ is independent of the inspection decision given $\theta$, then $\tilde{Pr}(Y | \theta, \text{inspected}) = \tilde{Pr}(Y | \theta)$. One potential source of bias is if, even conditional on $\theta$ (which includes the \textit{content} of the reports), DPR is making decisions that strongly correlate with the \textit{number} of reports. Then, all of our rate estimates would be biased upwards, as we selectively observe data for incidents with many reports. However, as we primarily care about \textit{heterogeneous} reporting rates across types, such a bias matters to the extent that it heterogeneously affects different types of incidents or geographic locations. Furthermore, according to DPR, the primary drivers of inspection decisions are the report characteristics, which are included in $\theta$. Nevertheless, an important direction for future work is directly addressing this censoring challenge.} While a seemingly strong assumption, we note that the $\theta$ we have available is the same data that the DPR sees about a report through their portal when making an inspection decision; any confounding would have to come from another source.

Nevertheless, to the extent that the above (likely small) bias affects practice, it may be valuable for 311 systems to systematically tag duplicates for all reports and then apply our methods. Relative to the missing data challenges that we centrally tackle in this work, i.e., incidents not reported and birth and death times, this duplicate censoring is cheaply addressable by city agencies.





\subsubsection{Creating an aggregated incident dataset.}
 \begin{figure}[tb]
	\centering
	%	\begin{subfigure}{.5\textwidth}
	% 		\centering
	\subfloat[][Number of reports per incident.]{
		\includegraphics[width=.45\textwidth]{plots/NumberReports_hist}
		% 		\caption{Census tract fixed effects}
		\label{fig:numreportshist}
		% 		\end{subfigure}
	}
	\hfill
	\subfloat[][Length of observation period.]{
		\includegraphics[width=.45\textwidth]{plots/Duration_hist}
		% 		\caption{Census tract fixed effects}
		\label{fig:durationhist}
		% 		\end{subfigure}
	}
	\caption{Distribution of number of reports and length of observation for each unique incident in the aggregated dataset. For most incidents, there are no reports after the first report (at least not in the observation period). There is a peak at 100 days for the observation period, due to our configuration in \Cref{eq:duration}, where we truncate longer periods to 100 days.}
\end{figure}




Before training models, we need to construct a dataset in which each row corresponds to an incident, and where we have the number of reports $\tilde M_i$ in an observation interval, the duration $\tilde T_i$ of that interval, and covariates $\theta$. We separated out an exploratory dataset of 8000 unique incidents, on which we conducted covariate selection as detailed below.\footnote{While the exploratory data was used to filter variables for ultimate analysis, and to develop and fine-tune our models, we note that we did not hold out a separate test set at the outset of the project; it was not clear how to cluster assign reports to test and train before developing our empirical strategy, and there were initial (ultimately resolved) data errors on how reports were tagged to unique incidents. Thus, our overall approach was selected and developed using the data on which we ultimately report results, and so it may be useful to acquire more recent data from DPR and verify our findings. The exploratory dataset was ultimately composed of 4463 unique incidents, after the filtering as described below.}


We filter out the reports corresponding to the uninspected service requests (as discussed above, we do not have duplicate information for these), and then use the provided incident label to group all service requests for the same incident. Then, we remove repeat caller reports as described above, comparing each caller to previous (ordered by time) callers for the same incident. Next, we must construct a valid observation interval for each incident.


%To create an aggregated dataset workable for our empirical methods, we focus on the information observed for each unique incident.

\paragraph{Constructing an observation interval $(\tilde t_i, \tilde t_i + \tilde T_i]$} As outlined in \Cref{thm:stoppingtimes}, we must be careful in how we choose an observation interval $(\tilde t_i, \tilde t_i + \tilde T_i]$ in which we count reports -- we need that the interval is inside the incident lifetime, i.e., we must end the interval before the incident is addressed, $\tilde t_i + \tilde T_i \leq t_i + T_i$. Both endpoints of the interval must also be stopping times, i.e., not use information from the future. As discussed above, the natural choice to start the observation period $\tilde t_i$ is the time of the first report, but choosing the observation end is a design choice.

We make the following choice. Let $t_i^{\text{INSP}}$ be the inspection time of incident $i$, and, $t_i^{\text{WO}}$ be the time that a work order is placed for incident $i$, if applicable. Then, $\tilde{T}_i$ of each incident $i$ is:
\begin{equation}
	\tilde{T}_i = \min \left\{100\text{ days},\  t_i^{\text{INSP}} - \tilde{t}_i,\  t_i^{\text{WO}} - \tilde{t}_i\right\}. 	\label{eq:duration}
\end{equation}
The maximum duration 100 is a design choice, for which we perform robustness checks (with 30 and 200 days); a maximum mitigates -- for incidents not inspected for a long time -- the inclusion of a time period in which an issue might have been resolved before an inspection, which would bias our estimates downward. \Cref{eq:duration} requires that inspection and work order times are stopping times; that they do not depend on the future trivially holds, and it is likely that they do not depend on the reporting {rate} except through the type $\theta$ and the sample path number of reports received up to that time. (It is not a problem that incidents with more reports are inspected sooner).

\vspace{1em}

\noindent \Cref{fig:numreportshist} shows the histogram of the number of reports per incident during the observation interval; \Cref{fig:durationhist} shows the distribution of durations; and \Cref{tab:Summary} shows how the average duration differs by Borough and report category. The heterogeneity in duration length (due to the speed of being inspected or worked on) demonstrates the value of \Cref{thm:stoppingtimes}.  For example, compared to `Prune' incidents, `Hazard' incidents tend to have more reports on average and shorter duration: residents have a higher reporting rate for hazardous incidents, and these incidents tend to be addressed more quickly. Suppose we had to use a fixed duration $D$, instead of an inspection/work order dependent time. If $D$ is large (e.g., $D \approx 15$ days), then we bias our estimates downward, as we're including time periods after an incident has already been addressed -- and the bias heterogeneously affects incident types, since some incidents are addressed sooner. On the other hand, a much shorter duration would substantially limit the data. Finally, Appendix \Cref{fig:daysfirstcomplaint} shows the average number of days after the first report that the $\ell$th duplicate report was submitted for an incident, for incidents with at least $k \geq \ell$ reports. The plots are largely linear (i.e., the average delay between the first and second report is the same as that between the third and forth report), consistent with reporting rates being homogeneous Poisson within the interval.



%Note that in practice, though inspection and work orders may depend on the number of reports that one incident receives, conditional on the number of reports an incident has received, the inspection time and work order placed time are typically independent on the reporting process, and only depend on the inspection personnel or the scheduling system for such inspection, thus $\tilde{t}_i+\tilde{T}_i$ satisfies our assumption in Theorem \ref{thm:stoppingtimes}.

%The benefit of such setting is that we are able to avoid anomalies created by human error where, for example, the inspection time is incorrectly logged.


%Even from these crude summary statistics, we are able to make some interesting observations.Our setting which uses stopping times as death times comes in handy here, as if using stopping times was not an option, we would have to use a fixed observation duration instead of a minimum of inspection time, work order time and some fixed value. In other words, using stopping times helps us bring out the variation of incidents in the data, which in turn helps with the estimation and recognition of heterogeneity.  These benefits all result from the use of stopping times as the hallmarks of the observation period, as established by \Cref{thm:stoppingtimes}.



\paragraph{Covariate selection and processing} Next, we select the covariates that compose type $\theta$. The data given to us by DPR includes a set of \textit{report} covariates (e.g., report \textit{Category}),\footnote{Occaisonally, different reports about the same incident disagree on the report covariates. We select the first report characteristics in those cases.} \textit{inspection} results (e.g., condition of tree at inspection time), and \textit{tree} characteristics (e.g., diameter of tree at breast height, tree species). We augment this data with \textit{socio-economic characteristics} as follows. Our data contains latitude-longitude coordinates for each inspection (and thus incident), using which we identify which of the over 2000 census tracts in New York City the incident is in, through a FCC API.\footnote{FCC Area API, https://geo.fcc.gov/api/census/} We then join this information with 2020 Census data obtained from the United States Census Bureau, which includes socio-economic characteristics such as race/ethnicity, education, income, and population density for each census tract. We are unable to match 9473 incidents to census tracts and discard them in our analysis.

Next, we perform covariate selection using the exploratory dataset. We remove report and inspection variables that are highly collinear, low variance, or with high number of missing values. Conversations with DPR also played a role in selection. %: for example, we include Borough fixed effects our analyses, as DPR indicated that each Borough has an agency sub-unit which handles requests---and so there might be differences in how different Boroughs conduct inspections.
Finally, we log transform several variables, and standardize all data. The exact list of all covariates selected is shown in Appendix \Cref{tab:desc}.

% Appendix \Cref{tab:desc} contains the covariates we use.



%\nikhil{Covariate selection on exploratory dataset}  \nikhil{For example: how select from report characteristics}

%Then, we separate an exploratory and model development dataset, on which we do the following.



\smallskip

Starting with the dataset discussed above, we filter out the incidents for which any of the covariates are missing, those with short logged reporting periods (Duration less than 0.1 days), and those in the exploratory dataset. We are left with a dataset of $78151$ incidents on which we conduct our main analyses; for each incident $i$, we have the duration of observance $\tilde{T}_i$, the number of total reports $\tilde M_i$, and all the various geographic and demographic covariates associated with it.




\subsection{Analyses, training, and evaluation}

We fit our models using Stan \citep{carpenter2017stan}, a Bayesian probabilistic programming language.

We use three sets of covariates. Every analysis includes our incident-specific covariates (inspection results, report \textit{Category}, tree size) and an intercept. Our \textbf{Base} analysis includes just these covariates along with \textit{Borough} level fixed effects. As the covariates are standardized, these coefficients all have a zero-mean Normal prior. \textit{Borough} and \textit{Category} are categorical variables; instead of dropping one level for each variable, to maintain identifiability we enforce a sum zero constraint\footnote{\url{https://mc-stan.org/docs/2_28/stan-users-guide/parameterizing-centered-vectors.html}} on their coefficients to ease interpretability. For the other categorical covariates, we drop one level each.

In our \textbf{Spatial} analysis, we include coefficients for each of the (over 2000) census tracts. We use an Intrinsic Conditional Auto-Regressive (ICAR) model~\cite{morris2019bayesian} for the spatial coefficients, alongside the incident level coefficients. In such models, each census tract coefficient is assumed to be normally distributed with a mean equal to the average of its neighbors -- i.e., spatial smoothness is encoded into the model, and so census tracts with few incidents borrow information from neighboring census tracts.
%
Finally, in our \textbf{Socio-economic} analyses, we include each census \textit{socio-economic} covariate \textit{individually} with the incident-specific covariates (e.g., the regression with \textit{Median Age} contains as coefficients the base covariates, but not \textit{Fraction Hispanic}; this choice is due to the census covariates being highly collinear). These covariates are also standardized, and coefficients prior means are set to zero.

For the \textbf{Base} covariates, we fit both the \textbf{standard} and \textbf{zero-inflated} Poisson regressions, and evaluate model fit. Both models perform similarly in terms of overall predictive power, with Pearson correlations of $0.1335$ and $0.1248$, respectively, for the mean prediction for number of reports for each incident vs the observed number of reports. Next, we perform a standard check for Bayesian models: whether the posterior prediction distribution matches the observed data distribution, as a test for whether the model captures the underlying data generating process; the resulting figure is omitted for brevity. We observe that each model roughly matches the observed distribution, but differ in various ways. The \textbf{standard} Poisson Regression under-estimates the (large) fraction that $\tilde M_i = 0$, but more accurately captures the distribution tail. Inversely, the \textbf{zero-inflated} Poisson Regression matches the fraction for small $\tilde M_i$ (where the majority of the mass is), at the cost of mis-estimating the tail.

% Appendix \Cref{fig:posteriors} compares the distribution for each model specification. 

These results suggest that if the goal is to predict number of reports for each incident, then there are model improvements to be made (for example, by allowing the zero-inflation fraction to depend on incident type, or by allowing non-homogeneous reporting rates). However, to understand how $\lambda_\theta$ varies by incident type $\theta$, we prefer our simpler specification; for the analyses below, we primarily report results with the \textbf{zero-inflated} Poisson regressions, choosing it because it better matches the primary distribution mass. Results with the \textbf{standard} model are similar. We further run these regressions on datasets with different configuration of the maximum duration in \Cref{eq:duration} and different filtering of repeat callers, as mentioned above. The results are similar, and are omitted in this short version for brevity.
%\todo{still editing below this}





==> subsections/4_results.tex <==
A substantial benefit of our approach is its ability to capture fine-grained reporting \textit{heterogeneity}, which is important in both (1) auditing the efficacy and equity of the reporting system, and (2) designing better approaches to respond to reports. We focus on understanding this heterogeneity, across \textit{incident characteristics} and \textit{neighborhood}, especially with respect to potential \textit{socio-economic equity} concerns. Here, we report results for the \textbf{zero-inflated Poisson regression}, including with ICAR spatial coefficients.



%\nikhil{Either the forest plot, or a regression coefficient table for zero inflated bayesian model with no census coefficients besides borough}




%\input{plots/basic_zeroinflated_nocens2_dur100_repmedium_300300-1nocens2_latexsummary.tex}
\input{plots/basic_zeroinflated_paper1_dur100_repmedium_300300-1nocens2_latexsummary.tex}
\input{plots/tab_ratescontext.tex}

\paragraph{Reporting heterogeneity across incident type} We first study how reporting rates vary by incident-level characteristics. \Cref{tab:basicinfrefcoef} shows the coefficients resulting from the zero-inflated regression, using our \textbf{Base} analysis covariates. \Cref{tab:contextualizingrates} contextualizes the coefficient estimates into average reporting delays.
%



 We find that reporting rate substantially (and statistically significantly) varies by incident type. In particular, we have several columns characterizing the results of an inspection by a forester. The following incident characteristics (as marked by the inspector) are characterized by higher resident reporting rates: higher risk ratings, and trees in Poor or Critical condition (as opposed to Excellent, Good, Fair, or Dead). Similarly, those incidents that the first resident reporter indicated was a Hazard (as opposed to e.g., a Root/Sewer/Sidewalk issue) are also reported at higher rates. These differences are practically relevant: the difference in coefficients between the Hazard and Illegal Tree Damage categories is $1.3$, and so Hazard incidents are reported at approximately a  $e^{1.3} \approx 3.6$ times higher rate than are Illegal Tree Damage incidents.\footnote{The interpretation is not exact, as we learn a single zero-inflation coefficient. However, coefficients in the non-zero-inflation model are similar.} Perhaps surprisingly, tree size is not strongly associated with reporting rate, given the other incident characteristics.

 These incident level associations mostly align with what one would expect, suggesting both that the reporting system is largely efficient (with more serious incidents reported faster) and that our method is precise enough to capture such heterogeneity. For example, DPR suggested to us that Root/Sewer/Sidewalk issues are particularly difficult for most residents to find, as the problem is often underground. This level of precision is not available for other methods to measure under-reporting, as one would need to construct equally precise estimates on the ground truth rate that incidents of different types occur.


 \begin{figure}[tb]
 	\centering
%	\begin{subfigure}{.5\textwidth}
% 		\centering
\subfloat[][Census tract spatial coefficients]{
 		\includegraphics[width=.44\textwidth]{plots/adjacencysmooth_censusmap}
% 		\includegraphics[width=.45\textwidth]{plots/tract_hierarchy_zeroinflated_hiertract11medpriornocens2_dur100_repmedium_300300-1nocens2_censusmap}
% 		\caption{Census tract fixed effects}
 		\label{fig:spatialmap}
% 		\end{subfigure}
}
 	\hfill
%	\subfloat[][Census tract demographic coefficients]{
%% 		\centering
%		\input{plots/basic_zeroinflated_bas_singlecens2_basic_zeroinflatedsinglecens2_dur100_repmedium_unicoefsequity.tex}
%% 		\subcaption{Census Tract Demographic coefficients}
% 		\label{tab:censuscoefficients}
%}
	\subfloat[][Census tract demographic coefficients]{
	% 		\centering
		\input{plots/basic_zeroinflated_noborough_paper1_dur100_repmedium_300300-1singlecens2__unicoefsequity.tex}
	% 		\subcaption{Census Tract Demographic coefficients}
	\label{tab:censuscoefficients}
}



 	\caption{Coefficients on spatial and socio-economic covariates. The census tract spatial coefficients are estimated using the ICAR spatial zero-inflated Poisson regression. The demographic coefficients are each estimated alone in a regression alongside the incident-specific covariates.}
 	\label{fig:spatialheterog}
 \end{figure}


 \paragraph{Spatial reporting heterogeneity} \Cref{tab:basicinfrefcoef} establishes that reporting rates vary substantially based on incident characteristics, but there further may be substantial residual spatial heterogeneity. We now analyze this heterogeneity, using the \textbf{ICAR Spatial zero-inflated Poisson regression} described above. \Cref{fig:spatialmap} shows the coefficient associated with each census tract---there are substantial (and statistically significant) spatial effects, on top of the effects of incident-specific variables as above. Notably, these coefficients are \textit{on the same order} as the incident-specific characteristics, suggesting substantial inefficiencies and inequities. For example, comparing the coefficients for downtown Manhattan to those for parts of Queens suggests that reports occur at a three times higher rate in downtown, even after controlling for the incident-level characteristics.

 Next, these spatial effects demonstrate that using just raw observed incident count for each census tract may be misleading. Appendix \Cref{fig:reginccoef} shows the relationship between the census tract coefficient and the number of unique incidents observed for that census tract in the time period. Perhaps surprisingly, there is a slight negative relationship. These differences may emerge for two reasons: (a) the non-identifiability between the rates incidents occur and are reported (\Cref{prop:identi}), and (b) that observed counts do not control for `legitimate' incident-specific characteristics (such as risk), that may correlate with geography.

\paragraph{Reporting socio-economic inequities} \Cref{fig:spatialmap} illustrates that there is substantial spatial heterogeneity in reporting behavior; as there is socio-economic geographic clustering in New York, such a pattern suggests potential inequities on socio-economic lines. We now study such inequities more directly.
%
Table \ref{tab:censuscoefficients} contains coefficients for each census covariate, when it is included \textit{alone} in a regression alongside the incident-specific covariates (full table omitted for brevity). We consider census covariates one-by-one, as otherwise the collinearity between variables complicate interpretation. We also include Borough fixed effects, and so these coefficients are best interpreted as within-Borough associations.

% Appendix \Cref{tab:coeffull} shows the full table, with Bayesian confidence intervals. 

We find that there are associations with these characteristics, though overall there is much spatial heterogeneity that cannot be explained by socioeconomic factors. The strongest association is with population density: the more people per unit area, the more people that might encounter an issue. We also find that race/ethnicity substantially correlates with reporting rates, as does education, wealth, and age, though at a smaller scale than spatial or incident-level coefficients. For example, one standard deviation increase in the proportion of white people is associated with a $5\%$ increase in reporting rate, conditional on incident-level covariates -- and this is on a similar level as density. %However, we note that Borough level fixed effects may be masking such associations.

%Basic inflated single census variable regressions
%med_age -0.047 (-0.061,-0.032)
%frac_hispanic 0.033 (0.017,0.048)
%frac_white 0.055 (0.039,0.07)
%frac_black -0.036 (-0.051,-0.02)
%frac_noHSGrad -0.022 (-0.036,-0.0072)
%frac_collegegrad 0.043 (0.028,0.058)
%frac_poverty -0.018 (-0.033,-0.0035)
%frac_renter 0.052 (0.036,0.068)
%frac_single_unit -0.062 (-0.079,-0.046)
%loghouseholdincome 0.017 (0.0029,0.031)
%logdensity 0.1 (0.085,0.12)




% \todo{something about similar results with other methods}


==> subsections/5_conclusion.tex <==
\label{sec:conclusion}
We develop a method to quantify inequities in resident reports and apply it to data from the 311 system in New York City. We believe that our method provides a powerful, general approach to precisely quantifying efficiency and equity in the use of resident crowdsourcing (``co-production'') system, without needing external ground-truth data. In our application, we find that there is substantial spatial heterogeneity in resident reporting, associated with socio-economic characteristics of the neighborhoods in which the incident occurred. Our method can be applied almost off-the-shelf to other co-production systems, as duplicate reports are already logged by many agencies. We also anticipate that other reporting systems -- such as for bug reports -- are amenable to our methods.

% \todo{copied from abstract, need fixing}

An important next step is to apply our findings to better \textit{design} and \textit{operate} 311 systems, for which our work provides a foundation. For example, one can use our reporting delay estimates to develop more equitable scheduling schemes for inspections, for example by re-ordering inspection priorities account based on average reporting rates.

% we study the identification of inequities in resident reports, with the 311 system in New York City as an example. We first present a general data-generating model, under which we introduce a metric for \textit{under-reporting} behavior. Inspired by the missing species problem, we suggest a way of using \textit{duplicate} reports to estimate it in order to overcome non-identifiability problems. Following this idea, we then developed multiple empirical approaches which accommodate to varying settings, and show that our approaches have potentials for future development. Through an application on data containing NYC residents' reports on malfunctioning trees, we showed that there exists

% \todo{1 paragraph summary}
% \todo{highight that duplicates method can be used for all sorts of 311 settings, since most cities log this information (NYU paper mentions that they took out duplicates)}

% One benefit of our method is that, . The use of duplicates is not confined to reports on trees, but can be extended to all sorts of incidents. In other settings, more elaborate and problem-specific configuration will have to be considered, and the flexibility of our methods would help accommodate that.


% \todo{This is useful for operations, and balancing for equity, etc}
% \todo{more generally, this question of who participates in crowdsourcing and mechanism design for that is interesting}

% Towards operations, our method also provide much insight. Estimating the reporting rate provides potentials for backtracking the timeline and infer a distributional estimate of the actual birth of each incident, upon we observe a report about it. This lays a groundwork for a . This can further contribute to more efficient response to other types of incidents, leading to much future work in the equitable allocation of government resources.



==> subsections/_comparing_methods_via_simulation.tex <==
\subsection{Comparing estimation methods via simulation}
\label{sec:simulation}

\input{plots/tab_sim}

Before applying our methods to real-world 311 data, we demonstrate the effectiveness of our methods via simulated data---in such simulations, we have full control over the data-generating process and thus can compare the estimation results with the true parameters. In particular, we use the simulator to illustrate (a) \Cref{prop:identi}, that attempting to recover reporting rates $\lambda_\theta$ from $N_\theta^\obs(T)$ is prone to bias; (b), that in \Cref{thm:stoppingtimes}, the assumption that both $\tilde{t}_i$ and $\tilde{t}_i+\tilde{T}_i$ are stopping times is essential, (c), that in a correctly-specified model setting, i.e., following the assumptions in \Cref{thm:stoppingtimes}, both the MLE in \Cref{eq:MLE} and the homogeneous Poisson regression recover the ground truth; and (d), that the regression approach is more data-efficient than the MLE, leading to tighter parameter estimates.


%To establish the robustness of our proposed methods, we first apply them on simulated data. The simulated data are generated through our proposed data-generating process, and validated by comparing with real-world data.

%The main advantage of using simulated data is that we have the `ground-truth' of this system. Due to the imbalance of reporting behavior, in real world data, the observed is only a biased sample of the truth. With

\paragraph{Simulator setup} We simulate a basic time-homogeneous system, as follows. We set the incident type to be a two-dimensional vector $\theta \in \bbR^2$. % = (\theta_1, \theta_2, \theta_3, \theta_4) \in \Theta_1\times\Theta_2\times\Theta_3 \times \Theta_4$.
Our simulator needs parameters for three processes: the incident birth process governed by homogeneous Poisson rate $\Lambda_\theta$, the reporting process governed by homogeneous Poisson rate $\lambda_\theta$, and a lifetime $T_i$ of each incident, generated in the following way: after each report, we sample two competing exponential clocks, one representing incident death and another the next report; the incident death rate can depend on the number of reports so far, reflecting, for example, that the agency prioritizes inspections for incidents with more reports. If the report happens before death, we increment the number of reports for the incident and repeat; otherwise, the incident has ``died'' and no more reports are logged.

Formally, for each type of incidents, we specify a parameter $\mu_\theta$ that is independent of $\lambda_\theta$ as the ``death rate'' of incidents; conditional on there has been $m$ reports of an incident of type $\theta$, we generate two exponentially distributed random variables, $d^m_\theta\sim \text{Exponential}(\mu_\theta\times (\gamma_\theta)^m)$, where $\gamma_\theta$ is a scaling parameter by our choice, and $r^m_\theta \sim \text{Exponential}(\lambda_\theta)$; if $d^m_\theta \le r^m_\theta$, we consider the incident dead, and let $T_i=\sum_{j=0}^{m-1}r^j_\theta + d^m_\theta$, otherwise increment $m$ and repeat the process.
%
% \todo{Three or 4 dimensional? Above and below are inconsistent}
Both the incident and reporting rates are set as a function of the type covariates, as in \Cref{eqn:lambdaregressionassumption}:
\begin{align*}
\Lambda_\theta = \exp\left(\alpha_\text{incident} + \beta_\text{incident}^T\theta\right) && \lambda_\theta = \exp\left(\alpha_\text{report} + \beta_\text{report}^T\theta\right)
\end{align*}
where $\alpha_{incident}\in \mathbb{R}$, $\beta_{incident}\in \mathbb{R}^2$, $\alpha_{report}\in \mathbb{R}$ and $\beta_{report}\in \mathbb{R}^2$ are varied across simulations. For simplicity in comparing the various methods, here we report simulation results for the case in which there are only 5 distinct types, the reporting rate for each type is $2$, i.e., $\alpha_{report}=\log(2)$ and $\beta_{report} = \textbf{0}$, but where incident rates $\Lambda_\theta$ vary by type.

Next, we need to set $\mu_\theta$ and $\gamma_\theta$, which governs the duration that the incident is alive. Given the above parameters, we do so in a manner that matches the distribution of the number of reports received per incident to the real data studied in the next section:  that 18.7\% of the received reports in the reporting period are duplicates of incidents already reported. For simplicity, we set these uniformly across all types. This calibration results in $\mu_\theta =  0.065$ and $\gamma_\theta = 100$ for all $\theta$.

% \zhi{just redid this and the sim, should check out now, conclusion is the same}

%The main purpose of our comparison is to determine the robustness of the various estimators to small sample sizes for a specific type of incidents. To this end, we fixed , and adjusted the incident rates for different types.

Finally, we fix the time span of our observation to be $T=300$ days, which by our parameter settings, is long enough for the system to converge to its long-run stationary distribution (in terms of the number of active incidents). Incidents and reports are generated according to the simulator setup. It is possible that some death times and consequently reports generated may be beyond the 300-days observation period. We discard any such reports.

The output of the simulator consists of all the incidents that occur and are reported at least once during this 300-days period. For all these incidents, the available data for our estimators is the time that each incident was reported the first time, the times and number of the subsequent reports, and the times of the incident death, if they occur before the end of the time span. To specify the observation period of each incident, in the setting of \Cref{thm:stoppingtimes}, we let $\tilde{t}_i$ be the time of the first report of such incident, and $\tilde{t}_i +\tilde{T}_i$ be the incident death time, or the end of the time span, if the death time is greater than it. This specification satisfies the assumption in \Cref{thm:stoppingtimes}. As a comparison, we add an incorrectly specified version of this observation period by letting $\tilde{t}_i +\tilde{T}_i$ be the time of the last report of this incident, in which case it is no longer a stopping time.


%For the purpose of validating our simulation framework, we compare the data generated by the simulator with real-world data on one key aspects -- the percentage of the duplicate reports over all reports. The reason that this is the key criterion to check is that, by manipulating the time scale, we can potentially change the number of incidents and reports and the rates for incident spawning and reporting. On the other hand the duplicate reports is in some sense `time-invariant' -- regardless of the time scale, if we observe for a long enough period, the percentage should always be the same. By the above setting, primarily the setting of the incident death time distribution, we are able to achieve a 18.7\% duplicates in the simulated data across all covariates, which matches that in the real data.



%To generate simulated datasets, there are a number of key aspects and parameters in the data-generating process that we have to determine.

%For each incident type $\theta$, we determine the incident rate using



% We then generate the incidents of type $\theta$ that happened in this duration of time according to a Poisson process with rate $\Lambda_\theta$.

%For each incident, we determine the number of times that it is reported in the following way. First, we calculate the reporting rate as
%
% We then set parameter $\mu_\theta$ as
%$$
%\mu_\theta = \frac{1-\exp(-0.423)}{\exp(-0.423)}\lambda_\theta = 0.527 \lambda_\theta.
%$$

%The lifetime $T_i$ of each incident $i$ is then .
% The reason behind such choice of parametrization will be explained later.

%\paragraph{Estimation procedures}





% Finally, .

% , and mark the incident in question as `open', as expected in reality.



%\textbf{Validation of simulated data.}



\paragraph{Simulator results} We compare five estimators: a ``naive'' estimator, that calculates $\frac{N_\theta^\obs(T)}{T}$, the ratio between the observed number of reports and the observation period; the MLE as derived in \Cref{eq:MLE} with correctly specified stopping times; the MLE with incorrectly specified observation ending times; a Poisson regression with correctly specified stopping times, and finally, a Poisson regression with incorrectly specified observation ending times. The regression methods were implemented using Scikit-learn \cite{scikit-learn}. We run each of the methods on the same simulated datasets, and iterated for 300 times. \Cref{tab:sim} summarizes our results: showing, for each distinct type with a differing incident rate, the estimates for $\lambda_\theta$ for each of the methods.
%; the poststratified MLE is by fitting a linear regression model with the MLE as dependent variable and the covariates as independent variable, and poststratify to get the estimate for each type

 These results indeed illustrate \Cref{prop:identi}, that attempting to recover reporting rates $\lambda_\theta$ from $N_\theta^\obs(T)$ is prone to bias: the naive method of counting the number of observed incidents conflates the incident rate with the reporting rate. Second, the stopping times assumption in \Cref{thm:stoppingtimes} is indeed crucial to a valid result, and in a correctly-specified model setting, both the MLE in \Cref{eq:MLE} and the homogeneous Poisson regression recover the ground truth reporting rate $\lambda_\theta$, regardless of the incident rate. However, third, the regression approach is more data-efficient than the MLE, leading to tighter parameter estimates -- especially  as the incident rate decreases, i.e., as the sample size in terms of the number of incidents decreases. This data efficiency is important in high dimensions, as in our real-world data application in the next section.





% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

%These results suggest that, estimates obtained from Poisson regression outperforms that from simple MLE in terms of both accuracy and precision, even in this most simplified model. It is worth noting that, however, even the simple MLE is able to give estimates very close to the truth, whereas the naive estimates fluctuate with the sample sizes, showing that it does not extinguish between incident rate and report rate.


==> subsections/_comparing_methods_via_simulation_short.tex <==
\subsection{Comparing estimation methods via simulation}
\label{sec:simulation}

% \input{plots/tab_sim}

Before applying our methods to real-world 311 data, we demonstrate the effectiveness of our methods via simulated data---in such simulations, we have full control over the data-generating process and thus can compare the estimation results with the true parameters. 

In particular, we use the simulator to illustrate the following results: (a) \Cref{prop:identi}, that attempting to recover reporting rates $\lambda_\theta$ from $N_\theta^\obs(T)$ is prone to bias; (b), that in \Cref{thm:stoppingtimes}, the assumption that both $\tilde{t}_i$ and $\tilde{t}_i+\tilde{T}_i$ are stopping times is essential, (c), that in a correctly-specified model setting, i.e., following the assumptions in \Cref{thm:stoppingtimes}, both the MLE in \Cref{eq:MLE} and the homogeneous Poisson regression recover the ground truth; and (d), that the regression approach is more data-efficient than the MLE, leading to tighter parameter estimates.



% \paragraph{Simulator results} We compare five estimators: a ``naive'' estimator, that calculates $\frac{N_\theta^\obs(T)}{T}$, the ratio between the observed number of reports and the observation period; the MLE as derived in \Cref{eq:MLE} with correctly specified stopping times; the MLE with incorrectly specified observation ending times; a Poisson regression with correctly specified stopping times, and finally, a Poisson regression with incorrectly specified observation ending times. The regression methods were implemented using Scikit-learn \cite{scikit-learn}. We run each of the methods on the same simulated datasets, and iterated for 300 times. \Cref{tab:sim} summarizes our results: showing, for each distinct type with a differing incident rate, the estimates for $\lambda_\theta$ for each of the methods.
%; the poststratified MLE is by fitting a linear regression model with the MLE as dependent variable and the covariates as independent variable, and poststratify to get the estimate for each type

%  These results indeed illustrate \Cref{prop:identi}, that attempting to recover reporting rates $\lambda_\theta$ from $N_\theta^\obs(T)$ is prone to bias: the naive method of counting the number of observed incidents conflates the incident rate with the reporting rate. Second, the stopping times assumption in \Cref{thm:stoppingtimes} is indeed crucial to a valid result, and in a correctly-specified model setting, both the MLE in \Cref{eq:MLE} and the homogeneous Poisson regression recover the ground truth reporting rate $\lambda_\theta$, regardless of the incident rate. However, third, the regression approach is more data-efficient than the MLE, leading to tighter parameter estimates -- especially  as the incident rate decreases, i.e., as the sample size in terms of the number of incidents decreases. This data efficiency is important in high dimensions, as in our real-world data application in the next section.





% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

%These results suggest that, estimates obtained from Poisson regression outperforms that from simple MLE in terms of both accuracy and precision, even in this most simplified model. It is worth noting that, however, even the simple MLE is able to give estimates very close to the truth, whereas the naive estimates fluctuate with the sample sizes, showing that it does not extinguish between incident rate and report rate.


==> subsections/app_otherempirical.tex <==
\subsection{Robustness checks -- \Cref{tab:basicinfrefcoef} with other specifications}
\label{sec:robustnesstables}
In this section, we present evidence for the robustness of our results in \Cref{tab:basicinfrefcoef} by reproducing its results with different configurations in Tables 6 through 10.

\todo{broken reference}

\input{plots/tract_hierarchy_zeroinflated_hiertract11medpriornocens2_dur100_repmedium_300300-1nocens2_latexsummary.tex}

%\input{plots/basic_nocens2_dur100_repmedium_300300-1nocens2_latexsummary.tex}
\input{plots/basic_paper1_dur100_repmedium_300300-1nocens2_latexsummary.tex}

%\input{plots/basic_zeroinflated_nocens2_dur30_repmedium_300300-1nocens2_latexsummary.tex}
\input{plots/basic_zeroinflated_paper1_dur30_repmedium_300300-1nocens2_latexsummary.tex}




%\input{plots/basic_zeroinflated_nocens2_dur200_repmedium_300300-1nocens2_latexsummary.tex}
\input{plots/basic_zeroinflated_paper1_dur200_repmedium_300300-1nocens2_latexsummary.tex}

%\input{plots/basic_zeroinflated_nocens2_dur100_repmostconservative_300300-1nocens2_latexsummary.tex}
\input{plots/basic_zeroinflated_paper1_dur100_repmostconservative_300300-1nocens2_latexsummary.tex}





==> subsections/inspection_discussion.tex <==
The DPR only marks duplicate reports corresponding to incidents that were inspected: for the $35\%$ of service requests not connected to an inspected incident, we do not know which (if any) other reports also refer to the same incident. As our method relies on the rate of duplicate reports, we must discard service requests not inspected.

This censoring may limit the generalizability of our findings, from measuring the reporting rates of all incidents, to measuring the reporting of incidents that tend to be inspected. This limitation to external validity may be acceptable: if the inspection decisions are correlated with incident importance (likely), then studying the (heterogeneous) reporting behavior for these incidents is a more important task than is studying that of minor incidents not deemed worth inspecting.

There is a second reason we believe that the censoring is relatively acceptable. In particular, we measure reporting rates as a function of incident type $\theta$, where, as described next, the type includes characteristics such as report category and incident risk. If our models are correctly specified, and $\theta$ is rich enough to capture inspection decisions (there is no confounding), then this censoring does not affect our estimates.\footnote{We aim to model $\tilde{Pr}(Y | \theta)$, where $Y$ is reporting behavior. However, with just data on inspected incidents, we can only estimate $\tilde{Pr}(Y | \theta, \text{inspected})$. If $Y$ is independent of the inspection decision given $\theta$, then $\tilde{Pr}(Y | \theta, \text{inspected}) = \tilde{Pr}(Y | \theta)$. One potential source of bias is if, even conditional on $\theta$ (which includes the \textit{content} of the reports), DPR is making decisions that strongly correlate with the \textit{number} of reports. Then, all of our rate estimates would be biased upwards, as we selectively observe data for incidents with many reports. However, as we primarily care about \textit{heterogeneous} reporting rates across types, such a bias matters to the extent that it heterogeneously affects different types of incidents or geographic locations. Furthermore, according to DPR, the primary drivers of inspection decisions are the report characteristics, which are included in $\theta$. Nevertheless, an important direction for future work is directly addressing this censoring challenge.} While a seemingly strong assumption, we note that the $\theta$ we have available is the same data that the DPR sees about a report through their portal when making an inspection decision; any confounding would have to come from another source.

Nevertheless, to the extent that the above (likely small) bias affects practice, it may be valuable for 311 systems to systematically tag duplicates for all reports and then apply our methods. (Relative to the missing data challenges that we centrally tackle in this work, i.e., incidents not reported and birth and death times, this duplicate censoring is cheaply addressable by city agencies).

%\todo{continue here}
% our analysis below finds how reporting rate varies across incident and socio-economic characteristics. If reporting behavior is different between inspected and uninspected incidents (likely, as incidents are )





%One important choice for filtering the dataset is that we only retain the service requests that were inspected. This is from the fact that our methods rely heavily on the duplicates, and only inspected service requests are marked whether they are duplicates or not.

% This choice does bring potential problems, since the inspected service requests are potentially a biased subset, and we have little information as to how we could correct for this bias.

% This calls for an avenue of future work which helps identify duplicate reports from description of problem, location, and other characteristics, which would aid our estimation methods.

%However, in our setting, we believe the practical impact of bias brought by this decision is small.  On the other hand, if when making the inspection decisions, the inspection dispatchers were provided with the same set or a subset of covariates as we use in estimation, it is safe to assume that there are no confounding variables between statistics of the inspected service requests and these covariates. This helps suppress the impact of such bias to an acceptable level.

==> supershort/1_intro_anon.tex <==
\label{sec:intro}

Crowdsourcing (``co-production'' \cite{yuan_co-production_2019,brabham_crowdsourcing_2015}) systems are an essential component of how modern cities are managed. People report problems that they encounter (via phone call, text, app, social media), which are then logged and responded to by city agencies. Such reporting systems are used in over 100 North American cities; for example, New York City's 311 system received over 2.7 million reports in 2021. Reports provide real-time updates on on-the-ground conditions \citep{schwester2009examination, hacker_spatiotemporal_2020,minkoff_nyc_2016, lee_crowdsourcing_2021-1}; these updates are used to make immediate decisions---such as which potholes to inspect and fix---and longer-term planning decisions, such as which streets to resurface. 

While reporting systems have gained popularity in the last few decades, there are many ongoing concerns regarding their function. One long-standing concern is whether---conditional on experiencing a similar issue---some residents\footnote{We use the term ``residents'' to denote anyone who might report an issue to the 311 system, including visitors.} are more likely to log a report and request government services \citep{thijssen2016you,clark_coproduction_2013,cavallo_digital_2014,minkoff_nyc_2016,kontokosta_bias_2021, hacker_spatiotemporal_2020, pak_fixmystreet_2017, kontokosta_equity_2017,obrien_ecometrics_2015,obrien_uncharted_2017,obrien_urban_2018}. If reporting behavior is heterogeneous (varies by neighborhood), then government services that rely on such reporting will also be inefficient and inequitable -- for example, reporting delays may correspond to delays in incidents being addressed, if the agency responds to incidents in the order that they are reported. 

The central methodological challenge in measuring heterogeneous behavior is the same reason cities rely on crowdsourcing: ground truth conditions are unknown. This induces a missing data challenge: researchers do not directly observe what incidents occurred; even when an incident is reported, researchers and the city do not directly observe when they occurred. Thus, it is difficult to determine whether one neighborhood is \textit{under-reporting} issues compared to other neighborhoods, or whether they truly experience fewer issues (due to, e.g., differences in infrastructure). More generally, this challenge regarding identifiability between reporting and ground truth rates is referred to as the \textit{benchmark} problem, and similarly appears in criminal justice, healthcare, and other domains; arrest data for predictive policing systems, for example, may conflate historical policing disparities versus true crime rates \cite{lum2016predict}; \citet{akpinar2021effect} study the downstream consequences of mistakenly using observed incident count as a proxy for the incident rate.

To this long-standing literature, we contribute a method with two distinct advantages: (1) we provide estimates for reporting \textit{delays} -- for an incident of a given type and neighborhood, how long after incident occurrence do we expect the incident to be first reported. Previous literature primarily considers the estimation of {whether an incident is reported at all}. (2) The method does not require external, ground truth data to estimate incident occurrence rates as distinct from reporting rates. As a result, we can estimate heterogeneous reporting rates as they differ across high-dimensional incident characteristics (incident category, type, risk level, exact location, etc.). Previous literature either (a) assume uniform incident occurrence and so assume that heterogeneity in the observed reports is a result of differential reporting rate \citep{clark_coproduction_2013,cavallo_digital_2014,minkoff_nyc_2016}; or (b) use external data to construct custom, domain-specific proxies for differences in incident occurrence, and then compare the estimates with observed rates \citep{kontokosta_bias_2021, hacker_spatiotemporal_2020, pak_fixmystreet_2017, kontokosta_equity_2017,obrien_ecometrics_2015}. Such an approach requires high-quality data on incident occurrence rates, which may be expensive to obtain for each incident characteristic.\footnote{See \Cref{app:related} for an extended discussion of this literature.}

As we show through a collaboration with the NYC Department of Parks and Recreation (NYC DPR), these advantages directly translate to \textit{operational relevance} in practice: agencies can use our method's estimates to change incident response policies, for more equitable and efficient government service allocation.  



\parbold{A method to identify reporting rates without ground truth data.} We develop a method to identify (heterogeneous) reporting rates, using \textit{just} the reporting data itself and without requiring proxies for ground truth incident rates---and the method can thus be used across crowdsourcing settings without extensive domain-specific model development or data. Our insight is that we can use information on {duplicate} reports about the same incident (which cities commonly log for operational reasons) to {disentangle} the reporting process from the incident occurrence process, thus identifying reporting rates \textit{conditional on an incident having occurred}. This insight originates from the \textit{missing species} estimation literature, where the number of {duplicate} observations provides evidence regarding the existence of unseen species \citep{orlitsky_optimal_2016, wu_chebyshev_2016, han2021competitive, charikar2019efficient}. However, our setting differs from that literature as incidents, unlike species, occur and are resolved over short time scales; and, even for observed incidents, we do not know \textit{when} they occurred, or \textit{how long} the incident existed. 

We show how to nevertheless convert the task to a standard \textit{Poisson rate estimation} challenge, for which a large empirical and theoretical literature exists. In particular, one can use the number of reports between the time of the first report (but not including it) and an estimated incident resolution time, to recover a {Poisson} likelihood with a corresponding rate function. %We show that the method is valid if the estimated death time is an \textit{under-}estimate of the resolution time and is a \textit{stopping time} (does not depend on the future).
An advantage of the method is that we can then leverage standard Poisson rate estimation methods to recover the rates that incidents of different types and in various neighborhoods are reported, conditional on the incident having occurred. For example, we empirically fit Bayesian Poisson regression models with spatial smoothing.  


\parbold{Application of our method to understand usage disparities.} We apply our method to resident reports made in New York City and the City of Chicago. Using primarily public data,\footnote{NYC DPR provided us with anonymized reporter details, so that we could filter out duplicate reports made by the same caller. The public data includes each report, its timestamp, report details, and agency response details.} we analyze reports made to the New York City Department of Parks and Recreation (NYC DPR), and the City of Chicago Departments of Transportation (CDOT) and Water Management (CDWM). 
%Our data is primarily publicly accessible, with the addition of anonymized reporter details and internal logs on incident inspection outcomes and work orders provided to us by the New York City Department of Parks and Recreation (NYC DPR).
%
We estimate how the reporting rate varies as a function of incident characteristics (e.g., the request category), spatial dynamics, and socio-economic characteristics of the neighborhood in which the incident occurred. We illustrate that our method is precise enough to find differences in reporting rates; for example, we find that reports for more hazardous incidents are submitted at substantially higher rates, conditional on the incident having occurred.

We then study spatial and socio-economic heterogeneity in New York City and Chicago. We find that there are substantial inter-location reporting differences; for example, comparing census tract-level fixed effects, we find that incidents are reported at a three times higher rate in downtown Manhattan (denser, higher income Borough) than in Queens, even after controlling for the incident-level characteristics. These differences are correlated with socio-economic and demographic factors: for example, in NYC, population density, fraction of college graduates, income, and fraction of the population that is white are all positively associated with reporting rates. These findings suggest that the allocation of government services, when reliant only on incident reporting, is inefficient and inequitable. %Reporting rates further vary by season. 

As we discuss, in partnership with NYC DPR, these estimates are being used to inform operational decisions, to reduce the effects of resulting inefficiencies and disparities. 
% \todo{update this summary with updated application}

\smallskip

\textbf{Code availability statement.} Our full code is available at \censor{the url to the code}.

\textbf{Data availability statement.} Public 311 data for both NYC and Chicago is available via their Open Data portals. In the GitHub repository above, we have included official links to the portals and further host the exact public data used in this work. The primary NYC results in \Cref{sec:results} are run on private data confidentially provided to us by NYC DPR that cannot be shared -- that data additionally contains columns for anonymized reporter identification, to allow filtering duplicate reports by the same user. However, all results replicate with the available public data, as reported in the Appendix. The Chicago analyses are fully based on publicly available data. 



==> supershort/3_empirical_1_identification.tex <==
% \zhi{begin a simplified rewrite of section 3 below. If we shorten it like this, can maybe merge with the current section 6, and be one section on methods}

% The central methodological challenge in identifying and estimating the reporting rate $\lambda$\footnote{In this section, we assume a fixed incident type $\theta$ in our discussion, and so omit it from the notation} is the lack of reliable ground truth data. As we show in Appendix \Cref{prop:identi}, if we rely solely on \textit{either} the \textit{observed} number of incidents \textit{or} number of reports, it is impossible to distinguish heterogeneous reporting behavior under the influence of varying ground truth conditions, even in the limit of dataset size. In particular, the observed data can result from either incident rate differences or reporting disparities. The idea -- confounding incident occurrence and reporting -- is an example of the canonical \textit{benchmark problem}. Nevertheless, many works in the resident crowdsourcing literature conduct such analyses. 

% Our first intuition is that by studying the \textit{duplicate} reports, $\lambda_\theta$ is identifiable. This result may not come as a surprise: if reports are generated according to a Poisson process with rate $\lambda_\theta$ \textit{after a known birth time}, classical results (see e.g., \cite{resnick1992adventures}) show that the number of reports observed within a fixed interval of length $t$ after its birth is distributed as a Poisson random variable with rate $\lambda_\theta t$, thus rendering the estimation of $\lambda_\theta$ trivial. 

% However, in face of unknown incident birth time, choosing such intervals becomes more difficult; choosing a fixed interval length, potentially for all incidents is also an extremely inefficient way of utilizing our data -- some incidents are inspected (and thus considered resolved so no further reports are submitted) within a day of first being reported, choosing an interval length this short leads us to discard much data we observed for other incidents. To tackle this, our second intuition is that we can choose \textit{sample path dependent observation intervals}, so that the reporting rate is still identifiable using data observed during such intervals, and we can maximally utilize our data.

% Consider an incident $i$, born and died at unknown times $t_i$ and $t_i+T_i$. We impose separate conditions on the start time $S_i$ and end time $E_i$ of an observation interval: for the start time $S_i$, conditional on observing the first report, we need its distribution to be independent of the reporting rate $\lambda$; for the end time $E_i$, conditional on the (potentially more than one) reports observed at any point, its distribution needs to be independent of the reporting rate $\lambda_i$.\footnote{We additionally need two trivial conditions that (a) the start and end time are contained within the birth and death time, and (b) the start time is before the end time. We assume that any specifications we consider will satisfy these two conditions, which is indeed the case for the actual specification we use in our analyses.}

% Under the above conditions, suppose for each incident $i$, the data $\mathcal{D}_i$ we observe include $S_i = s_i$, $E_i = e_i$, the number of reports within time period $(s_i, e_i]$, denoted by $\tilde{M}_i$, and their associated report times. Then, conditional on the history of reports before $s_i$, denoted by $\mathcal{H}_i$, the likelihood of the data $\mathcal{D}_i$ as a function of the reporting rate $\lambda$ can be decomposed as
% \begin{equation}
%     \mathcal{L}(\lambda|\mathcal{D}_i, \mathcal{H}_i) = p\left(\tilde{M}_i;\lambda(e_i-s_i)\right)f(\mathcal{D}_i), \label{eq:decompose}
% \end{equation}
% where
% \begin{equation}
%     p\left(\tilde{M}_i;\lambda(e_i-s_i)\right) = \frac{\left[\lambda (e_i-s_i)\right]^{\tilde{M}_i}}{\tilde{M}_i!} \exp\left(-\lambda (e_i-s_i)\right) \label{eq:poissonlikelihood}
% \end{equation}
% is the probability mass function of a Poisson distributed random variable with $\tilde{M}_i$ occurrences and rate parameter $\lambda(e_i-s_i)$, and $f(\mathcal{D}_i)$ is a function that does not depend on $\lambda$.



% \zhi{a simplified rewrite of section 3 above}



The central methodological challenge in identifying and estimating the reporting rate $\lambda_\theta$ is the lack of reliable ground truth data. As we show in Appendix \Cref{prop:identi}, if we rely solely on \textit{either} the \textit{observed} number of incidents \textit{or} number of reports, it is impossible to distinguish heterogeneous reporting behavior under the influence of varying ground truth conditions, even in the limit of dataset size. In particular, the observed data can result from either incident rate differences or reporting disparities. The idea -- confounding incident occurrence and reporting -- is an example of the canonical \textit{benchmark problem}. Nevertheless, many works in the resident crowdsourcing literature conduct such analyses. 


This section first shows that $\lambda_\theta$ is identifiable by studying the \textit{duplicate} reports. We develop a method that decomposes the likelihood of the data, enabling the use of standard Poisson rate estimation techniques; then, we leverage this result to develop Bayesian Poisson regression approaches to tackle the high-dimensionality of $\theta$ and estimate $\lambda_\theta$ as a function of it.

\subsection{Identifying reporting rate \texorpdfstring{$\lambda_\theta$}{}}
\label{sec:identification}

We show that $\lambda_\theta$ is identifiable using just reporting data, \textit{if we use data on duplicate reports} about the same incident. In this section, we assume a \textit{fixed} incident type $\theta$, and so omit it from the notation. 
%
Our main insight is that one can identify the reporting rate using \textit{duplicate} reports about the same incidents: the first incident report informs us that this incident exists, and the remaining reports identify the reporting rate.


Our empirical strategy is based on the following result, which directly tackles the two challenges we face: not all incidents are observed, and for observed incidents, we still do not observe the birth and death times. Our result shows that, if we carefully construct an observation interval to count the number of duplicate reports, the likelihood function of the data can be decomposed to only depend on the reporting rate $\lambda$ through a Poisson likelihood function, thus we can leverage standard Poisson rate estimation techniques. 

Consider an incident $i$, born and died at unknown times $t_i$ and $t_i+T_i$. We impose separate conditions on the start time $S_i$ and end time $E_i$ of an observation interval: for the start time $S$, conditional on observing the first report, its distribution needs to be independent of the reporting rate $\lambda$;
%Intuitively, this means that after the first report came in, we would have all the information we need to determine the start time of the observation interval, and determining its value does not involve knowing $\lambda$. One candidate for this would be $S:=\{x\text{ days after the first report}\}$, where $x\ge 0$; for this specification, $S$ would be a fixed number with probability 1 after observing the first report, thus satisfying the condition.
for the end time $E_i$, conditional on observing the first report, its distribution needs to be independent of $S_i$; furthermore, conditional on the (potentially more than one) reports observed at any point, its distribution needs to be independent of the reporting rate $\lambda$. 
%This condition allows for more flexibility in our choices. Hypothetically, let us say the government agency has such a rule in determining the inspection time: if there are already $k$ reports of an incident, it will be inspected $100/k$ days after the first report. In this specification, even though as more reports pour in, the distribution of this inspection time keeps changing, it still satisfies this condition and can be used as the end of our observation period.\footnote{We additionally need two trivial conditions that (a) the start and end time are contained within the birth and death time, and (b) the start time is before the end time. We assume that any specifications we consider will satisfy these two conditions, which is indeed the case for the actual specification we use in our empirical analysis.}

% We next present an informal version of the result, and defer the formal version to the Appendix.

% This result shows that -- even if the observation interval for a Poisson process is defined by \textit{stopping times}, rather than the true birth and death times -- the likelihood function can be decomposed such that we can leverage standard Poisson rate estimation techniques. A time $t$ is \textit{stopping time} if it depends only on events that occur before that time (e.g., on the number of reports received up to time $t$); i.e., conditional on this past and type $\theta$, it is independent of the future and the process parameter $\lambda$.


\begin{restatable}{theorem}{thmst}\label{thm:stoppingtimes}
Under the above conditions, suppose for each incident $i$, the data $\mathcal{D}_i$ we observe include $S_i = s_i$, $E_i = e_i$, the number of reports within $(s, e]$, denoted by $\tilde{M}_i$, and their associated report times. Then, conditional on the history of reports before $s_i$, denoted by $\mathcal{H}_i$, the likelihood of the data $\mathcal{D}_i$ as a function of the reporting rate $\lambda$ can be decomposed as
\begin{equation}
    \mathcal{L}(\lambda|\mathcal{D}_i, \mathcal{H}_i) = p\left(\tilde{M}_i;\lambda(e_i-s_i)\right)f(\mathcal{D}_i), \label{eq:decompose}
\end{equation}
where
\begin{equation}
    p\left(\tilde{M}_i;\lambda(e_i-s_i)\right) = \frac{\left[\lambda (e_i-s_i)\right]^{\tilde{M}_i}}{\tilde{M}_i!} \exp\left(-\lambda (e_i-s_i)\right) \label{eq:poissonlikelihood}
\end{equation}
is the probability mass function of a Poisson distributed random variable with $\tilde{M}_i$ occurrences and rate parameter $\lambda(e_i-s_i)$, and $f(\mathcal{D}_i)$ is a function that does not depend on $\lambda$.
\end{restatable}

This result is a direct corollary of Appendix \Cref{thm:decomp}, which follows from decomposing the likelihood function into full conditional probabilities, and applying the two conditions.
%
The decomposition in \Cref{eq:decompose} enables standard Poisson rate estimation methods to be applied. For example, when we observe data associated with multiple reports indexed by $i$, 
%reporting rate is homogeneous ($\lambda(\tau) \triangleq \lambda$), 
the maximum likelihood estimate is:
\begin{equation}
\hat{\lambda}^{MLE} = \frac{\sum_{i}\tilde M_i}{\sum_{i}(e_i-s_i)}. \label{eq:MLE}
\end{equation}

Perhaps surprisingly, we could not find rate estimation literature in which observation period length $\tilde T_i$ also depends on the sample path,
%(but is a stopping time)
%and so require \Cref{thm:decomp}, in order 
which helps us use our data more efficiently. In our data, incidents may be fixed (via a work order) or reports may stop being tagged to the incident after an inspection -- these outcomes are represented by the death time $t_i + T_i$. However, these outcomes are potentially dependent on the reports: for example, incidents with more reports or reported as a \textit{Hazard} type may be prioritized for an inspection or work order. Without \Cref{eq:decompose}, classical Poisson process results (see e.g., \cite{resnick1992adventures}) require us to choose a fixed observation interval for all incidents, so that the likelihood of the data still adheres to the Poisson distribution as in \Cref{eq:decompose}, leading us to discard much data -- some incidents are inspected within a day of first being reported,.

% \Cref{thm:decompe} also allows the use of more data: in our data, incidents may be fixed (via a work order) or reports may stop being tagged to the incident after an inspection -- these outcomes are represented by the death time $t_i + T_i$. However, these outcomes are \textit{potentially dependent on the reports}: for example, incidents with more reports or reported as a \textit{Hazard} type may be prioritized for an inspection or work order. Without the above stopping time result, we would need to choose a fixed observation duration $\tilde T$ such that $\tilde t_i + \tilde T \leq t_i + T_i$ for all incidents $i$, leading us to discard much data -- some incidents are inspected within a day of first being reported. With \Cref{thm:decompe}, however, we can choose \textit{data dependent} duration $\tilde T_i$, as described below. 


\textbf{Applying the result to our setting.} How do we apply the above result to our setting? Given that we do not know birth time $t_i$ or lifetime $T_i$, we require a known interval $(S_i, E_i] \subseteq [t_i, t_i + T_i]$ such that we know the number of reports in that interval, and that $S_i$ and $E_i$ satisfy the desired conditions. Then, various standard Poisson rate estimation methods can be applied. 


The best choice for $S_i$ is the (observed) time of the first report, and so we count reports starting \textit{after} the first report---this time is the earliest that we know the incident exists, and so it maximizes the interval length. This choice formalizes the idea that our method uses the first report to establish an incident existing (and a timestamp for it), and then other reports to identify the reporting rate.

%  and before our chosen end time $\tilde t_i + \tilde T_i$


Setting $E_i$ is a design choice. 
%We require that the end time $\tilde t_i+ \tilde T_i$ is a stopping time, and that $\tilde t_i+ \tilde T_i \leq t_i + T_i$, i.e., that we do not extend the interval past when the incident can no longer be reported. Choosing too high a duration $\tilde T_i$ risks under-estimating $\lambda(\cdot)$; unfortunately, $t_i + T_i$ is unobserved and so the condition cannot be directly verified. On the other hand, choosing too low a duration $\tilde T_i$ throws away data, increasing variance. 
In our empirical application, we leverage government \textit{agency response} data, detailing the time when each incident was inspected or worked on. We choose the minimum of this time and $\tilde t_i + \bar T$, where $\bar T$ is a maximum duration design choice; we validate our estimates with multiple choices of $\bar T$ in \Cref{sec:robustnesstables}. Note that even though government agencies may vary their response time based on the number of reports received of one incident, these responses are made without knowledge of the actual reporting rate, and thus satisfy our required condition. The addition of $\bar T$ alleviates the concern that $E_i$ may extend beyond the actual and potentially unknown death time $t_i + T_i$ of an incident, and thus risk underestimating $\lambda$ -- agency responses may be delayed due to various reasons, by which time the incident may have already been resolved by other parties.


